Minimax Rates and Adaptivity in Combining Experimental and Observational Data

Randomized controlled trials (RCTs) are the gold standard for evaluating the causal effect of a treatment; however, they often have limited sample sizes and sometimes poor generalizability. On the other hand, non-randomized, observational data derived from large administrative databases have massive sample sizes and better generalizability, but they are prone to unmeasured confounding bias. It is thus of considerable interest to reconcile effect estimates obtained from randomized controlled trials and observational studies investigating the same intervention, potentially harvesting the best from both realms. In this paper, we theoretically characterize the potential efficiency gain of integrating observational data into the RCT-based analysis from a minimax point of view. For estimation, we derive the minimax rate of convergence for the mean squared error, and propose a fully adaptive anchored thresholding estimator that attains the optimal rate up to poly-log factors. For inference, we characterize the minimax rate for the length of confidence intervals and show that adaptation (to unknown confounding bias) is in general impossible. A curious phenomenon thus emerges: for estimation, the efficiency gain from data integration can be achieved without prior knowledge on the magnitude of the confounding bias; for inference, the same task becomes information-theoretically impossible in general. We corroborate our theoretical findings using simulations and a real data example from the RCT DUPLICATE initiative [Franklin et al., 2021b].

==> combining clinical and observational datasets/01-intro.tex <==
%!TEX root = 00-main.tex
\section{Introduction}
% \label{sec: intro}
Evaluating the causal effect of a medical treatment or policy intervention remains the central query in biomedical and social sciences. While the randomized controlled trials (RCTs) remain the gold standard \textcolor{black}{for generating high-quality causal evidence}, they often have limited sample sizes and are not representative of the target population of scientific interest \citep{rothwell2005external, Stuart:2011aa, deaton2009instruments,deaton2018understanding}. 
On the other hand, a plethora of observational data have been collected for administrative and research purposes and are increasingly available to researchers in the form of disease registries, biobanks, administrative claims databases and electronic health records. Observational data typically have massive sample sizes and better resemble the population of scientific interest; however, researchers often refrain from interpreting the obtained conclusion as \emph{causal} due to the almost universal concern of unmeasured confounding bias. In fact, according to authors instructions of the flagship {\it Journal of the American Medical Association} (\citealp{JAMA_instructions}), ``causal language (including use of terms such as effect and efficacy) should be used only for randomized clinical trials.'' The goal of this article is to study how to estimate the average treatment effect (ATE) of a well-defined target population by reconciling RCTs and observational studies investigating the same scientific question and potentially harvesting the best from both realms.

One important special case of our framework is estimating ATE of a target population using only relevant RCTs; in other words, we would like to generalize the RCT estimates to a target population of scientific interest. This topic has been extensively studied in the literature under the themes of ``generalizability", ``transportability'', and ``improving RCTs' external validity'' \citep{cole2010generalizing, Stuart:2011aa,tipton2013improving, pearl2014external,hartman2015sample, bareinboim2016causal,Buchanan:2018aa,Dahabreh:2019aa}; see review papers by \citet{colnet2020causal} and \citet{degtiar2021review} and references therein. 
In this special case, observational data are only used to inform researchers of subject characteristics in the target population; no treatment or outcome observational data are needed or leveraged in research along this line. 
Another important special case is when the target population concurs with the RCT study population and observational data are used to improve the efficiency of RCT estimates. 
To this end, \citet{gagnon2021precise} proposed a design-based approach that leverages large-scale observational data to fit regression or flexible machine learning models and conduct regression adjustment for randomization-based inference of RCT data; see \citet{aronow2013class} for similar strategies. 
Observational data are not used beyond helping gauge a better regression adjustment fit to improve the randomization inference efficiency and are thus not leveraged to their full potential.

Estimating causal effects using both RCTs and observational studies inevitably involves the century-old bias-variance trade-off. 
Observational data play the role of double-edged sword here: they are blessed with a sometimes enormous sample size and could dramatically improve estimation precision under suitable conditions; 
on the other hand, they may leak bias into the otherwise unbiased RCT estimates. 
Developing a principled and adaptive approach to bias-variance trade-off thus lies at the heart of combining RCTs and observational studies for optimal ATE estimation. 
To the best of our knowledge, few works have formally studied this problem, let alone the development of adaptive algorithms.
% to combining RCTs and observational studies. 
Two notable exceptions are \citet{yang2020elastic} and \citet{yang2020improved}. The former developed a hypothesis-testing-based integrative estimator that pools the RCT data and observational data when a certain criterion is met. The bias-variance trade-off is controlled by the choice of the critical region when testing whether the observational data violate the no unmeasured confounding assumption. 
The latter posited a functional form on the unmeasured confounding bias and proposed to estimate it using semiparametric theory. 
However, both works rely on the assumption that the sample size ratio between the observational data and the RCT data is \emph{bounded}. Such an assumption does not capture the fact that the sample size of observational data can be \emph{much larger} than that of the RCT data, and it effectively rules out the possibility of obtaining \emph{order-wise} improvement, even if the confounding bias is negligible.

% Under their framework, the bias-variance trade-off is controlled by the choice of the critical region when testing whether the observational data violate the no unmeasured confounding assumption. Although \citet{yang2020elastic} provide a data-driven approach to selecting the critical region, it lacks theoretical underpinnings.

Our overarching goal is to theoretically characterize the potential efficiency gain from integrating observational data into the analysis based on RCT alone. 
The main contributions are two-folds. 
\begin{enumerate}
\item For estimation, we derive the minimax rate of convergence for the mean squared error. Interestingly, the rate can be achieved by an oracle estimator that takes a \emph{dichotomous} form: when the magnitude of the confounding bias exceeds a certain threshold, we estimate the causal effect using the RCT alone; when the magnitude is below this threshold, we pool the two data sources together, as if the confounding bias never exists.
We further propose a fully adaptive estimator, termed \emph{anchored thresholding} estimator, that nearly attains the minimax rate up to poly-log factors without any prior knowledge on the magnitude of the bias. 
% of any combined estimator and show that the optimal rate can be achieved by an estimator that is anchored at the RCT-based-estimator and adapts to the unknown internal validity bias of the estimator based on observational data. 

\item For statistical inference, we characterize the minimax {rate for the} length of confidence intervals (CIs).  {The minimax rate for CI length is similar in functional form to that for estimation, and can be attained similarly by a dichotomous oracle procedure.}
However, the story for adaptivity becomes drastically different.
We show that constructing adaptive CIs that attains the minimax rate is generally impossible, unless there is strong prior knowledge on the magnitude of the confounding bias.
As a corollary, our results indicate the existence of a threshold such that 
if one does not believe the magnitude of confounding bias is much smaller than this threshold, then \emph{any} uniformly valid CIs can only outperform the RCT-only CI by at most a constant factor.
% of any uniformly valid confidence interval and prove that adaptation is impossible with unknown internal validity bias of the estimator based on observational data.
\end{enumerate}


%\textcolor{red}{1. Introduce notation, estimands and assumptions. 2. Review estimates of causal effects in RCT and observational studies. 3. Describe and dissect sources of bias. 4. Describe an oracle best linear combination and its properties. 5. Describe an adaptive approach. 6. Construct confidence interval. 7. Simulation studies. 8. Real data.}

\noindent\textbf{Notations.}
We conclude this section by introducing some notations that will be used throughout this paper. 
Given $a, b \in \bbR$, we denote $a\lor b = \max\{a, b\}$ and $a\land b = \min\{a, b\}$.
For two positive sequences $\{a_n\}$ and $\{b_n\}$, we write 
$a_n \lesssim b_n$ to denote $\limsup a_n/b_n < \infty$, 
and we let $a_n \gtrsim b_n$ to denote $b_n \lesssim a_n$. 
Meanwhile, the notation $a_n\asymp b_n$ means $a_n \lesssim b_n$ and $a_n \gtrsim b_n$ simultaneously.
Moreover, we write $a_n\ll b_n$ or $a_n = o(b_n)$ to mean $b_n/a_n\to\infty$ and $a_n\gg b_n$ to mean $b_n \ll a_n$.
We use $\overset{p}{\to}$ to denote convergence in probability and we use $X_n = o_p(1)$ to denote $X_n\overset{p}{\to} 0$.

==> combining clinical and observational datasets/02-setup.tex <==
%!TEX root = 00-main.tex
\section{Set-up}
\label{sec: setup}
\subsection{Estimands and Baseline Estimators}
Suppose the existence of a binary treatment $ A\in \{0,1\} $, potential outcomes $\{Y(1), Y(0)\}$ and baseline observed covariates $\mathbf{X}$. 
Throughout the article, we assume the consistency and Stable Unit Treatment Value Assumption (SUTVA)  so that the observed outcome $Y$ satisfies $Y= AY(1) + (1-A)Y(0)$ \citep{Rubin1980}.
Our estimand of interest is the average treatment effect of a target population (PATE) $\beta^\star = \mathbb{E}[Y{(1)} - Y{(0)}]$, where $\mathbb{E}[\cdot]$ is taken with respect to the joint distribution of $(\mathbf{X}, Y(0), Y(1))$ over the target population. 


A random sample of size $n_c$ from the target population was selected into an RCT according to some sample selection protocol. We use $S = c$ to indicate selection into the RCT and let $\mathcal{C}$ denote the associated index set so that $|\mathcal{C}| = n_c$. We write the RCT data as $\mathcal{D}_{c} = \{(Y_i, A_i, \mathbf{X}_i, S_i = c):~i \in \mathcal{C}\}$, which are  assumed to be independent and identically distributed according to the joint law of $\big(Y(1), Y(0), A, \mathbf{X}\big) \mid S = c$. We denote the average treatment effect in the RCT population as $\beta^\star_{c} = \mathbb{E}[Y(1) - Y(0) \mid S = c]$. 
\begin{assumption}[Design of RCT]\label{assump: design of RCT} \rm
Assume $A \indep (Y(1), Y(0)) \mid \mathbf{X}, S=c$, the treatment assignment probability $ \pi_c(\mathbf{x}):= P(A=1\mid \mathbf{X}=\mathbf{x}, S=c) $ is \emph{known}, and $\pi_c(\mathbf{X})>0$ with probability 1 with respect to the law of $\bfX\mid S = c$. 
\end{assumption}

Under Assumption \ref{assump: design of RCT},  $\beta^\star_c$ is identified from  $\mathcal{D}_c$ and can be estimated via the inverse probability weighting (IPW) estimator  \citep{horvitz1952generalization}:
\begin{equation}
\label{eq:cipw}
\hat\beta_{c, \textsf{IPW}}  = \frac{1}{n_c} \sum_{i\in \mathcal{C}}  \bigg(\frac{A_i Y_i }{\pi_c(\mathbf{X}_i)} - \frac{(1-A_i) Y_i }{1- \pi_c(\mathbf{X}_i)}\bigg).
\end{equation}
Alternatively, $\beta^\star_c$ can be estimated via the following augmented inverse probability weighting (AIPW) estimator \citep{robins1994estimation, bang2005doubly}:
\begin{align*}
% \begin{split}
\hat\beta_{c, \textsf{AIPW}}
&  = \frac{1}{n_c} \sum_{i\in \mathcal{C}}\bigg(\frac{A_i (Y_i -\mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} ) )  }{\pi_c(\mathbf{X}_i)} - \frac{(1-A_i)(Y_i -\mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ) ) }{1- \pi_c(\mathbf{X}_i)} \\
\label{eq:caipw}
& \qquad \qquad \qquad +\mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} )   - \mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} )\bigg),\numberthis
% \end{split}
\end{align*}
where  $ \mu_{ca}(\bfx; \bsalpha_{ca} )$ is a parametric specification (parametrized by $\bsalpha_{ca}$) of the conditional outcome mean $\mu_{ca}(\bfx) = \mathbb{E}[Y \mid \bfX=\bfx, A = a, S = c]$ and $ \hat \bsalpha_{ca} $ an estimator of $ \bsalpha_{ca}$, for $a=0,1$. 
In an RCT with known treatment assignment probability $\pi_c(\bfx)$, the AIPW estimator $ \hat\beta_{c, \textsf{AIPW}}$ consistently estimates $\beta^\star_c$ even when $\mu_{ca} (\bfx; \bsalpha_{ca})$ do not correctly specify $\mu_{ca}(\bfx)$, and is semiparametric efficient if they do \citep{bang2005doubly,tsiatis2007semiparametric}. 
The AIPW estimator $ \hat\beta_{c, \textsf{AIPW}}$ is also guaranteed to be more efficient than $\hat\beta_{c, \textsf{IPW}}$ when $\pi_c(\bfx)$ does not depend on the covariate vector $\bfx$ (e.g., under random treatment assignment),  $\mu_{ca}(\bfx; \bsalpha_{ca})$ are linear parametric models of $\mu_{ca}(\bfx)$, and $ \hat \bsalpha_{ca}$ are the corresponding least squares estimators \citep{tsiatis2008covariate, ye2020principles}. 

In parallel, a random sample of size $n_o$ from the target population was collected in an observational study. We use $S = o$ to indicate selection into the observational study and let $\mathcal{O}$ denote the associated index set so that $|\mathcal{O}| = n_o$. Typically, $n_o \gg n_c$.  We write the observational data as
$\mathcal{D}_{o} = \{(Y_i, A_i, \mathbf{X}_i, S_i = o):~i \in \mathcal{O}\}$, which are assumed to be independent and identically distributed according to the joint law of $\big(Y(1), Y(0), A, \mathbf{X}\big) \mid S = o$. We denote the  average treatment effect in the observational study population as $\beta^\star_{o} = \mathbb{E}[Y(1) - Y(0) \mid S = o]$. Without additional assumptions, $\beta^\star_\rct \neq \beta^\star_\obs$ and neither agrees with the estimand of interest $\beta^\star$. 
    
For estimation, we impose a positivity assumption on the treatment assignment probability in the observational data  \citep{rosenbaum1983central}. 

\begin{assumption}[Positivity of Treatment Assignment in Observational Study]\label{assump: positivity obs} 
Assume the treatment assignment probability $\pi_o(\mathbf{X}):= P(A=1\mid \bfX, S=o)>0$ with probability 1 with respect to the law of $\bfX \mid S = \obs$.
\end{assumption}
Let  $\mu_{oa}(\bfx) = \mathbb{E}[Y \mid \mathbf{X}=\bfx, A = a, S = o]$ be the conditional outcome means in the observational data, and  $\mu_{oa}(\bfx;  \bsalpha_{oa})$ be their corresponding parametric specifications for $a = 0, 1$. Also let $\pi_{o}(\bfx; \bseta)$ be a parametric specification of $\pi_o(\bfX)$. Under Assumption \ref{assump: positivity obs},  the observational study counterparts of $\cipw$ and $\caipw$ defined in \eqref{eq:cipw} and \eqref{eq:caipw} can then be formed as
\begin{align}
\label{eqn:oipw}
    \hat\beta_{o, \textsf{IPW}} &= \frac{1}{n_o} \sum_{i\in \mathcal{O}}  \bigg(\frac{A_i Y_i }{\pi_{o}(\mathbf{X}_i; \hat \bseta)} - \frac{(1-A_i) Y_i }{1- \pi_{o}(\mathbf{X}_i; \hat \bseta) }\bigg) ,\\
        \hat    \beta_{o, \textsf{AIPW}} &=  \frac{1}{n_o} \sum_{i\in \mathcal{O}}\bigg(\frac{A_i (Y_i -\mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} ) )  }{\pi_{o}(\mathbf{X}_i; \hat\bseta )} - \frac{(1-A_i)(Y_i -\mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} ) ) }{1- \pi_{o}(\mathbf{X}_i;\hat\bseta)}  \nonumber\\
\label{eqn:oaipw}
        & \qquad \qquad\qquad + \mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} )   - \mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} )\bigg),
\end{align}
where $\hat\bseta$ and $\hat\bsalpha_{oa}$ are estimators of $\bseta$ and $\bsalpha_{oa}$, respectively. 

\subsection{Internal Validity Bias}
\label{subsec: internal validity}

Internal validity refers to an effect estimate being (asymptotically) unbiased for the causal effect. Under Assumption \ref{assump: design of RCT} which states that treatment assignment in the RCT population is manipulated by the experimenter and depends only on the observed covariates, both $\hat\beta_{c, \textsf{IPW}}$ and $\hat\beta_{c, \textsf{AIPW}}$ are internally valid: they are consistent and asymptotically normal estimators for the causal estimand $\beta^{\star}_c$.  On the other hand, under  Assumption \ref{assump: positivity obs}, $\hat\beta_{o, \textsf{IPW}}$ and $\hat\beta_{o, \textsf{AIPW}}$ have internal validity bias as they are estimating a non-causal quantity $
\beta_o=\mathbb{E}\left[Y\mid  S = o, A=1\right] - \mathbb{E}\left[Y\mid  S = o, A=0\right]
$, which is not necessarily equal to $\beta^\star_o$ due to unmeasured confounding; see Appendix \ref{appx:internal_bias} for a more detailed analysis of the internal validity bias. 






\subsection{External Validity Bias}
\label{subsec: external validity}
External validity is concerned with how well the effect estimates generalize to other contexts \citep{degtiar2021review}. This bias often arises from the interplay between effect heterogeneity and the difference between the study and target populations. We focus primarily on the setting where the observational data represent the target population, as formalized below.
\begin{assumption}[Target Population]\label{assump:target}
% either one of the following holds:
% \begin{itemize}
    % \item[(a)] The RCT data represent the target population, so that $(\mathbf{X}, Y(0), Y(1)\mid S=c) \overset{d}{=} ( \mathbf{X}, Y(0), Y(1))$;
    % \item[(b)] 
   The target distribution $(Y(1), Y(0), \bfX)$ and the observational study population $(Y(1), Y(0), \bfX)\mid S=o$ are the same.
% \end{itemize}
\end{assumption}



We remark that our method and theory developed in Sections \ref{sec:estimation} and \ref{sec:inference} can be extended in a \emph{mutatis mutandis} fashion to accommodate other settings, such as when the RCT data represent the target population, or even when there is a separate target population that is distinct from either RCT or observational data. 
% For ease of exposition, we defer the discussion of such extensions to Appendix \ref{appx:rct_as_target}.

% In contrast, the former setting is relevant when the investigator is interested only in the subjects with a particular set of characteristics.
% Before proceed further, we remark that our method and theory developed in Section \ref{sec: method} could be extended in a \emph{mutatis mutandis} fashion to handle the case where there is a separate target population that is different from the population represented by either the RCT or the observational data. But we do not pursue this direction in this article. 
% \paragraph{The observational population is the target.}

It is clear that $\beta^\star = \beta^\star_\obs$ under Assumption \ref{assump:target}. When the observational data are representative of the target population, the two RCT-based estimators $\cipw$ and $\caipw$, albeit internally valid, may suffer from external validity bias. To eliminate the external validity bias, we make the following standard \emph{conditional mean exchangeability} assumption, also known as the \emph{generalizability} assumption \citep{Stuart:2011aa, Dahabreh:2019aa, degtiar2021review}. 

\begin{assumption}[Conditional Mean Exchangeability]\label{assump: study selection exchangeability} 
$\mathbb{E}[Y(1)- Y(0)| \mathbf{X}, S = c] = \mathbb{E}[Y(1)- Y(0) | \mathbf{X}]$.
\end{assumption}

Assumption \ref{assump: study selection exchangeability} states that participating in the RCT does not modify the treatment effect in every strata defined by $\mathbf{X}$, which will hold if all patient characteristics that modify the treatment effect and differ between the RCT population and the target population are measured.  

Under Assumptions \ref{assump:target}, \ref{assump: study selection exchangeability} and a often-made \emph{RCT participation positivity} assumption which states that the participation probability defined as $e_\rct(\bfx) = \bbP(S = \rct\mid \bfX =\bfx, S \in \{\rct, \obs\})$ is strictly bounded away from $0$ and $1$ almost surely, the PATE  $\beta^\star$ can be identified from the RCT data via inverse probability of participation weighting (IPPW) or augmented inverse probability of participation weighting (AIPPW) \citep{Stuart:2011aa,Dahabreh:2019aa,lu2019causal, degtiar2021review}. 
Here we use $S \in \{\rct, \obs\}$ to indicate that the probability is calculated for a subject in the RCT or the observational study. 
However, in practice, the  RCT participation probability would decay to zero if $n_\obs\gg n_\rct$ as both $n_o$ and $n_c$ go to infinity, thus invalidating the  RCT participation positivity assumption.  For this reason, we make a weaker assumption that does not assume away  decaying RCT participation probability.


\begin{assumption}[Bounded Density Ratio]
% \label{assump: bdd density ratio}
Assume $\bbP(\mathbf{X}= \mathbf{x}\mid S=o) / \bbP( \mathbf{X}= \mathbf{x} \mid S=c)<\infty$ for all $\mathbf{x}$ with positive density in the target population. 
\end{assumption}

To tackle the challenge imposed by decaying RCT participation probability, we randomly sample a subset of size $n_c$ from the observational data, denoted as $\mathcal{D}_{\mathcal{O}_1}$, and use $\mathcal{D}_{\mathcal{C}}\cup\mathcal{D}_{\mathcal{O}_1} $ to estimate the RCT participation probability and then adjust for the external validity bias of the RCT-based estimators using IPPW or AIPPW as follows:
\begin{align*}
\begin{split}
    \hat\beta_{c, \textsf{IPPW}}  &= \frac{1}{n_c} \sum_{i\in \mathcal{C}} \bigg[ \frac{A_i Y_i }{\pi_c(\mathbf{X}_i)} - \frac{(1-A_i) Y_i }{1- \pi_c(\mathbf{X}_i)}\bigg] \frac{ 1-e_{{c}}(\mathbf{X}_i; \hat  \bsxi )  }{e_{{c}}(\mathbf{X}_i; \hat  \bsxi )    },\\
\hat\beta_{c, \textsf{AIPPW}}   & = \frac{1}{n_c} \sum_{i\in \mathcal{C}} \bigg[\frac{A_i (Y_i -\mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} ) )  }{\pi_c(\mathbf{X}_i)} - \frac{(1-A_i)(Y_i -\mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ) ) }{1- \pi_c(\mathbf{X}_i)}  \bigg] \frac{ 1-e_{{c}}(\mathbf{X}_i; \hat  \bsxi )  }{e_{{c}}(\mathbf{X}_i; \hat  \bsxi )  } \\
&\qquad + \frac{1}{n_c} \sum_{i\in \mathcal{O}_1} \mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} )   - \mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ),
\end{split}
\end{align*}
where $e_{{c}}(\mathbf{x};  \bsxi )$ is a parametric specification of $e_\rct(\bfx)$ and $\hat \bsxi$ an estimator of $ \bsxi$ obtained from $\mathcal{D}_{\mathcal{C}}\cup\mathcal{D}_{\mathcal{O}_1} $. 
It can be shown that when $e_{{c}}(\mathbf{X}_i;  \bsxi )$ is correct, the probability limit of $\hat\beta_{c, \textsf{IPPW}} $ is $\beta^\star$; when either  $e_{{c}}(\mathbf{X}_i;  \bsxi )$ or $ \{\mu_{c1} (\mathbf{X}_i;  \bsalpha_{c1} ),  \mu_{c0} (\mathbf{X}_i;  \bsalpha_{c0} )\}$ is correct,  the probability limit of $\hat\beta_{c, \textsf{AIPPW}} $ is $\beta^\star$ \citep{Dahabreh:2019aa}. 

The remaining observational data $\mathcal{D}_{\mathcal{O}_2} = \mathcal{D}_{\mathcal{O}}\setminus\mathcal{D}_{\mathcal{O}_1}$ of size $n_{o_2}$ are then used to construct estimators $\hat\beta_{o_2,\textsf{IPW}}$ and $\hat\beta_{o_2,\textsf{AIPW}}$ according to \eqref{eqn:oipw} and \eqref{eqn:oaipw}, which potentially suffer from the internal validity bias as discussed in Section \ref{subsec: internal validity}. In practice, IPW-type estimators like $\cippw, \caippw, \ooipw$, and $\ooaipw$ may be unstable when the (estimated) weights are close to zero, and researchers often stabilize the weights by normalization  \citep{robins2007comment}; we use $\hat\beta_{c, \textsf{sIPPW}}$, $\hat\beta_{c, \textsf{sAIPPW}}$, $\hat\beta_{o_2, \textsf{sIPW}}$, and $\hat\beta_{o_2, \textsf{sAIPW}}$ to denote their stabilized versions. More details are provided in Appendix \ref{appx:stablization}.

The consistency, asymptotic normality, and influence function representation of all aforementioned estimators are standard and can be immediately obtained from \citet[Chapter 6.1]{newey1994}; see Appendix \ref{appx:influence_func} for details.

==> combining clinical and observational datasets/03-method.tex <==
%!TEX root = 00-main.tex


\section{Estimation}\label{sec:estimation}


\subsection{An Oracle Estimator and Its Optimality}
\textcolor{black}{
Let $\hat \beta_\rct$ denote a generic estimator constructed from the RCT data and $\hat \beta_\obs$ a generic estimator constructed from the observational data.
For instance, if there is no external validity bias, then researchers could take $\hat\beta_\rct = \hat\beta_{c, \textsf{IPW}}$, or $\hat\beta_{\rct} = \hat\beta_{\rct, \textsf{AIPW}}$, or their stabilized versions, and $\hat\beta_\obs = \hat\beta_{o, \textsf{IPW}}$, or $\hat\beta_\obs = \hat\beta_{o, \textsf{AIPW}}$, or their stabilized versions.
In the presence of external validity bias, based on the discussion in Section \ref{subsec: external validity}, it is desirable to choose $\hat\beta_\rct = \hat\beta_{c, \textsf{IPPW}}$, or $\hat\beta_\rct = \hat\beta_{c, \textsf{AIPPW}}$, or their stabilized versions, and $\hat\beta_\obs = \hat\beta_{o_2, \textsf{IPW}}$, or $\hat\beta_\obs = \hat\beta_{o_2, \textsf{AIPW}}$, or their stabilized versions.}
Recall that $\hat\beta_\obs$ potentially suffers from the internal validity bias quantified by 
\begin{equation*}
    % \label{eq:bias}
\Delta =  \beta^\star - \beta_\obs.
\end{equation*}

% \sxc{Use $n_c, n_o$ only, mention that when we use IPPW, we need to overload $n_c \leftarrow n_c+n_{o_1}, n_o \leftarrow n_{o_2}$}
We assume both $\hat\beta_\rct$ and $\hat\beta_\obs$ admit asymptotic linear expansions, formalized by Assumption \ref{assump:asymp_linear}.
\begin{assumption}[Existence of Asymptotic Linear Expansions]
\label{assump:asymp_linear}
Suppose there exist influence functions $\psi_\rct(\bfX, A, Y)$, $\psi_\obs(\bfX, A, Y)$ such that as $n_\rct \land n_{\obs} \to \infty$, 
% \tye{for $\hat\beta_c$, should be $2n_c$ and  $\sum_{i\in \mathcal{C}\cup \mathcal{O}_1}$. Maybe in this section, redefine $\mathcal{C}$ and $\mathcal{O}$ to be general notations.} \sxc{should be fine since we can absorb the factor of 2 into $\psi_\rct$?} \tye{You are right. But still need $\sum_{i\in \mathcal{C}\cup \mathcal{O}_1}$ for the IPPW and AIPPW estimator.}
\begin{align*}
    \sqrt{n_\rct}(\hat\beta_\rct - \beta^\star) &  = \frac{1}{\sqrt{n_\rct}} \sum_{i\in \Rct}  \psi_\rct(\bfX_i, A_i, Y_i) +  o_p(1),  \\
    \sqrt{n_{\obs}}(\hat\beta_\obs - \beta_\obs) &  = \frac{1}{\sqrt{n_{\obs}}} \sum_{i\in\Obs}  \psi_\obs(\bfX_i, A_i, Y_i) +  o_p(1).
\end{align*}
Moreover, the influence functions are mean zero with finite second and third moments given by $\bbE[(\psi_\rct(\bfX_i, A_i, Y_i))^2] = \sigma_\rct^2$ and $\bbE[|\psi_\rct(\bfX_i, A_i, Y_i)|^3] = \rho_\rct$ for all $i \in \calC$, and $\bbE[(\psi_\obs(\bfX_i, A_i, Y_i))^2] = \sigma_\obs^2$ and $\bbE[|\psi_\obs(\bfX_i, A_i, Y_i)|^3] = \rho_\obs$ for all $i \in \Obs$. 
\end{assumption}

\begin{remark}
The asymptotic linear expansion part of Assumption \ref{assump:asymp_linear} is satisfied by various choices of $\hat\beta_\rct$ and $\hat\beta_\obs$; see Section \ref{subsec: internal validity} and \ref{subsec: external validity}. 
Assumption \ref{assump:asymp_linear} also assumes the existence of finite third moments as our analysis makes use of the Berry-Essen theorem. While this assumption could be relaxed, e.g., by invoking generalizations of Berry-Esseen theorem that only requires finite fractional moment \citep[Chapter 16]{feller2008introduction}, we do not pursue it here.
\end{remark}
\begin{remark}
    \textcolor{black}{
    Careful readers may have noticed that the asymptotic linear expansion technically does not hold for settings when a part of the observational data is used in the construction of $\hat\beta_\rct$ (e.g., $\hat\beta_{\rct, \textsf{IPPW}}$ and $\hat\beta_{\rct, \textsf{AIPPW}}$). However, in such scenarios, we can simply overload the notations and re-define 
    % $n_\rct \leftarrow n_\rct + n_{o_1}= 2 n_\rct, 
    $\calC \leftarrow \calC \cup \calO_1$, $n_\obs\leftarrow n_{\obs_2}$, and $\calO\leftarrow\calO_{2}$, and all the theoretical results in later sections will hold provided $n_\obs \geq (1+\ep)n_\rct$ for some absolute constant $\ep >0$.}
\end{remark}

% \sxc{From now on, $n_{o_2}$ and $\calO_2$ should NOT appear in our method and theory sections.}

% \tye{"allow to be arbitrarily large" is still confusing. E.g., in the next section, we allow $\Delta$ to be arbitrarily large, and our adaptive estimator should be the optimal choice (rather than $\hat\beta_c$).}                                                                                                                                                                                                                             
% \sxc{Move ``if we have prior knowledge on $\overline{\Delta}$'' earlier and talk about $\overline{\Delta}$ only}

\textcolor{black}{
Let us introduce a scalar $\overline\Delta \geq 0$ and assume that $|\Delta| \leq \overline\Delta$.
To motivate the procedure, consider the following two extreme cases.
If $\overline\Delta$ is very large, then in the worst case, incorporating the observational data can only do harm to our task of estimating $\beta^\star$. 
In this case, the worst-case optimal choice is arguably the RCT-only estimator $\hat\beta_\rct$. 
On the other hand, if $\overline{\Delta}$ is negligibly small, then the problem is reduced to aggregating two asymptotically (almost) unbiased and Gaussian estimators.
 % to minimize the overall variance. 
As the bias is negligibly small, a natural choice is taking the convex combination of the two estimators, with the weights chosen to minimize the overall variance:}
\begin{align}
    \label{eq:naive_estimator}
    \hat\beta_\weight = (1-\weight) \hat\beta_\rct + \weight \hat \beta_\obs,
    \qquad 
    \textnormal{where }
    \weight = \frac{\sigma_\rct^2/n_\rct}{ \sigma_\rct^2/n_\rct + \sigma_\obs^2/n_{\obs}}.
\end{align}
We refer to $\hat\beta_\weight$ as the \emph{naively-pooled} estimator.

\textcolor{black}{Following the above discussion, if we have prior knowledge on $\overline\Delta$, then we can choose which estimator to use based on the magnitude of $\overline\Delta$.}
In particular, we can implement the following oracle strategy: (1) when $\overline\Delta$ exceeds a certain threshold, then use the RCT-only estimator; (2) when $\overline\Delta$ is below that threshold, then use the naively-pooled estimator. The performance of such a procedure is given in the following theorem.

\begin{theorem}[Performance of the Oracle Estimator]
\label{thm:oracle_estimator}
For any estimator $\hat\beta$ of $\beta^\star$, we let $\amse(\hat\beta)$ be its asymptotic mean-squared error, so that 
$
    {\bbE[|\hat \beta - \beta^\star|^2]}/{\amse(\hat\beta)} \to 1
$
as $n_\rct \land n_{\obs}\to \infty$.
Under Assumption \ref{assump:asymp_linear}, as $n_\rct\land n_{\obs} \to \infty$, we have
\begin{align*}
    % \label{eq:amse_baselines}
    \amse(\hat\beta_\rct) = \frac{\sigma_\rct^2}{n_\rct},
    \qquad
    \amse(\hat\beta_\weight) =  \frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} + \bigg(\frac{\sigma_\rct^2/n_\rct}{\sigma_\rct^2/n_\rct + \sigma_\obs^2/n_{\obs}}\bigg)^2 \cdot \Delta^2.
\end{align*}
% If we additionally assume $n_\obs \geq (1+\ep)n_\rct$ for some {absolute} constant $\ep > 0$ (i.e., the observational data are more abundant than the RCT data), then 
As a result, the following oracle estimator
\begin{align}
    \label{eq:oracle_estimator}
    \hat\beta_{\orac} = 
    \begin{cases}
        \hat\beta_\rct & \textnormal{ if } \overline\Delta \geq {\sigma_\rct}/{\sqrt{n_\rct}}\\
        \hat\beta_\weight & \textnormal{ otherwise}
    \end{cases}
\end{align}
satisfies 
\begin{align}
    \label{eq:amse_oracle_estimator}
    \amse(\hat\beta_\orac) \leq\frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} + \frac{\sigma_\rct^2}{n_\rct} \land \overline\Delta^2.
\end{align}
\end{theorem}
\begin{proof}
    See Appendix \ref{prf:thm:oracle_estimator}.
\end{proof}

The choice of setting the threshold at $\sigma_\rct/\sqrt{n_\rct}$ in the oracle estimator is based on the following calculations. Note that in practice, the observational data are usually much more abundant than the RCT data, i.e., ${\sigma_\obs^2}/{n_{\obs}} \ll \sigma_\rct^2/n_\rct$. In this case, we have $\weight = 1 + o(1)$, and ${\sigma_\rct^2 \sigma_\obs^2}/({n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2}) \ll {\sigma_\rct^2}/{n_\rct}$. 
Thus, we can simplify the formula for $\amse(\hat\beta_\weight)$ as $o(\sigma_\rct^2/n_\rct) + (1+o(1))\Delta^2$.
It follows that the RCT-only estimator would outperform the naively-pooled estimator (in terms of $\amse$) provided the magnitude of the bias exceeds $\sigma_\rct/\sqrt{n_\rct}$.
Such a choice of the threshold is also intuitive from the perspective of the classical bias-variance decomposition: incorporating $\hat\beta_\obs$ will only be useful if its bias does not exceed the standard deviation of $\hat\beta_\rct$.


Curious readers may wonder if the upper bound in \eqref{eq:amse_oracle_estimator}, achieved by the oracle estimator, is information-theoretically optimal among all estimators.
In the following, we describe a simple yet canonical data-generating process and show that $\hat\beta_\orac$ is indeed minimax rate optimal. 
Apart from being a model of what happens in practice, this data generating process serves as a theoretical benchmark that enables us to give a rigorous treatment of optimality. 
% Before diving into details, we emphasize that the data generating process we are to describe \textcolor{red}{should \emph{not} be interpreted as any realistic model of what happens in practice}. Rather, it serves as a theoretical benchmark that enables us to give a rigorous treatment of optimality.

\begin{model}
\label{model}
Suppose the RCT data are generated as follows. For each $i\in\Rct$, we first generate a covariate vector $\bfX_i\sim \bbP_{X}$. Then, we generate the treatment $A_i \sim \Bern(\pi_\rct(\bfX_i))$ for some function $\pi_\rct(\bfx) \in (0, 1)$. 
Finally, we generate $Y_i(A_i) \sim N((A_i-1/2)\beta^\star + \bsgamma_\rct^\top \bfX_i, \sigma_\rct^2)$ where $\bsgamma_\rct$ is a vector with the same dimension as $\bfX_i$. 

Meanwhile, suppose the observational data are generated as follows. 
For each $i\in\Obs$, we first generate the treatment $A_i\sim \Bern(\pi_\obs)$ for some scalar $\pi_\obs\in(0, 1)$.
Then, we generate an unmeasured confounding variable $U_i\sim N(-(A_i-1/2)\Delta, \sigma_\obs^2/2)$ and a covariate vector $\bfX_i\sim \bbP_{X}$.
% Hence, we have $\bfX_i\perp (A_i, U_i)$.  
We finally generate $Y_i(A_i)\sim N((A_i-1/2)\beta^\star + U_i + \bsgamma_\obs^\top \bfX_i, \sigma_\obs^2/2)$, where $\bsgamma_\obs$ is a vector with the same dimension as $\bfX_i$. 
\end{model}

By the design of RCT (i.e., Assumption \ref{assump: design of RCT}), the observed responses in the RCT data satisfy 
$$
Y_i\mid A_i, \bfX_i \overset{i.i.d.}{\sim} N((A_i-1/2)\beta^\star + \bsgamma_\rct^\top \bfX_i, \sigma_\rct^2).
$$ 
From our discussion in Section \ref{sec: setup}, it is easy to construct an estimator $\hat\beta_\rct$ that is asymptotically normal with mean $\beta^\star$ and variance of order $\sigma_\rct^2/n_\rct$ (note that we do not need to weight by the participation probability as $\beta^\star_\rct = \beta^\star_\obs = \beta^\star$ in the above model).
Meanwhile, marginalizing over $U_i$, the observed responses in the observational data satisfy 
$$
Y_i\mid A_i, \bfX_i \overset{i.i.d.}{\sim} N((A_i-1/2)\beta_\obs + \bsgamma_\obs^\top \bfX_i , \sigma_\obs^2),
$$ 
where $\beta_\obs = \beta^\star - \Delta$. Thus, even if $\bsgamma_\obs$ is known, the best one can do is to produce an estimator $\hat\beta_\obs$ that is centered at $\beta_\obs$. 

Consider the following parameter space:
\begin{align}
    \label{eq:param_space}
    \calP_{\overline\Delta} = \{(\beta^\star, \beta_\obs): |\beta^\star - \beta_\obs|\leq \overline\Delta\}.
\end{align}
The following theorem gives the minimax lower bound under Model \ref{model}.

\begin{theorem}[Minimax Lower Bound]
\label{thm:lb}
Under Model \ref{model}, we have
\begin{equation*}
    % \label{eq:lb}
    \inf_{\hat \beta} \sup_{(\beta^\star, \beta_\obs)\in\calP_{\overline\Delta}} \bbE[|\hat\beta - \beta^\star|^2] \gtrsim \frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} + \frac{\sigma_\rct^2}{n_\rct} \land \overline\Delta^2,
\end{equation*}
where the infimum is taken over all measurable functions of the observed RCT and observational data.
\end{theorem}
\begin{proof}
    See Appendix \ref{prf:thm:lb}.
\end{proof}



\begin{figure}[t]
    \centering
    \includegraphics[width = 0.49\textwidth]{phase_transition.pdf}
    \caption{Phase transition for the minimax rate. When $\overline\Delta\gtrsim \sigma_\rct/\sqrt{n_\rct}$, the RCT-only estimator is minimax optimal; when $\overline\Delta\lesssim \sigma_\rct/\sqrt{n_\rct}$, the naively-pooled estimator is minimax optimal.} 
    \label{fig: phase_transition}
\end{figure}
% \tye{The $\Delta$ in Figure 1 should be $\bar\Delta$.}

The above theorem, along with Theorem \ref{thm:oracle_estimator}, confirms the minimax optimality of the oracle estimator $\hat\beta_\orac$. These two theorems together also reveal a curious phase transition phenomenon depicted in Figure \ref{fig: phase_transition}: when $\overline\Delta \gtrsim \sigma_\rct/\sqrt{n_\rct}$, then the minimax rate becomes $\Theta(\sigma_\rct^2/n_\rct)$, and such a rate is achieved by the RCT-only estimator $\hat\beta_\rct$;
when $\overline\Delta \lesssim \sigma_\rct/\sqrt{n_\rct}$, then the minimax rate becomes $\Theta({\sigma_\rct^2 \sigma_\obs^2}/({n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2}) + \overline\Delta^2)$, and such a rate is achieved by the naively-pooled estimator $\hat\beta_\weight$.
A conceptually similar phase transition phenomenon has been identified in other statistical problems that involve multiple data sources \citep{chen2021theorem}.



\subsection{Adaptation via {Anchored} Thresholding}\label{subsec: adaptive_procedure}
In this section, we design a fully adaptive estimator that does not need prior knowledge of $\overline\Delta$, and we prove that this estimator achieves nearly the same performance as the oracle estimator $\hat\beta_{\orac}$, up to poly-log factors. 
% \tye{clarify? because one is about $\Delta$, one is about $\bar\Delta$.} \sxc{I modify the statement of the results, now all the results should only involve $\overline{\Delta}$. As we discussed earlier focusing on a specific value of $\Delta$ may lead to some weird consequences.} 

If we can estimate the bias $\Delta$ sufficiently well by some $\hat\Delta$, then we can ``de-bias'' the observational-data-only estimator by computing $\hat\beta_\obs + \hat\Delta$. Since the resulting estimator is approximately unbiased, we may aggregate $\hat\beta_\rct$ and $\hat\beta_\obs + \hat\Delta$ by forming
$
    (1 - \weight) \hat\beta_\rct + \weight (\hat \beta_\obs + \hat\Delta),
$
similar to our construction of the naively-pooled estimator in \eqref{eq:naive_estimator}.

There are two key issues in the above construction. First, since the variances are usually unknown in practice, we need to replace the weight $\omega$ by its estimated counterpart
$$
    \hat \weight = \frac{\hat \sigma_\rct^2/n_\rct}{\hat \sigma_\rct^2/n_\rct + \sigma_\obs^2/n_{\obs}},
$$
where $\hat\sigma_\rct, \hat\sigma_\obs$ are estimators of $\sigma_\rct, \sigma_\obs$, respectively. The other, and perhaps more important issue, lies in the choice of $\hat\Delta$. Since $\hat\beta_\rct$ and $\hat\beta_\obs$ are respectively asymptotically unbiased for $\beta^\star$ and $\beta_\obs$, a tempting choice of $\hat\Delta$ is
$$
    \tilde\Delta = \hat\beta_\rct - \hat\beta_\obs.
$$
However, a careful thought reveals that $\tilde\Delta$ is not sufficient for our purpose of obtaining a better estimator than $\hat\beta_\rct$: if we use $\hat\Delta = \tilde \Delta$, then we would get
$$
    (1-\weight) \hat\beta_\rct + \weight (\hat\beta_\obs + \tilde\Delta) = (1-\weight) \hat\beta_\rct + \weight \hat\beta_\rct = \hat\beta_\rct.
$$
In other words, the accuracy of $\tilde\Delta$ is not enough to provide any efficiency gain against the RCT-only estimator $\hat\beta_\rct$. Clearly, more work is needed.

% We start by constructing an preliminary estimator that pools all the data together:
% $$
%     \tilde \beta : =  (1-\hat\weight) \hat\beta_\rct + \hat\weight  \hat \beta_\obs, \qquad \hat \weight = \frac{\hat \sigma_\rct^2/n_\rct}{\hat \sigma_\rct^2/n_\rct + \sigma_\obs^2/n_{\obs_2}},
% $$
% where $\hat\sigma_\rct$ and $\hat\sigma_\obs$ are estimators of $\sigma_\rct$ and $\sigma_\obs$, respectively.
% Since $\beta_\obs \neq \beta^\star$, the above estimator is biased, and the magnitude of the bias is $\hat \weight |\Delta|$.
% We then try to de-bias $\tilde\beta$ by estimating $\Delta$. 
% A naive estimator is given by
% $$
%     \tilde \Delta = \hat \beta_\rct - \hat \beta_\obs.
% $$
% If we use the above estimator to de-bias $\tilde \beta$, the final estimator becomes $\hat\beta = \tilde \beta + \hat\weight\tilde\Delta = \hat\beta_\rct$, i.e., we get back to $\hat\beta_\rct$ and there is no efficiency gain. 

To proceed, we make two observations. First, we know that $\tilde \Delta$, after proper scaling, is asymptotically Gaussian as $n_\rct \land n_{\obs}\to\infty$, and the asymptotic mean and variance of $\tilde \Delta$ are given by $\Delta$ and ${\sigma_\rct^2}/{n_\rct} + {\sigma_\obs^2}/{n_{\obs}}$, respectively. A standard concentration of measure argument gives that $|\Delta - \tilde \Delta| \lesssim \lambda \sqrt{({\sigma_\rct^2}/{n_\rct} + {\sigma_\obs^2}/{n_{\obs}})}$ with probability tending to one, as long as $\lambda$ is a diverging sequence as $n_\rct\land n_{\obs}\to\infty$ \citep{boucheron2013concentration}.
Second, we know that the observational data 
are {useful only} when the bias $\Delta$ is small. These two observations motivate the following procedure:

\begin{equation}
    \label{eq:est_delta}
    \hat \Delta_\lambda = \argmin_{\delta} |\delta| \qquad \textnormal{subject to } |\delta - \tilde \Delta| \leq 
    \lambda \cdot 
    % \sfc \sqrt{\log (n_\rct\land n_{\obs_2})} \cdot
    \sqrt{\frac{\hat\sigma_\rct^2}{n_\rct} + \frac{\hat\sigma_\obs^2}{n_{\obs}}},
\end{equation} 
where $\lambda > 0$ is a hyperparameter. Intuitively, the above procedure {selects an estimator of the bias $\Delta$} with the minimum absolute value (based on our second observation), among all ``plausible'' candidates, where the ``plausibility'' is quantified by our first observation.

Such a procedure is reminiscent of many well-known methods in high-dimensional statistics, such as the Dantzig selector in sparse linear models \citep{candes2007dantzig} and nuclear norm minimization in matrix completion \citep{candes2009exact,candes2010power}, where one seeks for an estimator that minimizes certain complexity measures (in our case, the absolute value) subject to a constraint that ensures the error control.

Note that \eqref{eq:est_delta} can be solved via soft-thresholding: 
$$
    \hat \Delta_\lambda = 
    \begin{cases}
        \textnormal{sgn}(\tilde \Delta)\Big(|\tilde \Delta| - \lambda \cdot
        \sqrt{\frac{\hat\sigma_\rct^2}{n_\rct} + \frac{\hat\sigma_\obs^2}{n_{\obs}}}\Big)
        & \textnormal{if } 
        |\tilde \Delta| \geq \lambda \cdot
        \sqrt{\frac{\hat\sigma_\rct^2}{n_\rct} + \frac{\hat\sigma_\obs^2}{n_{\obs}}},\\
        0
        & \textnormal{otherwise}.
    \end{cases}
$$
Thus, one can alternatively view \eqref{eq:est_delta} as a LASSO-type estimator \citep{tibshirani1996regression} {as it searches for the $\delta$} that minimizes $|\tilde \Delta - \delta|^2 + \lambda' |\delta|$ for a particular choice of $\lambda'$.

Once $\hat\Delta_\lambda$ is obtained, the final estimator for $\beta^\star$ is given by 
\begin{equation*}
    % \label{eq:final_estimator}
    \hat \beta_\lambda = (1-\hat\weight) \hat\beta_\rct + \hat\weight (\hat\beta_\obs + \hat\Delta_\lambda).
\end{equation*}
{Because this estimator is anchored at the RCT-only estimator $\hat\beta_\rct$ and integrates a de-biased observational-data-only estimator obtained from soft-thresholding, we name $\hat\beta_\lambda$ the \emph{anchored thresholding} estimator.} 
% \sxc{We need to give a reason for calling the whole procedure as ``anchored thresholding'', or we just call it soft thresholding estimator / adaptive estimator}
The following theorem characterizes the performance of $\hat\beta_\lambda$.

\begin{theorem}[Performance of the Anchored Thresholding Estimator]
\label{thm:high_prob_bound_adaptive_estimator}
Let Assumption \ref{assump:asymp_linear} hold. In addition, assume $\sigma_\rct^2/n_\rct\gtrsim \sigma_\obs^2/n_{\obs}$
% $n_\obs \geq (1+\ep)n_\rct$ for some absolute constant $\ep > 0$, 
and $\hat\sigma_\rct \overset{p}{\to} \sigma_\rct, \hat\sigma_\obs \overset{p}{\to} \sigma_\obs$ as $n_\rct \land n_\obs \to \infty$. 
As long as we choose $\lambda \gtrsim 1$, there exists an absolute constant $\sfc > 0$ such that with probability at least $1- o(1) - e^{-\sfc \lambda^2}$, we have
\begin{equation*}
    % \label{eq:high_prob_bound_adaptive_estimator}
     |{\hat\beta_\lambda} - \beta^\star|^2 \lesssim  \lambda^2 \cdot \bigg(\frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} + \frac{\sigma_\rct^2}{n_\rct} \land \overline{\Delta}^2\bigg).
\end{equation*} 
\end{theorem}
\begin{proof}
    See Appendix \ref{prf:thm:high_prob_bound_adaptive_estimator}.
\end{proof}

By the above theorem, if we choose $\lambda \asymp \sqrt{\log (n_\rct\land n_{\obs})}$, then we conclude that with probability tending to one, the adaptive estimator $\hat\beta_\lambda$ achieves nearly the same performance as the oracle estimator, up to poly-log factors.
The $o(1)$ term in the high probability statement depends on the rate of convergence of $\hat\sigma_\rct$ and $\hat\sigma_\obs$, as well as the two $o_p(1)$ terms appeared in the asymptotic linear expansion of $\hat\beta_\rct$ and $\hat\beta_\obs$. 




% \subsubsection{Another adaptive procedure}
% % \sxc{This procedure}
% Let $\hat \Delta$ be the estimator obtained via anchored thresholding. Then we simply use
% $$
%     \hat \beta_{\hat \weight}, \qquad \hat\weight = \frac{\sigma_\rct^2/n_\rct}{\sigma_\rct^2/n_\rct + \sigma_\obs^2/n_{\obs_2} + \hat\Delta^2}.
% $$
% Namely we replace the $\Delta$ in $\weight^\star$ by $\hat \Delta$. Then one can show that Theorem \ref{thm:high_prob_bound_adaptive_estimator} also holds for $\hat \beta_{\hat\weight}$. \sxc{check empirically}

% Of course, we know that $\hat\beta_{\tilde \weight}$, where $\tilde \weight = \frac{\sigma_\rct^2/n_\rct}{\sigma_\rct^2/n_\rct + \sigma_\obs^2/n_{\obs_2} + \tilde\Delta^2}$, $\tilde \Delta = \hat\beta_\rct - \hat\beta_\obs$ is not enough. This is easy to demonstrate empirically. It seems that we can show something like: if $\Delta = 0$, with constant probability, the error of $\hat \beta_{\tilde \weight}$ is at least $\sigma_\rct/\sqrt{n_\rct}$.

% The construction of confidence interval is easy if we are allowed to do sample splitting. 
% We use the first half of RCT data and the first half of OBS data to get $\hat \weight$.
% We then use the second half of RCT data and the second half of OBS data to get $\hat\beta_{\hat\weight}$. Note that $\hat\weight$ is independent of the second half of RCT data and the second half of OBS data. Thus, conditional on the randomness of $\hat\weight$, the sample split estimator $\hat\beta_{\hat \weight}$ is asymptotically normal. This gives a valid CI for every realization of $\hat\weight$, and thus is a valid CI if we marginalize over the randomness of $\hat\weight$. \sxc{What parameter is it covering?}
% One thing that I am not sure is whether the length of the CI indeed has the correct scaling on $\Delta$. Maybe it is possible to cook up something like: with high probability, the length of this CI is upper bounded by xxx...

% Note that the same strategy for CI construction can be applied to our previous adaptive estimator. There, we let $\hat\weight = \frac{\sigma_\rct^2/n_\rct}{\sigma_\rct^2/n_\rct + \sigma_\obs^2/n_{\obs_2}}$. We estimate $\hat\Delta$ from the first half of the data. Then construct $\tilde \beta = (1-\hat\weight)\hat\beta_\rct + \hat\weight \hat\beta_\obs$ using the second half of the data. The final estimator $\hat\beta = \tilde \beta + \hat\weight\hat \Delta$. Conditional on $\hat \Delta$, the distribution of $\hat\beta$ is asymptotically normal.


\section{Statistical Inference}\label{sec:inference}

\subsection{Minimax Rate for the Length of Confidence Intervals}
Under Assumption \ref{assump:asymp_linear}, we can always construct a valid CI for $\beta^\star$ using the RCT-only estimator $\hat\beta_\rct$, and its length is of order $\sigma_\rct/\sqrt{n_\rct}$.
If $n_\obs \gg n_\rct$, is it possible to construct a CI that is \emph{order-wise} better than the naive construction?
% If so, is it possible to do so without the knowledge of $\Delta$ or $\overline\Delta$?
To answer this question in a rigorous fashion, we adopt the minimax framework pioneered by \cite{cai2004adaptation} and \cite{cai2017confidence}. 
We again use Model \ref{model} as our working model to benchmark the information-theoretic limit of CI construction.

Recall the parameter $\calP_{\overline\Delta}$ specified in \eqref{eq:param_space}. Let $\calI_\alpha(\calP_{\overline{\Delta}})$ be the set of all level $(1-\alpha)$ CIs that are uniformly valid over $\calP_{\overline{\Delta}}$:
$$
    \calI_\alpha(\calP_{\overline\Delta}) = \bigg\{[L(\calD_\Rct, \calD_\Obs)), U(\calD_\Rct, \calD_\Obs) ]: \bbP_{(\beta^\star, \beta_\obs)}(L \leq \beta^\star \leq  U)\geq 1-\alpha , \forall (\beta^\star, \beta_\obs) \in \calP_{\overline{\Delta}}\bigg\}.
$$
In the above display, $L$ and $U$ are two measurable functions of both the RCT data $\calD_\Rct$ and the observational data $\calD_\Obs$.
For any $\ci_\alpha = [L, U]\in \calI_\alpha(\calP_{\overline\Delta})$, its length is 
$
    \len(\ci_\alpha) = U - L.
$
The \emph{minimax length} of CIs over $\calP_{\overline\Delta}$ is defined as
$$
    \len_\alpha^\star(\calP_{\overline\Delta}) = \inf_{\ci_\alpha\in \calI_\alpha(\calP_{\overline\Delta})} \sup_{(\beta^\star, \beta_\obs)\in\calP_{\overline\Delta}} \bbE[\len(\ci_\alpha)].
$$
Analogous to the notion of minimax rate {for the mean squared error}, the minimax length captures the worst-case performance of CI construction over a pre-specified parameter space.

The following theorem characterizes the rate of convergence for the minimax length.
\begin{theorem}[{Minimax Rate of CI Length}]
\label{thm:minimax_length}
Under Model \ref{model}, we have
\begin{equation}
    \label{eq:minimax_length}
    \len_\alpha^\star(\calP_{\overline\Delta}) \gtrsim 
    \frac{\sigma_\rct\sigma_\obs}{\sqrt{n_\rct\sigma_\obs^2 + n_\obs\sigma_\rct^2}} + \frac{\sigma_\rct}{\sqrt{n_\rct}} \land \overline\Delta,
\end{equation} 
provided $\alpha \leq \Phi(-1/4)-\ep$ for some absolute constant $\ep\in(0, \Phi(-1/4))$.
\end{theorem}
\begin{proof}
    This is a special case of Theorem \ref{thm:minimax_adaptive_length} proved in Appendix \ref{prf:thm:minimax_adaptive_length}.
\end{proof}

The above result should not come as a surprise, as the right-hand side of \eqref{eq:minimax_length} is precisely the square-root of the minimax rate for the mean squared error given in Theorems \ref{thm:oracle_estimator} and \ref{thm:lb}.

Similar to the oracle estimator introduced in \eqref{eq:oracle_estimator}, we can construct an oracle CI that achieves the above lower bound. In particular, we define 
\begin{align}
    \label{eq:oracle_ci_L}
    L_\alpha & = 
    \begin{cases}
        \hat\beta_\rct - \Phi^{-1}(1-\frac{\alpha}{2}) \cdot \frac{\sigma_\rct}{\sqrt{n_\rct}}
        & \textnormal{ if } \overline\Delta \geq \sigma_\rct/\sqrt{n_\rct}\\
        \hat\beta_\weight - \Phi^{-1}(1-\frac{\alpha}{2})\cdot \frac{\sigma_\rct\sigma_\obs}{\sqrt{n_\rct\sigma_\obs^2 + n_{\obs}\sigma_\rct^2}} -\overline\Delta
        & \textnormal{ otherwise},
    \end{cases}\\
    \label{eq:oracle_ci_U}
    U_\alpha & = 
    \begin{cases}
        \hat\beta_\rct + \Phi^{-1}(1-\frac{\alpha}{2}) \cdot \frac{\sigma_\rct}{\sqrt{n_\rct}}
        & \textnormal{ if } \overline\Delta \geq \sigma_\rct/\sqrt{n_\rct}\\
        \hat\beta_\weight + \Phi^{-1}(1-\frac{\alpha}{2})\cdot \frac{\sigma_\rct\sigma_\obs}{\sqrt{n_\rct\sigma_\obs^2 + n_{\obs}\sigma_\rct^2}} + \overline\Delta
        & \textnormal{ otherwise}.
    \end{cases}
\end{align}
That is, when $\overline\Delta \geq \sigma_\rct/\sqrt{n_\rct}$, we construct the CI based on the RCT-only estimator $\hat\beta_\rct$, whereas when $\overline\Delta < \sigma_\rct/\sqrt{n_\rct}$, we first construct the CI based on the naively-pooled estimator and then enlarge it by $\overline\Delta$. The properties of this CI are given below.

\begin{theorem}[Oracle CI]
\label{thm:oracle_ci}
Consider the CI defined in \eqref{eq:oracle_ci_L} and \eqref{eq:oracle_ci_U}.
Under Assumption \ref{assump:asymp_linear}, for any $\alpha\in(0, 1)$, we have
$$
    \bbP(\beta^\star \in [L_\alpha, U_\alpha]) \geq 1-\alpha - o(1)
$$
as $n_\rct \land n_{\obs}\to \infty$. 
If 
% $n_\obs \geq (1+\ep)n_\rct$ and 
$\alpha \geq \ep$ for some absolute constant $\ep\in(0, 1)$, then 
$$
\bbE[\len([L_\alpha, U_\alpha])]\lesssim \frac{\sigma_\rct\sigma_\obs}{\sqrt{n_\rct\sigma_\obs^2 + n_\obs\sigma_\rct^2}} + \frac{\sigma_\rct}{\sqrt{n_\rct}} \land \overline\Delta.
$$
\end{theorem}
\begin{proof}
    See Appendix \ref{prf:thm:oracle_ci}. 
\end{proof}

Combining \textcolor{black}{Theorems \ref{thm:minimax_length} and \ref{thm:oracle_ci}}, we conclude that when $\overline\Delta$ is known, it is indeed possible to construct a CI that is strictly better than the naive one based on the RCT-only estimator, and such an oracle CI is minimax optimal in terms of its expected length.








\subsection{When Is Adaptation Possible?}
Up to now, the results regarding inference is nearly identical to the results regarding estimation: as long as $\overline\Delta$ is known, we have an oracle procedure that attains the minimax lower bound. However, we are to see that the story for adaptation is drastically different. Without prior knowledge of $\overline\Delta$, it is in general not possible to construct a CI that achieves comparable performance as the oracle CI.

To formalize the above claim, let us introduce another parameter $\underline\Delta \leq \overline\Delta$ and consider a smaller parameter space
$$
    \calP_{\underline\Delta} = \{(\beta^\star, \beta_\obs): |\beta^\star - \beta_\obs|\leq \underline\Delta\} \subseteq \calP_{\overline\Delta}.
$$
We then define
$$
    \len_\alpha^\star(\calP_{\underline\Delta}, \calP_{\overline\Delta}) = 
    \inf_{\ci_\alpha\in \calI_\alpha(\calP_{\overline\Delta})} \sup_{(\beta^\star, \beta_\obs)\in\calP_{\underline\Delta}} \bbE_{(\beta^\star, \beta_\obs)} [\len(\ci_\alpha)],
$$
i.e., the minimax CI length over the smaller parameter space $\calP_{\underline\Delta}$ when we require the CI to be \emph{uniformly valid} over the larger parameter space $\calP_{\overline\Delta}$.
The above quantity measures the difficulty of adaptation to unknown $\underline\Delta$. 
For example, if 
% Adaptation from $\calP_{\overline\Delta}$ to $\calP_{\underline\Delta}$ is said to be possible if
$$
    \len_\alpha^\star(\calP_{\underline\Delta}, \calP_{\overline\Delta}) \asymp \len_\alpha^\star(\calP_{\underline\Delta}, \calP_{\underline\Delta}) = \len_\alpha^\star(\calP_{\underline\Delta}),
$$
then it tells that even if we require uniform coverage over the larger parameter space $\calP_{\overline{\Delta}}$, we can still construct a CI whose minimax length is of the same order as if we only require coverage over the smaller parameter space $\calP_{\underline{\Delta}}$.
In this case, we conclude that adaptation is possible.
On the contrary, if
$$
    \len_\alpha^\star(\calP_{\underline\Delta}, \calP_{\overline\Delta}) \gg  \len_\alpha^\star(\calP_{\underline\Delta}),
$$
then we know that requiring uniform coverage over $\calP_{\overline\Delta}$ would result in a much wider CI, and hence adaptation is impossible.

The following theorem gives a lower bound of $\len_\alpha^\star(\calP_{\underline\Delta}, \calP_{\overline\Delta})$.
\begin{theorem}[Minimax Length of Adaptive CIs]
\label{thm:minimax_adaptive_length}
Under Model \ref{model}, for any $\underline\Delta\leq \overline\Delta$, we have
\begin{equation}
    \label{eq:minimax_adaptive_length}
    \len_\alpha^\star(\calP_{\underline\Delta}, \calP_{\overline\Delta}) \gtrsim 
    \frac{\sigma_\rct\sigma_\obs}{\sqrt{n_\rct\sigma_\obs^2 + n_\obs\sigma_\rct^2}} + \frac{\sigma_\rct}{\sqrt{n_\rct}} \land \overline\Delta,
\end{equation} 
provided $\alpha \leq \Phi(-1/4)-\ep$ for some absolute constant $\ep\in(0, \Phi(-1/4))$.
\end{theorem}
\begin{proof}
    See Appendix \ref{prf:thm:minimax_adaptive_length}.
\end{proof}

Note that the lower bound in \eqref{eq:minimax_adaptive_length} has no dependence on $\underline\Delta$. Combining the above result with Theorems \ref{thm:minimax_length} and \ref{thm:oracle_ci}, we conclude that adaptation is in general not possible. As a concrete example, suppose that 
$$
    \frac{\sigma_\rct\sigma_\obs}{\sqrt{n_\rct\sigma_\obs^2 + n_\obs\sigma_\rct^2}} \lesssim \underline\Delta \ll \overline\Delta \lesssim \frac{\sigma_\rct}{\sqrt{n_\rct}},
$$
under which case we have
$$
    \len_\alpha^\star(\calP_{\underline\Delta}, \calP_{\overline\Delta}) \gtrsim \overline\Delta \gg \underline\Delta \asymp 
     \len_\alpha^\star(\calP_{\underline\Delta}).
$$
Moreover, the gap for adaptation, measured by the ratio between $\overline\Delta$ and $\underline\Delta$, can be as large as $\sqrt{n_\obs/n_\rct}$.

There are certain cases where adaptation is possible. For example, if we have prior knowledge that 
$
    \overline\Delta \lesssim {\sigma_\rct\sigma_\obs}/{\sqrt{n_\rct\sigma_\obs^2 + n_\obs\sigma_\rct^2}},
$
then the lower bound \eqref{eq:minimax_adaptive_length} becomes ${\sigma_\rct\sigma_\obs}/{\sqrt{n_\rct\sigma_\obs^2 + n_\obs\sigma_\rct^2}}$. Such a length can be achieved by constructing a CI based on the naively-pooled estimator and enlarging it by a constant multiple of ${\sigma_\rct\sigma_\obs}/{\sqrt{n_\rct\sigma_\obs^2 + n_\obs\sigma_\rct^2}}$. As another example, if $\overline\Delta\gtrsim \sigma_\rct/\sqrt{n_\rct}$, then the lower bound \eqref{eq:minimax_adaptive_length} reads $\sigma_\rct/\sqrt{n_\rct}$, and such a length is achieved by the CI based on the RCT-only estimator.

In view of Theorem \ref{thm:minimax_adaptive_length}, in practice, if we do not have strong prior knowledge that $\overline\Delta\ll \sigma_\rct/\sqrt{n_\rct}$, then the CI based on the RCT-only estimator is optimal from a worst-case point of view.







==> combining clinical and observational datasets/04-simulation.tex <==
%!TEX root = 00-main.tex

\section{Simulation Studies}
% \label{sec: simulation}
We consider the following data-generating process in the population:
\begin{equation} \label{eq: simu population}
% \begin{split}
    X_1, X_2, X_3 \sim N(0, 1);\qquad 
    Y(0) = X_1 + X_2 + X_3 + \epsilon,~Y(1) = Y(0) + \beta(X_1, X_2, X_3),
% \end{split}
\end{equation}
where $\epsilon \sim N(0, 1)$. The first factor in the simulation design concerns about the effect heterogeneity:
\begin{description}
\item[Factor 1:] Treatment effect heterogeneity: a constant treatment effect $\beta(X_1, X_2, X_3) = 2$ and a heterogeneous treatment effect $\beta(X_1, X_2, X_3) = 2 - X_1 - X_2$. In either case, the PATE $\beta^\star = 2.$
\end{description}
We consider the following selection model into an RCT:
\begin{equation*}
\text{logit}\{\bbP(S = c \mid X_1, X_2, X_3)\} = -7 + X_1 - X_2.
\end{equation*}
According to this sample selection model, the marginal probability $P(S = c) \approx 0.25\%$. We simulate a population of $100,000$ so that $n_c \approx 250$ in each simulated RCT dataset. For each simulated RCT sample, we assign treatment $A$ randomly with probability $\pi_c = 1/2$ and $Y = A\cdot Y(1) + (1-A)\cdot Y(0)$. Note that the interplay between selection heterogeneity and treatment effect heterogeneity induces an external validity bias when $\beta(X_1, X_2, X_3) = 2 - X_1 + X_2$.

In parallel, we simulate an observational dataset with sample size $n_{\text{o}}$. Covariates and potential outcomes are simulated under \eqref{eq: simu population}. We assign treatment $A$ according to  $A \sim \text{Bern}(\text{expit}\{1 - X_1 - b \cdot X_3\})$, and $Y = A\cdot Y(1) + (1-A)\cdot Y(0)$. 
We consider a scenario where $X_3$ is an unmeasured confounder and hence the observed observational data $\mathcal{D}_o$ consist only of $\{X_1, X_2, A, Y\}$. This induces an internal validity bias when $b \neq 0$. The second and third factors are concerned about the observational data generating process. 

\begin{description}
\item[Factor 2:] Observational data sample size $n_o = 10,000$, $50,000$, and $100,000$.
\item[Factor 3:] Magnitude of internal validity bias controlled by $b$: (i) small or no bias $b = 0, 0.01, 0.1$, (ii) moderate bias $b = 0.5, 0.6, 0.7$, and (iii) large bias $b = 2, 3, 10$.
\end{description}

For each simulated pair of RCT and observational data, we construct an RCT-based estimator $\hat\beta_c$, an observational-data-based estimator $\hat\beta_o$,  an oracle estimator $\hat\beta_\orac$ that uses the oracle bias $\Delta$, and a family of adaptive estimators $\hat\beta_{\lambda}$ parameterized by $\lambda$. 
For a constant treatment effect $\beta(X_1, X_2, X_3) = 2$, we consider $(\hat\beta_c, \hat\beta_o) = (\hat\beta_{c, \textsf{IPW}}, \hat\beta_{o, \textsf{IPW}})$, $(\hat\beta_c, \hat\beta_o) = (\hat\beta_{c, \textsf{AIPW}}, \hat\beta_{o, \textsf{AIPW}})$, and we set $\lambda = \lambda_1 \cdot \sqrt{\log (n_\rct\land n_{\obs})}$ for some constant $\lambda_1$.  
For the heterogeneous treatment effect $\beta(X_1, X_2, X_3) = 2 - X_1 - X_2$, we consider $(\hat\beta_c, \hat\beta_o) = (\hat\beta_{c, \textsf{IPPW}}, \hat\beta_{o_2, \textsf{IPW}})$ and $(\hat\beta_c, \hat\beta_{o}) = (\hat\beta_{c, \textsf{AIPPW}}, \hat\beta_{o_2, \textsf{AIPW}})$. 
When constructing the $\hat\beta_{c, \textsf{IPPW}}$ and $\hat\beta_{c, \textsf{AIPPW}}$, we estimate the participation probability using RCT data and a random subsample of size $n_c$ from the observational data, and we set $\lambda = \lambda_1 \cdot \sqrt{\log (n_\rct\land n_{\obs_2})}$ for some constant $\lambda_1$. 



\begin{table}[t]
\centering
\caption{Ratios of the mean squared error of each estimator to that of the oracle estimator $\hat{\beta}_\weight$ when $n_o = 10000$. Estimators considered in the table are the RCT-based estimator $\hat{\beta}_c$, the observational-data-based estimator $\hat{\beta}_o$, and the anchored thresholding estimator $\hat{\beta}_{\lambda}$. 
% with $\lambda = \lambda_1 \cdot \sqrt{\log(n_c \land n_{o_2})}$.
}
\label{tbl: simulation results}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccccc}
 &$\hat\beta_c$ & $\hat\beta_o$ &\multicolumn{2}{c}{$\hat\beta_{\lambda}$} & $\hat\beta_c$ & $\hat\beta_o$ &\multicolumn{2}{c}{$\hat\beta_{\lambda}$}\\
    \hline
    \hline
   % \\
   \multicolumn{9}{c}{$\beta(X_1, X_2, X_3) = 2$} \\
    \hline
 \multirow{2}{*}{\begin{tabular}{c}b\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{IPW}\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{IPW}\end{tabular}} 
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.5$\end{tabular}}
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.6$\end{tabular}}
    &\multirow{2}{*}{\begin{tabular}{c}\textsf{AIPW}\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{AIPW}\end{tabular}} 
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.5$\end{tabular}}
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.6$\end{tabular}}
  \\  \\
  
  0.00 & 29.03 & 1.03 & 3.61 & 2.14  & 23.11 & 1.06 & 3.05 & 1.89 \\ 
  0.01 & 28.23 & 1.06 & 4.25 & 2.72  & 23.60 & 1.06 & 3.53 & 2.23 \\ 
  0.10 & 8.85 & 1.07 & 1.73 & 1.34  & 6.62 & 1.09 & 1.50 & 1.25 \\ 
  %0.30 & 1.33 & 1.09 & 0.84 & 0.87  & 1.01 & 1.15 & 0.81 & 0.86 \\ 
  %0.40 & 1.00 & 1.41 & 0.93 & 1.03  & 1.00 & 1.87 & 1.13 & 1.29 \\ 
  0.50 & 1.00 & 1.98 & 1.18 & 1.33  & 1.00 & 2.84 & 1.48 & 1.74 \\ 
  0.60 & 1.00 & 2.91 & 1.51 & 1.76  & 1.00 & 3.88 & 1.72 & 2.07 \\ 
  0.70 & 1.00 & 3.74 & 1.71 & 2.06  & 1.00 & 5.30 & 1.95 & 2.44 \\ 
  2.00 & 1.00 & 12.87 & 2.32 & 3.05  & 1.00 & 18.13 & 2.40 & 3.17 \\ 
  3.00 & 1.00 & 17.72 & 2.21 & 2.98  & 1.00 & 23.54 & 2.20 & 2.93 \\ 
  10.00 & 1.00 & 20.87 & 2.26 & 3.01 & 1.00 & 29.93 & 2.28 & 3.04 \\  
  % \\
    \hline
    \hline
   \multicolumn{9}{c}{$\beta(X_1, X_2, X_3) = 2 - X_1 - X_2$} \\
    \hline

\multirow{2}{*}{\begin{tabular}{c}b\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{IPPW}\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{IPW}\end{tabular}} 
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.5$\end{tabular}}
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.6$\end{tabular}}
    &\multirow{2}{*}{\begin{tabular}{c}\textsf{AIPPW}\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{AIPW}\end{tabular}} 
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.5$\end{tabular}}
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.6$\end{tabular}}
  \\  \\  
  0.00 & 28.81 & 1.04 & 3.61 & 2.23 & 25.26 & 1.05 & 3.25 & 2.04 \\ 
   0.01 & 31.66 & 1.05 & 4.51 & 2.73 & 27.70 & 1.05 & 3.94 & 2.43 \\ 
   0.10 & 8.91 & 1.06 & 1.73 & 1.33 & 7.34 & 1.07 & 1.69 & 1.35 \\ 
   %0.30 & 1.42 & 1.09 & 0.87 & 0.90 & 1.05 & 1.06 & 0.78 & 0.82 \\ 
   %0.40 & 0.99 & 1.38 & 0.94 & 1.03 & 1.00 & 1.85 & 1.11 & 1.26 \\ 
   0.50 & 1.00 & 1.91 & 1.17 & 1.32 & 1.00 & 2.63 & 1.39 & 1.60 \\ 
   0.60 & 1.00 & 2.81 & 1.41 & 1.66 & 1.00 & 3.67 & 1.58 & 1.91 \\ 
   0.70 & 1.00 & 3.76 & 1.66 & 2.02 & 1.00 & 4.87 & 1.80 & 2.24 \\ 
   2.00 & 1.00 & 13.07 & 2.22 & 2.94 & 1.00 & 18.44 & 2.21 & 2.93 \\ 
   3.00 & 1.00 & 18.60 & 2.42 & 3.25 & 1.00 & 26.37 & 2.44 & 3.29 \\ 
   10.00 & 1.00 & 23.45 & 2.49 & 3.36 & 1.00 & 30.90 & 2.35 & 3.14 \\ \hline
\end{tabular}}
\end{table}


Table \ref{tbl: simulation results} summarizes the simulation results when $n_o = 10,000$. Results for $n_o = 50,000$ and $n_o = 100,000$ are similar and can be found in Appendix \ref{appx:more_simulation}. Under each data-generating process, we calculated the mean squared error of each estimator, including the oracle estimator $\hat\beta_{\orac}$, the RCT-based estimator $\hat\beta_c$, the observational-data-based estimator $\hat\beta_o$, and a collection of adaptive estimators $\hat\beta_{\lambda}$ with different choices of $\lambda_1$, and reported the MSE of each estimator as a multiple of that of the oracle estimator. The simulation results aligned well with theory and intuition. When $b$ and hence the level of unmeasured confounding is small, the RCT-based estimator $\hat\beta_c$ performs much poorly compared to the oracle estimator. For instance, when $\beta(X_1, X_2, X_3) = 2$ and $b = 0.01$, $\hat\beta_c$ has a mean squared error as large as $28$ times of that of $\hat\beta_\orac$ when $\hat\beta_c$ is constructed via inverse probability weighting and a mean squared error as large as $23$ times of that of $\hat\beta_\orac$ when constructed via augmented inverse probability weighting. At the other end of the spectrum, the observational-data-based estimator $\hat\beta_o$ performs poorly when there is a large degree of unmeasured confounding. On the other hand, the adaptive estimator $\hat\beta_{\lambda}$ has rather consistent performance across the spectrum of the level of unmeasured confounding, with a mean squared error within a small multiple of that of the oracle estimator. These patterns remain true when the treatment effect is homogeneous or heterogeneous, and when $\hat\beta_c$ and $\hat\beta_o$ are constructed in different ways.

% \textcolor{red}{I need to re-do the figure.}

%Finally, Figure \ref{fig: simu} plots the distribution of the RCT-based estimator $\hat{\beta}_c$, the observational-data-based estimator $\hat{\beta}_o$, and the proposed adaptive estimator $\hat{\beta}_{\lambda}$. In Figure \ref{fig: simu}, the distribution of $\hat{\beta}_\rct$ is centered at $\beta^\star = 2$ but spreads widely, whereas the distribution of $\hat{\beta}_\obs$ is concentrated at the wrong place. The adaptive estimator sacrifices a little on the unbiasedness but gains a lot in reducing the variance. Moreover, $\hat\beta_{\lambda}$ automatically adapts to the unknown discrepancy between $\hat{\beta}_c$ and  $\hat{\beta}_o$, becoming more similar to $\hat\beta_\obs$ when the bias is small (Figure \ref{fig: simu}(a)) and more similar to $\hat\beta_\rct$ when the bias is large (Figure \ref{fig: simu}(b)).




%\begin{figure}[t]
%    \centering
%    \subfloat[$b = 0.3$]{\includegraphics[width = 0.49\textwidth]{const_0_3.pdf}}
%     \subfloat[$b = 0.5$]{\includegraphics[width = 0.49\textwidth]{const_0_5.pdf}}
%    \caption{Distribution of the RCT-based estimator, observational-data-based estimator, and the proposed adaptive estimator. \tye{Specify the simulation settings.}}
%    \label{fig: simu}
%\end{figure}

==> combining clinical and observational datasets/06-real_data.tex <==
%!TEX root = 00-main.tex


\section{Real Data Example: the  RCT DUPLICATE Initiative}

\begin{table}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccc}
       \multirow{4}{*}{\begin{tabular}{c}\textbf{Study Name}\end{tabular}}   & \multirow{4}{*}{\begin{tabular}{c}\textbf{Outcome}\end{tabular}}  & 
       \multirow{4}{*}{\begin{tabular}{c}\textbf{RCT} \\\textbf{Sample}\\\textbf{Size}\end{tabular}}  & 
       \multirow{4}{*}{\begin{tabular}{c}\textbf{RCT} \\\textbf{Estimate}\end{tabular}}  & 
       \multirow{4}{*}{\begin{tabular}{c}\textbf{OBS} \\\textbf{Sample}\\\textbf{Size}\end{tabular}}  & 
       \multirow{4}{*}{\begin{tabular}{c}\textbf{OBS} \\\textbf{Estimate}\end{tabular}}  & 
       \multirow{4}{*}{\begin{tabular}{c}\textbf{Anchored} \\\textbf{Thresholding} \\\textbf{Estimate}\end{tabular}} 
       \\ \\ \\ \\
       \hline
       \multirow{2}{*}{\begin{tabular}{c}\textsf{LEADER} \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}3P MACE \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}9,340 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0183\\ (0.0072) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}168,692 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0071 \\ (0.0007) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}-0.0075 \end{tabular}} \\ \\
       
        \multirow{2}{*}{\begin{tabular}{c}\textsf{DECLARE-TIMI 58} \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}HHF + death \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}17,160 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0092\\ (0.0034) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}49,790 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0050 \\(0.0010) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}-0.0053 \end{tabular}} \\ \\
        
        \multirow{2}{*}{\begin{tabular}{c} \textsf{EMPA-REG OUTCOME} \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}3P MACE \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}7,020 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0163\\ (0.0081) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}103,750 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0012\\ (0.0006) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}-0.0043 \end{tabular}} \\ \\
        
           \multirow{2}{*}{\begin{tabular}{c} \textsf{CANVAS} \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}3P MACE \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}10,142 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0168 \\ (0.0062) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}152,198 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0029\\ (0.0005) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}-0.0074 \end{tabular}} \\ \\
           
      \multirow{2}{*}{\begin{tabular}{c} \textsf{CARMELINA} \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}3P MACE \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}6,979 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}0.0037\\ (0.0078) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}101,826 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0056\\ (0.0011) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}-0.0054 \end{tabular}} \\ \\
      
         \multirow{2}{*}{\begin{tabular}{c} \textsf{TECOS} \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}3P MACE + angina \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}14,523 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0015\\ (0.0053) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}349,478 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0091 \\ (0.0007) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}-0.0089 \end{tabular}} \\ \\
       
       
       \multirow{2}{*}{\begin{tabular}{c} \textsf{SAVOR-TIMI 53} \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}3P MACE \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}16,492 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0001\\ (0.0041) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}182,128 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0080 \\ (0.0007) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}-0.0064 \end{tabular}} \\ \\
       
       \multirow{2}{*}{\begin{tabular}{c} \textsf{CAROLINA} \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}3P MACE \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}6,033 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0025\\ (0.0083) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}48,262 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0035\\ (0.0012) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}-0.0035 \end{tabular}} \\ \\
       
        \multirow{2}{*}{\begin{tabular}{c} \textsf{TRITON-TIMI 38} \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}3P MACE \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}13,608 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0206\\ (0.0052) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}43,864 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0110\\ (0.0018) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}-0.0129 \end{tabular}} \\ \\
        
        
         \multirow{2}{*}{\begin{tabular}{c} \textsf{PLATO} \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}3P MACE \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}18,624 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0166\\ (0.0044) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}27,960 \end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}-0.0149\\ (0.0027) \end{tabular}}  & \multirow{2}{*}{\begin{tabular}{c}-0.0154 \end{tabular}} \\ \\
       
    \end{tabular}}
    \caption{Results from 10 RCTs and their corresponding emulation studies. 3P MACE indicates 3-point major adverse cardiovascular events (myocardial infarction, stroke, or cardiovascular death). }
    \label{tab: real data summary table}
\end{table}
To assess whether non-randomized, observational claims data could provide accurate causal estimates of medical products, \cite{franklin2020nonrandomized, Franklin:2021aa} launched the RCT DUPLICATE initiative (Randomized, Controlled Trials Duplicated Using Prospective Longitudinal Insurance Claims: Applying Techniques of Epidemiology) where findings from a selected cohort of RCTs are compared to findings from observational health care claims data investigating the same clinical questions. Specifically, \cite{Franklin:2021aa} emulated the study design of $8$ cardiovascular outcome trials of antidiabetic medications and $2$ trials of antiplatelets using observational claims data by selecting the same primary outcome, treatment strategy, and applying the same inclusion and exclusion criteria so that the RCT cohort and observational cohort are similar in observed covariates. To estimate the effect of intervention from observational claims data, \cite{Franklin:2021aa} used $1$-to-$1$ propensity-score matching (\citealp{rosenbaum1983central,rosenbaum1985constructing}) and embedded observational data into an approximate randomized controlled trial. Just like any covariate adjustment methodology, statistical matching can only remove the overt bias but not the hidden bias due to unmeasured confounding; therefore, the effect estimate based on the observational data could be potentially biased. Using published summary data in \cite{Franklin:2021aa}, we calculated the effect of each intervention on event rate (defined as the rate that a pre-specified composite outcome, e.g., 3-point major adverse cardiovascular events, occurs) in each of the $10$ RCTs and their corresponding matched observational studies. Table \ref{tab: real data summary table} summarizes the results from 10 RCTs and their corresponding observational study emulations. Overall, we observe that the observational-data-based estimator and the RCT-based estimator align reasonably well. We then applied the adaptive procedure to pool together the RCT-based and observational-data-based estimates. We set the hyper-parameter $\lambda_1 = 0.5$ as guided by our simulation studies. The anchored thresholding estimates agreed with the RCT-only estimates in sign in all but the CARMELINA trial, and fell within the $95\%$ confidence interval of the RCT-only estimates in all $10$ trials. As demonstrated by our extensive simulations, the anchored thresholding estimates are expected to have near optimal mean square errors regardless of the magnitude of hidden bias in observational study emulations.


==> combining clinical and observational datasets/appx.tex <==
%!TEX root = 00-main.tex


\section{Additional Details}


\subsection{Bias Analysis of the Observational-Data-Only Estimators}\label{appx:internal_bias}
 To understand how the internal validity bias arises from unobserved confounding, we consider an unmeasured confounder $U$ such that the treatment assignment becomes ignorable once conditional on $(\mathbf{X}, U)$ \citep{rosenbaum1983sens,rosenbaum1983central, Imbens2003}, i.e., $ A  \indep ( Y(1), Y(0)) \mid \mathbf{X}, U, S=o$ but $ A \nindep ( Y(1), Y(0)) \mid \mathbf{X}, S=o$. Hence,
 \begin{align*}
\beta_o^\star&= \bbE( Y {(1)}  \mid S=o ) -  \bbE( Y {(0)}  \mid S=o ) \\
	&= \bbE\left[ \frac{A Y }{\pi_o(\bfX, U)} \mid S= o \right]  - \bbE\left[ \frac{(1-A) Y}{1-\pi_o(\bfX, U) } \mid S= o \right] \\
	&=   \bbE\left[ \frac{AY}{\pi_o(\bfX)  } \left\{ \frac{1-\pi_o(\bfX)}{\gamma (\bfX, U)}  + \pi_o(\bfX)  \right\}  \mid S= o \right]  \\
	&\qquad - \bbE\left[ \frac{(1-A) Y}{1-\pi_o(\bfX)} \left\{ \pi_o(\bfX)\gamma(\bfX, U)  + 1-\pi_o(\bfX) \right\}  \mid S= o \right],     
\end{align*}
where $\gamma(\mathbf{X}, U) = \text{OR}(\pi_{o}(\mathbf{X}, U), \pi_{o}(\mathbf{X}))$ is the odds ratio of the true propensity score $\pi_{o}(\mathbf{X}, U) = P(A= 1 \mid \mathbf{X}, U, S = o)$ that takes into account the unmeasured confounder $U$ and the observed propensity score $\pi_{o}(\mathbf{X}) = \bbP(A = 1 \mid \mathbf{X}, S = o)$.
Given that
\begin{align*}
    \beta_o= \bbE\left[ \frac{A Y }{\pi_o(\bfX)} \mid S= o \right]  - \bbE\left[ \frac{(1-A) Y}{1-\pi_o(\bfX) } \mid S= o \right],
\end{align*}
one can readily check that the difference $\Delta = \beta^\star - \beta_\obs =  \beta_o^\star - \beta_o$ takes the following form:
\begin{align*}
% \begin{split}
  \Delta & =  \mathbb{E}\left[ \frac{(1-A) Y\pi_{o}(\mathbf{X})}{1-\pi_{o}(\mathbf{X})} \left\{  1-\gamma(\mathbf{X}, U)  \right\}  \mid S= o \right]\\
  % \label{eqn: Obs data internal validity bias}
  & \qquad - \mathbb{E}\left[ \frac{AY(1-\pi_{o}(\mathbf{X}))}{\pi_{o}(\mathbf{X})  } \left\{   1- \frac{1}{\gamma (\mathbf{X}, U)}  \right\}  \mid S= o \right].
% \end{split}
\end{align*}
% where $\gamma(\mathbf{X}, U) = \text{OR}(\pi_{o}(\mathbf{X}, U), \pi_{o}(\mathbf{X}))$ is the odds ratio of the true propensity score $\pi_{o}(\mathbf{X}, U) = P(A= 1 \mid \mathbf{X}, U, S = o)$ that takes into account the unmeasured confounder $U$ and the observed propensity score $\pi_{o}(\mathbf{X}) = \bbP(A = 1 \mid \mathbf{X}, S = o)$. 
In this way, $\Delta$ measures the internal validity bias from the observational data. 
There are other ways to parametrize and represent the bias $\Delta$. Our method and theory developed in Sections \ref{sec:estimation} and \ref{sec:inference} do \emph{not} depend on the particular parametrization and allows for arbitrary bias from the observational-data-only estimator.

\subsection{Stabilized Estimators}\label{appx:stablization}
It is well know that IPW-type estimators like $\cippw, \caippw, \ooipw$, and $\ooaipw$ can be unstable when the (estimated) weights are close to zero. To alleviate this issue, one can apply the stabilization method by normalizing the weights to sum to one \citep{robins2007comment}. The stabilized estimators are asymptotically equivalent to their unstabilized counterparts but they have better finite-sample performance.
For example, the stabilized version of $\caippw$ is 
\begin{align*}
        &\hat\beta_{c, \textsf{sAIPPW}} \\
        &= \bigg[  \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{A_i(1-e_{{c}}(\mathbf{X}_i; \hat \bsxi )) }{\pi_c(\mathbf{X}_i)e_{{c}}(\mathbf{X}_i; \hat \bsxi ) }\bigg]^{-1} \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{A_i(1-e_{{c}}(\mathbf{X}_i; \hat \bsxi )) (Y_i -\mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} ) )  }{\pi_c(\mathbf{X}_i)e_{{c}}(\mathbf{X}_i; \hat \bsxi ) } \\
        &  - \bigg[  \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{(1-A_i)(1-e_{{c}}(\mathbf{X}_i; \hat \bsxi ))}{(1- \pi_c(\mathbf{X}_i))e_{{c}}(\mathbf{X}_i; \hat \bsxi )} \bigg]^{-1}\frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{(1-A_i)(1-e_{{c}}(\mathbf{X}_i; \hat \bsxi ))(Y_i -\mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ) ) }{(1- \pi_c(\mathbf{X}_i))e_{{c}}(\mathbf{X}_i; \hat \bsxi )}   \\
& + \frac{1}{n_c} \sum_{i\in \mathcal{O}_1} \mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} )   - \mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ). 
\end{align*}
% Finally, it is well know that estimators like $\hat\beta_{o_2, \textsf{IPW}}, \hat\beta_{o_2, \textsf{AIPW}}, \hat\beta_{c, \textsf{IPPW}},$ and $ \hat\beta_{c, \textsf{AIPPW}}$ can be unstable when the treatment assignment and study selection probability $\pi_o(\mathbf{x}), 1-\pi_o(\mathbf{x}),$ and $ e_c(\mathbf{x})$, or their parametric specifications are close to 0 for some $\mathbf{x}$. To alleviate this issue, one can apply the stabilization method by normalizing the weights to sum to 1 \citep{robins2007comment}.  For example, the stabilized RCT-based AIPPW estimator $\hat\beta_{c, \textsf{sAIPPW}}$ is 
% \begin{align} \label{eqn: c,sAIPPW}
% \begin{split}
%       \hat\beta_{c, \textsf{sAIPPW}} &= \bigg[  \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{A_i(1-e_{{c}}(\mathbf{X}_i; \hat \xi )) }{\pi_c(\mathbf{X}_i)e_{{c}}(\mathbf{X}_i; \hat \xi ) }\bigg]^{-1} \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{A_i(1-e_{{c}}(\mathbf{X}_i; \hat \xi )) (Y_i -\mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} ) )  }{\pi_c(\mathbf{X}_i)e_{{c}}(\mathbf{X}_i; \hat \xi ) } \\
%       & \qquad - \bigg[  \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{(1-A_i)(1-e_{{c}}(\mathbf{X}_i; \hat \xi ))}{(1- \pi_c(\mathbf{X}_i))e_{{c}}(\mathbf{X}_i; \hat \xi )} \bigg]^{-1}\frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{(1-A_i)(1-e_{{c}}(\mathbf{X}_i; \hat \xi ))(Y_i -\mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ) ) }{(1- \pi_c(\mathbf{X}_i))e_{{c}}(\mathbf{X}_i; \hat \xi )}   \\
% &\qquad + \frac{1}{n_c} \sum_{i\in \mathcal{O}_1} \mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} )   - \mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ); 
% \end{split}
% \end{align}
and the stabilized AIPW estimator version of $\ooaipw$ is given by 
\begin{align*}
% \begin{split}
        \hat\beta_{o_2, \textsf{sAIPW}} &=
        \bigg[\frac{1}{n_{o_2}} \sum_{i\in \mathcal{O}_2}\frac{A_i  }{\pi_{o}(\mathbf{X}_i; \hat\bseta )} \bigg]^{-1}\frac{1}{n_{o_2}} \sum_{i\in \mathcal{O}_2} \frac{A_i (Y_i -\mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} ) )  }{\pi_{o}(\mathbf{X}_i; \hat\bseta )}  \\
        & \qquad - \bigg[\frac{1}{n_{o_2}} \sum_{i\in \mathcal{O}_2}\frac{1-A_i  }{1-\pi_{o}(\mathbf{X}_i; \hat\bseta )} \bigg]^{-1}\frac{1}{n_{o_2}} \sum_{i\in \mathcal{O}_2}\frac{(1-A_i)(Y_i -\mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} ) ) }{1- \pi_{o}(\mathbf{X}_i;\hat\bseta)}\\
        &    \qquad   +\frac{1}{n_{o_2}} \sum_{i\in \mathcal{O}_2} \mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} )   - \mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} ). 
% \end{split}
\end{align*}


\subsection{Influence Function Representation}\label{appx:influence_func}
The estimators $\cippw, \caippw, \ooipw$, and $\ooaipw$ discussed in Section \ref{sec: setup} of the main article are generally referred to as the two-step estimators, which depend on some ``first-step''  estimators of nuisance parameters. A general device to analyze the two-step estimators is to stack the moment equations from the first step and the second step and apply the generalized method of moments (GMM) framework \citep[Chapter 6.1]{newey1994}. 

Take $\ooaipw$, the AIPW estimator based on the observational study, as an example.  Suppose that the first component of $\bfX$ is 1, representing the intercept. Let $O:= (Y, \bfX, A)$ denote the observed data vector and let $\bsphi = (\bsalpha_{o0}, \bsalpha_{o1},  \bseta) $ collect all nuisance parameters.  Then $\ooaipw$ can be written as the solution to a moment equation $n_{o_2}^{-1} \sum_{i\in \mathcal{O}_2}  g
(O_i, \beta; \hat \bsphi) = 0 $, where 
\begin{align*}
    g(O, \beta; \bsphi) &= \frac{A (Y- \mu_{o1} (\bfX; \bsalpha_{o1} )) }{\pi_o (\bfX; \bseta)} - \frac{(1-A) (Y-\mu_{o0} (\bfX; \bsalpha_{o0} )) }{1- \pi_o (\bfX; \bseta)} \\
    &\qquad + \mu_{o1} (\bfX; \bsalpha_{o1} )  - \mu_{o0} (\bfX; \bsalpha_{o0} ) - \beta. 
\end{align*}
The nuisance parameter estimator $\hat\bsphi$ can also be written as the solution to a set of moment equations $n_{o_2}^{-1} \sum_{i\in \mathcal{O}_2} m(O_i,  \bsphi) = 0 $, with $m(O, \bsphi)  = ( m(O, \bsalpha_{o0})^\top,  m(O, \bsalpha_{o1})^\top,  m(O, \bseta)^\top )^\top$, where 
\begin{align*}
       m(O, \bsalpha_{o0})& = (1- A) \bfX (Y-  \bsalpha_{o0}^\top \bfX), \\
       m(O, \bsalpha_{o1})& = A \bfX (Y-  \bsalpha_{o1}^\top \bfX), \\
       m(O, \bseta)& = \bfX (A-  \textsf{expit}(\bseta^\top \bfX)). 
\end{align*}
The definition of the moment equations $g $ and $m$, and the nuisance parameter $\bsphi$ should depend on the focal estimator, but we omit the subscripts for notational simplicity. 

 Let $\bar \bsphi$ be the solution to $\bbE[m(O, \bsphi)\mid S=o]= 0$ and let 
\begin{align*}
   &   G_\bsphi = \bbE [ \nabla_\bsphi g(O, \beta_o;\bar\bsphi)  \mid S=o ], \qquad M =  \bbE [ \nabla_\bsphi m(O, \bar\bsphi)  \mid S=o ],\\
    & g(O) = g(O, \beta_o;\bar\bsphi),  \qquad m(O) = m(O, \bar\bsphi). 
\end{align*}
By Theorem 6.1 of \cite{newey1994}, when either $\pi_o (\bfX; \bseta)$ or $\{\mu_{o0} (\bfX; \bsalpha_{o0} ), \mu_{o1} (\bfX; \bsalpha_{o1} )\}$ is correct,  we have that $\ooaipw$ is asymptotically linear, i.e., 
\begin{align*}
    \sqrt{n_{o_2}} (\ooaipw - \beta_o) =   \sum_{i\in \mathcal{O}_2} \{ g(O_i) - G_\bsphi M^{-1} m(O_i)  \} / \sqrt{n_{o_2}} +o_p(1). 
\end{align*}
Moreover, $\ooaipw$ is consistent and asymptotically normal, satisfying 
\begin{align*}
    \sqrt{n_{o_2}} (\ooaipw - \beta_o) \xrightarrow{d} N\big(0,  \bbE[ \{ g(O) - G_\bsphi M^{-1} m(O) \}^2\mid S=o ] \big). 
\end{align*}
This also gives a consistent variance estimator of $\ooaipw$ by replacing the population-level quantities in its asymptotic variance with their sample analogues. In practice, there is an easy way to obtain the variance estimator: first stack $g(O, \beta;\bsphi)$ and $m(O, \phi)$ together to form $\tilde g(O,\beta;\bsphi)= (g(O, \beta;\bsphi)^\top,m(O, \phi)^\top)^\top $, then solve for estimators of $(\beta, \bsphi^\top)^\top$ simultaneously using GMM (e.g., using the \textsf{gmm} package in \textsf{R} \citep{gmmpackage}). The variance estimator of $\ooaipw$ can be obtained immediately from the corresponding diagonal component of the outputted variance-covariance matrix.
The other estimators $\cippw, \caippw $ and $ \ooipw$ can be analyzed in the same way; the details are omitted. 





% \subsection{RCT as the Target Population}\label{appx:rct_as_target}
% If the RCT data represent our target population, then the counterpart of Assumption \ref{assump:target} is as follows.
% % \begin{assumption}[Target Population]
% \begin{customassump}{C'}[Target population]
% Assume 
% % either one of the following holds:
% % \begin{itemize}
%     % \item[(a)] The RCT data represent the target population, so that $(\mathbf{X}, Y(0), Y(1)\mid S=c) \overset{d}{=} ( \mathbf{X}, Y(0), Y(1))$;
%     % \item[(b)] 
%     $\bbE[Y(a)\mid \bfX, S = \rct] = \bbE[Y(a)\mid \bfX]$ for any $a\in\{0, 1\}$.
% % \end{itemize}
% \end{customassump}

% The above assumption implies that $\beta^\star = \beta^\star_\rct$.
% Now, the RCT-based estimators $\hat\beta_{c, \textsf{IPW}}$ and $\hat\beta_{c, \textsf{AIPW}}$ (as well as their stabilized versions) are free of both internal and external validity bias, making them consistent estimators of $\beta^\star$.

% On the other hand, the two estimators $\oipw$ and $\oaipw$ constructed using the observational data are even more invalid: in addition to the interval validity bias, they now have an extra source of bias, given by
% $$
%     \Delta_\exter = \beta^\star - \beta^\star_\obs = \beta^\star_\rct - \beta^\star_\obs.
% $$
% Without further assumptions, $\Delta_\exter$ can be further decomposed into two parts: one part arises from the variation in sample selection probability, and another arises from ``posterior drift'', namely $\bbE[Y(a)\mid\bfX, S = \obs]\neq \bbE[Y(a)\mid \bfX]$ for $a \in\{0, 1\}$. 
% While one can adjust for the external validity bias by assuming the counterpart of Assumption \ref{assump: study selection exchangeability} and adopting inverse participation probability weighting, we argue that the benefit from such adjustments are marginal. 
% For one thing, due to the presence of interval validity bias, it is not clear if such adjustments would decrease or further increase the overall bias $\Delta + \Delta_\exter$, where $\Delta$ is the interval validity bias defined in \eqref{eqn: Obs data internal validity bias}. For another, since $n_\rct$ is typically much smaller than $n_\obs$, the accuracy of such adjustments is not guaranteed. The forgoing discussion suggests that using $\oipw$ and $\oaipw$ (as well as their stabilized versions) may be the best one can do if the goal is to estimate $\beta^\star = \beta^\star_\rct$ with the observational data alone.

% Note that all the results in Section \ref{sec: method} can be generalized to accommodate the current setting, as one can absorb the extra $\Delta_\exter$ into the definition of $\Delta$.
% In fact, the results in Section \ref{sec: method} would hold as long as one can construct two estimators $\hat\beta_\rct$ and $\hat\beta_\obs$, where $\hat\beta_\rct$ is $\sqrt{n_\rct}$-consistent for $\beta^\star$, $\hat\beta_\obs$ is $\sqrt{n_\obs}$-consistent for $\beta_\obs$, and the overall bias is $\Delta = \beta^\star - \beta_\obs$. Thus, the method and theory developed in Section \ref{sec: method} can be extended to the case where there is a separate target population that is distinct from either RCT or observational data.

% \subsection{A Minimax Lower Bound in a Toy Causal Model}\label{appx:lb}


% Suppose the RCT data are generated as follows. For each $i\in\Rct$, we first generate a covariate vector $\bfX_i\sim \bbP_{\rct, X}$. Then, we generate the treatment $A_i \sim \Bern(\pi_\rct(\bfX_i))$ for some function $\pi_\rct(\bfx)$ that is strictly bounded away from zero and one for any $x$ in the support of $\bbP_{\rct, X}$. 
% Finally, we generate $Y_i(A_i) \sim N(A_i\beta^\star_\rct + \bsgamma_\rct^\top \bfX_i, \sigma_\rct^2)$ where $\bsgamma_\rct$ is a vector with the same dimension as $\bfX_i$. 
% We assume the target population is the RCT itself, i.e., $\beta^\star = \beta_\rct^\star$.
% Note that when $\bsgamma_\rct$ is known, then doing regression adjustment followed by IPW would give an estimator $\hat\beta_\rct$ that is distributed as $N(\beta^\star_\rct, \sigma_\rct^2/n_\rct)$.

% {\color{red}
% Meanwhile, suppose the observational data are generated as follows. 
% For each $i\in\Obs$, we first generate the treatment $A_i\sim \Bern(\pi_\obs)$, then we 
% generate an unmeasured confounding variable $U_i\sim N(A_i, 1)$ and a covariate vector $\bfX_i\sim \bbP_{\obs, X}$, where  $\bbP_{\obs, X}=\bbP_{\rct, X}$, i.e., there is no covariate shift. Hence, we have $\bfX_i\perp (A_i, U_i)$.  We finally generate $Y_i(A_i)\sim N(\beta^\star_\obs A_i + U_i + \bsgamma_\obs^\top \bfX_i, \sigma_\obs^2)$, where $\bsgamma_\obs$ is a vector with the same dimension as $\bfX_i$. Suppose that $\beta_\obs^\star=\beta_\rct^\star=\beta^\star$. Based on the imposed data generating process, we can marginalize over the distribution of $U_i\mid A_i, \bfX_i$ and obtain $Y_i(A_i)\mid\bfX_i, A_i\sim N((\beta^\star_\obs+1)A_i + \bsgamma_\obs^\top \bfX_i, \sigma_\obs^2+1)$. 
% When $\bsgamma_\obs$ is known, since $U_i$ is unobserved, 
% regression adjustment followed by IPW can only produce an estimator $\hat\beta_\obs$ that is distributed as $N(\beta_\obs, \sigma_{o}/n_{o_2})$, 
% where $\beta_\obs = \beta_\obs^\star +1$.
% }


% Meanwhile, suppose the observational data are generated as follows. 
% For each $i\in\Obs$, we first independently generate a confounding variable $U_i \sim \textnormal{Rademacher}(1/2)$ and a covariate vector $\bfX_i\sim \bbP_{\obs, X}$. 
% The treatment is generated according to $A_i \sim \Bern(\pi_\obs(\bfX_i, U_i))$, where the two functions $\pi_\obs(\bfx, \pm 1)$ are strictly bounded away from zero and one for any $x$ in the support of $\bbP_{\obs, X}$. 
% We finally generate $Y_i(A_i)\sim N((\beta^\star_\obs+U_i)A_i + \bsgamma_\obs^\top \bfX_i, \sigma_\obs^2)$, where $\bsgamma_\obs$ is a vector with the same dimension as $\bfX_i$. 
% Since $U_i$ has mean zero, $\beta_\obs^\star$ is the causal parameter in the observational data.
% Due to the presence of $U_i$, the observed data distribution differs from the potential outcome distribution. As the result, even if $\bsgamma_\obs$ is known, regression adjustment followed by IPW can only produce an estimator $\hat\beta_\obs$ that is distributed as $N(\beta_\obs, \sigma_\obs^2 /n_{\obs})$, where $\beta_\obs = \bbE[Y_i|A_i=1] - \bbE[Y_i|A_i=0]$.
% With some algebra, one can give an explicitly formula for $\beta_\obs$ (see Appendix \ref{prf:eq:beta_obs_explicit_formula} for a detailed proof):
% \begin{equation}
% 	\label{eq:beta_obs_explicit_formula}
% 	\beta_\obs = \beta_\obs^\star + \bbE\bigg[\frac{\pi_\obs(\bfX_i, 1) - \pi_\obs(\bfX_i, -1)}{\pi_\obs(\bfX_i, 1) + \pi_\obs(\bfX_i, -1)}\bigg] \in (\beta_\obs^\star - 1, \beta_\obs^\star + 1).
% \end{equation}	
% For simplicity, we assume $\pi_\obs(\bfx, \pm 1)$ are such that $\beta_\obs = 2\beta_\obs^\star$. Note that this implicitly places a restriction on the magnitude of $\beta_\obs^\star$. In particular, it is not hard to see that $-1 < \beta_\obs^\star < 1$ must hold. 

% Under this toy model, it is possible to construct RCT-based estimator $\hat\beta_\rct$ that consistently estimate $\beta^\star = \beta^\star_\rct$. However, it is impossible to do the same using the observational data along, due to the presence of both interval and external validity bias, and we quantify the overall bias by $\Delta = \beta^\star - \beta_\obs = \beta^\star_\rct - \beta_\obs$.
% % We assume there is no external validity bias in this toy model, namely $\beta_\rct^\star = \beta_\obs^\star = \beta^\star$. However, internal validity bias still exists, as one can see from \eqref{eq:beta_obs_explicit_formula}.
% We consider the following parameter space indexed by $\bar\Delta > 0$:
% \begin{align*}
% 	\label{eq:param_space}
% 	\calP(\bar\Delta) & := \{(\beta^\star_\rct, \beta^\star_\obs): |\beta^\star-\beta_\obs|\leq \bar\Delta 
% 	\}.\numberthis
% \end{align*}
% % Suppose the RCT data are generated by $A_i\sim \Bern(p_\rct), Y_i|A_i \sim N(A_i\beta_\rct^\star, \sigma_\rct^2)$ for any $i\in\Rct$, whereas the OS data are generated by $A_i\sim\Bern(p_\obs), Y_i |A_i \sim N(A_i\beta_\obs, \sigma_\obs^2)$ for any $i\in\Obs$. \sxc{effectively there is no unmeasured confounding in OS data so the only source of discrepancy stems from non-transportability. Is there any simple model that also takes unmeasured confounding into account?} Suppose $p_\rct, p_\obs$ are both strictly bounded away from one. Consider the following parameter space indexed by some $\Delta >0$:
% % \begin{equation}
% 	% \label{eq:param_space}
% 	% \calP(\Delta) := \{(\beta_\rct^\star, \beta_\obs)\in\bbR^2: |\beta^\star_\rct-\beta_\obs|\leq \Delta\}.
% % \end{equation}	
% The quantity $\bar\Delta$ is an upper bound on the magnitude of the overall bias $\Delta$.
% The following theorem gives the minimax lower bound for estimating $\beta^\star$ in the above toy model.


% % \begin{theorem}[Minimax lower bound]
% % \label{thm:lb}
% % Under the aforementioned model, we have
% % \begin{equation}
% % 	\label{eq:lb}
% % 	\inf_{\hat \beta} \sup_{(\beta^\star_\rct, \beta^\star_\obs)\in\calP(\bar\Delta)} \bbE[|\hat\beta - \beta^\star|^2] \gtrsim \frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} + \frac{\sigma_\rct^2}{n_\rct} \land \bar\Delta^2,
% % \end{equation}
% % where the infimum is taken over all measurable functions of the observed RCT and observational data.
% % \end{theorem}
% % \begin{proof}
% % 	See Appendix \ref{prf:thm:lb}.
% % \end{proof}
% % Comparing \eqref{eq:lb} with \eqref{eq:amse_convex_comb_alt_formula}, we see that the best convex combination $\hat\beta_{\weight^\star}$ is indeed minimax rate optimal, at least under the toy causal model considered above.

\newpage
\section{Technical Proofs}




\subsection{Proof of Theorem \ref{thm:oracle_estimator}}\label{prf:thm:oracle_estimator}
The proof relies on the following version of Berry-Esseen theorem.
\begin{theorem}[Berry-Esseen theorem]
\label{thm:berry_esseen}
Let $X_1, \hdots, X_n$ be independent random variables with 
$$
    \bbE[X_i] = 0, \qquad \bbE[X_i^2] = \sigma_i^2, \qquad \bbE[|X_i|^3]  = \rho_i, \qquad \forall i\in[n].
$$
Then 
$$
    \sup_{t\in\bbR} \bigg|\bbP\bigg( \frac{\sum_{i\in[n]} X_i}{\sqrt{\sum_{i\in[n]} \sigma_i^2}} \leq t\bigg) - \Phi(t)\bigg| \leq \frac{6\sum_{i\in[n]} \rho_i}{(\sum_{i\in[n]} \sigma_i^2)^{3/2}},
$$
where $\Phi(t)$ is the CDF of $N(0, 1)$.
\end{theorem}
\begin{proof}
    See, e.g., Theorem 2 in Chapter 16 of \cite{feller2008introduction}.
\end{proof}

We will in fact prove the following stronger result:
\begin{equation}
    \label{eq:amse_convergence_convex_comb}
    \sup_{{\tilde{\weight}}\in[0, 1]} \bigg|\frac{\bbE[|\hat\beta_{\tilde{\weight}} - \beta^\star|^2]}{\amse(\hat\beta_{\tilde{\weight}})} - 1\bigg| \to 0 \qquad \textnormal{as }  n_\rct \land n_{\obs} \to \infty,
\end{equation}  
where 
\begin{equation*}
    % \label{eq:amse_formula_convex_comb}
    \amse(\hat\beta_{\tilde{\weight}}) = 
    \frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2 \sigma_\obs^2}{n_{\obs}} + {\tilde{\weight}}^2\Delta^2.
\end{equation*}
The formula for $\amse(\hat\beta_\rct)$ and $\amse(\hat\beta_w)$ follows by setting $\tilde\weight = 0$ and $\tilde\weight = \weight$, respectively. As an immediate result, we have
$$
    \amse(\hat\beta_\orac) = 
    \begin{cases}
        \frac{\sigma_\rct^2}{n_\rct} & \textnormal{ if }  \overline\Delta \geq \sigma_c/\sqrt{n_\rct}\\
        \frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} + \weight^2 \Delta^2 & \textnormal{ otherwise},
    \end{cases}.
$$
If $\overline\Delta \geq \sigma_\rct/\sqrt{n_\rct}$, we have
$$
    \amse(\hat\beta_\orac) = \frac{\sigma_\rct^2}{n_\rct}  = \frac{\sigma_\rct^2}{n_\rct}\land \overline{\Delta}^2 \leq 
    \frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} +  \frac{\sigma_\rct^2}{n_\rct}\land {\overline{\Delta}^2}.
$$
If $\overline\Delta < \sigma_\rct/\sqrt{n_\rct}$, we have
$$
   \amse(\hat\beta_\orac) \leq  \frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} + \weight^2 \Delta^2 \leq \frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} + \overline\Delta^2 = \frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} +  \frac{\sigma_\rct^2}{n_\rct}\land \overline{\Delta}^2.
$$
% Since $n_\obs \geq (1+\ep)n_\rct$, we have
% $
%     n_{\obs} = n_\obs - n_\rct \geq n_\obs - \frac{1}{1+\ep} n_\obs = \frac{\ep}{1+\ep} n_\obs \gtrsim n_\obs.
% $
% It follows that
% $$
%     \amse(\hat\beta_\orac) \lesssim 
%     \frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} + \overline\Delta^2
%      = \frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} +  \frac{\sigma_\rct^2}{n_\rct}\land \overline{\Delta}.
% $$
The formula for $\amse(\hat\beta_\orac)$ follows by combining the above two cases.


It suffices to prove \eqref{eq:amse_convergence_convex_comb}.
For notational simplicity, we write $\psi_\rct(X_i, A_i, Y_i) = \psi_{\rct, i}$ for $i\in\Rct$ and $\psi_\obs(X_i, A_i, Y_i) = \psi_{\obs, i}$ for $i\in\Obs$.
By Berry-Esseen theorem (see Theorem \ref{thm:berry_esseen}), for any fixed ${\tilde{\weight}}\in[0, 1]$, we have
\begin{align*}
     \sup_{t\in\bbR}\bigg|\bbP\bigg[ 
    \frac{ {(1-{\tilde{\weight}}) n_\rct^{-1} \sum_{i\in\Rct} \psi_{\rct, i}} + {{\tilde{\weight}} n_{\obs}^{-1}\sum_{i\in\Obs} \psi_{\obs, i}} }{\sqrt{\frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2 \sigma_\obs^2}{n_{\obs}}}} \leq t\bigg] - \Phi(t)\bigg| 
    & \leq 6 \cdot \frac{\frac{(1-{\tilde{\weight}})^3 \rho_\rct}{n_\rct^2} + \frac{{\tilde{\weight}}^3 \rho_\obs}{n_{\obs}^2}}{\bigg(\frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2\sigma_\obs^2}{n_{\obs}}\bigg)^{3/2}}\\
    & \leq 6 \bigg(\frac{\rho_\rct}{\sigma_\rct^3 \sqrt{n_\rct}} + \frac{\rho_\obs}{\sigma_\obs^3 \sqrt{n_{\obs}}}\bigg).
\end{align*}
Taking the supremum over ${\tilde{\weight}}\in[0, 1]$ at both sides, we get
\begin{align*}
    & \sup_{{\tilde{\weight}} \in [0, 1]}
    \sup_{t\in\bbR}\bigg|\bbP\bigg[ 
    \frac{ {(1-{\tilde{\weight}}) n_\rct^{-1} \sum_{i\in\Rct} \psi_{\rct, i}} + {{\tilde{\weight}} n_{\obs}^{-1}\sum_{i\in\Obs} \psi_{\obs, i}} }{\sqrt{\frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2 \sigma_\obs^2}{n_{\obs}}}} \leq t\bigg] - \Phi(t)\bigg| 
    \label{eq:berry_esseen_comvex_comb}
    \leq 6 \bigg(\frac{\rho_\rct}{\sigma_\rct^3 \sqrt{n_\rct}} + \frac{\rho_\obs}{\sigma_\obs^3 \sqrt{n_{\obs}}}\bigg).\numberthis
\end{align*}
From the definition of $\hat\beta_{\tilde{\weight}}$ and Assumption \ref{assump:asymp_linear}, we have
\begin{align*}
    \frac{\hat\beta_{\tilde{\weight}} - [(1-{\tilde{\weight}})\beta^\star + {\tilde{\weight}} \beta_\obs]}{\sqrt{ \frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2 \sigma_\obs^2}{n_{\obs}}}} 
    & = \frac{ (1-{\tilde{\weight}})n_\rct^{-1} \sum_{i\in\calC} \psi_{\rct, i} + {\tilde{\weight}} n_{\obs}^{-1}\sum_{i\in\Obs}\psi_{\obs, i} + (1-{\tilde{\weight}}) o_p(n_\rct^{-1/2}) + {\tilde{\weight}} o_p(n_{\obs}^{-1/2}) }{\sqrt{ \frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2 \sigma_\obs^2}{n_{\obs}}}} \\
    & = \frac{ (1-{\tilde{\weight}})n_\rct^{-1} \sum_{i\in\calC} \psi_{\rct, i} + {\tilde{\weight}} n_{\obs}^{-1}\sum_{i\in\Obs}\psi_{\obs, i}  }{\sqrt{ \frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2 \sigma_\obs^2}{n_{\obs}}}} + o_p(1).
\end{align*}
Using \eqref{eq:berry_esseen_comvex_comb} and invoking Slutsky's theorem, we get
\begin{equation}
    \label{eq:asymp_normal_convex_comb}
    \frac{\hat\beta_{\tilde{\weight}} - [(1-{\tilde{\weight}})\beta^\star + {\tilde{\weight}} \beta_\obs]}{\sqrt{ \frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2 \sigma_\obs^2}{n_{\obs}}}} \xrightarrow{d} N(0, 1)
\end{equation}  
as $n_\rct \land n_{\obs} \to \infty$, where $\overset{d}{\to}$ denotes convergence in distribution and the rate of convergence is independent of the value of ${\tilde{\weight}}$. We now write
\begin{align*}
    & |\hat \beta_{\tilde{\weight}} - \beta^\star|^2 \\
    & = \bigg| (1-{\tilde{\weight}})\hat\beta_\rct + {\tilde{\weight}} \hat\beta_\obs - [(1-{\tilde{\weight}})\beta^\star + {\tilde{\weight}} \beta_\obs] - {\tilde{\weight}} \Delta\bigg|^2 \\
    & = \bigg| (1-{\tilde{\weight}})\hat\beta_\rct + {\tilde{\weight}} \hat\beta_\obs - [(1-{\tilde{\weight}})\beta^\star + {\tilde{\weight}} \beta_\obs]\bigg|^2 - 2 {\tilde{\weight}} \Delta \bigg((1-{\tilde{\weight}})\hat\beta_\rct + {\tilde{\weight}} \hat\beta_\obs - [(1-{\tilde{\weight}})\beta^\star + {\tilde{\weight}} \beta_\obs]\bigg) + {\tilde{\weight}}^2\Delta^2.
\end{align*}
By \eqref{eq:asymp_normal_convex_comb}, we have
\begin{align*}
    & \frac{\bbE\bigg| (1-{\tilde{\weight}})\hat\beta_\rct + {\tilde{\weight}} \hat\beta_\obs - [(1-{\tilde{\weight}})\beta^\star + {\tilde{\weight}} \beta_\obs]\bigg|^2}{ \frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2 \sigma_\obs^2}{n_{\obs}}}  = 1+o(1), \qquad \frac{\bbE\bigg[ (1-{\tilde{\weight}})\hat\beta_\rct + {\tilde{\weight}} \hat\beta_\obs - [(1-{\tilde{\weight}})\beta^\star + {\tilde{\weight}} \beta_\obs] \bigg]}{\sqrt{ \frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2 \sigma_\obs^2}{n_{\obs}}}} = o(1),
\end{align*}
where the $o(1)$ term is independent of the value of ${\tilde{\weight}}$. Thus, 
\begin{align*}
     \frac{\bbE|\hat\beta_{\tilde{\weight}} - \beta^\star|^2}{\frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2 \sigma_\obs^2}{n_{\obs}} + {\tilde{\weight}}^2\Delta^2} 
    & =  1 + o(1) +  \frac{\bbE\bigg[(1-{\tilde{\weight}})\hat\beta_\rct + {\tilde{\weight}} \hat\beta_\obs - [(1-{\tilde{\weight}})\beta^\star + {\tilde{\weight}} \beta_\obs]\bigg]}{\sqrt{\frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2 \sigma_\obs^2}{n_{\obs}}}} \cdot \frac{2 {\tilde{\weight}} \Delta \sqrt{ \frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2 \sigma_\obs^2}{n_{\obs}} }}{\frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2 \sigma_\obs^2}{n_{\obs}} + {\tilde{\weight}}^2\Delta^2} \\
    & = 1+ o(1) + o(1) \cdot \frac{2 {\tilde{\weight}} \Delta \sqrt{ \frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2 \sigma_\obs^2}{n_{\obs}} }}{\frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2 \sigma_\obs^2}{n_{\obs}} + {\tilde{\weight}}^2\Delta^2}.
    % & = 1 + o(1),
\end{align*}
The proof of \eqref{eq:amse_convergence_convex_comb} is concluded by noting that
$$
    \frac{2 |{\tilde{\weight}} \Delta| \sqrt{ \frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2 \sigma_\obs^2}{n_{\obs}} }}{\frac{(1-{\tilde{\weight}})^2 \sigma_\rct^2}{n_\rct} + \frac{{\tilde{\weight}}^2 \sigma_\obs^2}{n_{\obs}} + {\tilde{\weight}}^2\Delta^2} \leq 1,
$$
which follows from $a^2 + b^2 \geq 2ab$ for any $a, b \in \bbR$.








\subsection{Proof of Theorem \ref{thm:lb}}\label{prf:thm:lb}
    We first prove
    \begin{equation}
        \label{eq:lb_1}
        \inf_{\hat\beta} \sup_{(\beta^\star, \beta_\obs)\in \calP_{\overline\Delta}} \bbE [|\hat \beta - \beta^\star|^2] 
        \gtrsim \frac{\sigma_\rct^2}{n_\rct} \land \bar\Delta^2 .
    \end{equation}  
    To show this, consider the prior distribution $\beta^\star = \delta v_\rct, \beta_\obs = \delta v_\obs$, where $v_\rct, v_\obs \in \{\pm 1\}$ are independent symmetric Rademacher random variables, and $\delta$ is a constant that satisfies $\delta\leq \bar\Delta/2$, whose exact value will be determined later. The requirement of $\delta \leq \bar\Delta/2$ is to make sure 
    $$
    |\beta^\star - \beta_\obs| = \delta |v_\rct - v_\obs|\leq \overline\Delta,
    $$ 
    so that the specified prior distribution is indeed placed on the parameter space $\calP_{\overline\Delta}$. 
    Now, we proceed by
    \begin{align*}
        & \inf_{\hat\beta} \sup_{(\beta^\star, \beta_\obs)\in \calP_{\overline\Delta}} \bbE [|\hat \beta - \beta^\star|^2] \\
        & \geq 
        \inf_{\hat\beta} \bbE_{v_c, v_o} \bbE [|\hat \beta - \delta v_\rct|^2] \\
        & = \delta^2 \inf_{\hat v_\rct\in\{\pm 1\}}\bbE_{v_\rct, v_\obs} \bbE[|\hat v_\rct - v_\rct|^2] \\
        & \gtrsim \delta^2 \inf_{\hat v_\rct\in\{\pm 1\}}\bbE_{v_\rct, v_\obs} \bbP(\hat v_\rct \neq v_\rct)  \\
        & \geq \delta^2 \bbE_{v_\obs,\{\bfX_i\}, \{A_i\}}\inf_{\hat v_\rct\in\{\pm 1\}}\bbP(\hat v_\rct \neq v_\rct ~|~ v_\obs, \{\bfX_i\}, \{A_i\})\\
        & = \delta^2 \bbE_{v_\obs,\{\bfX_i\}, \{A_i\}} \inf_{\hat v_\rct\in\{\pm 1\}} \frac{1}{2}\bigg(\bbP(\hat v_\rct = -1 ~|~ v_\rct = +1, v_\obs, \{\bfX_i\}, \{A_i\})\\
        \label{eq:lb_reduction}
        & \qquad\qquad\qquad\qquad\qquad\qquad\qquad  + \bbP(\hat v_\rct = +1 ~|~ v_\rct = -1, v_\obs,  \{\bfX_i\}, \{A_i\})\bigg) \numberthis,
    \end{align*}
    Note that the infimum term in the right-hand side above is the type-\RN{1} plus type-\RN{2} error of testing $H_0: v_\rct = +1$ v.s. $H_1: v_\rct = -1$ conditional on the knowledge of $v_\obs$, $\{A_i: i\in \Rct\cup \Obs\}$ and $\{\bfX_i: i\in \Rct\cup\Obs\}$. The likelihood function under $H_0$ is given by
    \begin{align*}
        L_0 & = \bigg(\prod_{i\in\Rct, A_i = 1} \frac{1}{\sqrt{2\pi \sigma_\rct^2}} \exp\{-(Y_i - \delta/2 - \bsgamma_\rct^\top \bfX_i)^2/(2\sigma_\rct^2)\}\bigg) \\
        & \qquad \times \bigg(\prod_{i\in\Rct, A_i = 0}\frac{1}{\sqrt{2\pi \sigma_\rct^2}} \exp\{-(Y_i + \delta/2 - \bsgamma_\rct^\top \bfX_i)^2/(2\sigma_\rct^2)\}\bigg) \\
        & \qquad \times \bigg(\prod_{i\in\Obs, A_i = 1} \frac{1}{\sqrt{2\pi \sigma_\obs^2}} \exp\{-(Y_i - \delta v_\obs/2 - \bsgamma_\obs^\top \bfX_i)^2/(2\sigma_\obs^2)\}\bigg) \\
        & \qquad \times
        \bigg(\prod_{i\in\Obs, A_i = 0} \frac{1}{\sqrt{2\pi \sigma_\obs^2}} \exp\{-(Y_i + \delta v_\obs/2 -\bsgamma_\obs^\top \bfX_i)^2/(2\sigma_\obs^2)\}\bigg),
    \end{align*}    
    and the likelihood function under $H_1$ is given by
    \begin{align*}
        L_1 & = \bigg(\prod_{i\in\Rct, A_i = 1} \frac{1}{\sqrt{2\pi \sigma_\rct^2}} \exp\{-(Y_i + \delta/2 - \bsgamma_\rct^\top \bfX_i)^2/(2\sigma_\rct^2)\}\bigg) \\
        & \qquad \times \bigg(\prod_{i\in\Rct, A_i = 0} \frac{1}{\sqrt{2\pi \sigma_\rct^2}} \exp\{-(Y_i - \delta/2 - \bsgamma_\rct^\top \bfX_i)^2/(2\sigma_\rct^2)\}\bigg) \\
        & \qquad \times \bigg(\prod_{i\in\Obs, A_i = 1} \frac{1}{\sqrt{2\pi \sigma_\obs^2}} \exp\{-(Y_i - \delta v_\obs/2 - \bsgamma_\obs^\top \bfX_i)^2/(2\sigma_\obs^2)\}\bigg) \\
        & \qquad \times
        \bigg(\prod_{i\in\Obs, A_i = 0} \frac{1}{\sqrt{2\pi \sigma_\obs^2}} \exp\{-(Y_i + \delta v_\obs/2 -\bsgamma_\obs^\top \bfX_i)^2/(2\sigma_\obs^2)\}\bigg),
    \end{align*}    
    By Neyman--Pearson Lemma, the optimal test that minimizes the sum of type-\RN{1} and type-\RN{2} error is given by rejecting $H_0$ when $L_1 \geq L_0$. This criterion translates to rejecting $H_0$ when
    $$
        \sum_{i\in\Rct, A_i = 1} (Y_i -\bsgamma_\rct^\top \bfX_i) - \sum_{i\in\Rct, A_i = 0} (Y_i -\bsgamma_\rct^\top \bfX_i)\leq 0.
    $$
    Under $H_0$, we know that $Y_i - \bsgamma_\rct^\top \bfX_i \mid A_i, \bfX_i \overset{i.i.d.}{\sim} N( (A_i-1/2)\delta, \sigma_\rct^2)$ for any $i\in\Rct$.
    Denoting $n_{\rct, 1} = |\{i\in \Rct: A_i = 1\}|$ and $n_{\rct, 0} = |\{i\in \Rct: A_i = 0\}|$.
    The left-hand side above is then distributed as
    $$
        N\bigg(
            \frac{\delta(n_{c, 1} + n_{c, 0})}{2},
            \sigma_\rct^2 (n_{c, 1} + n_{c, 0})
        \bigg)
        \overset{d}{=}
        N\bigg(
            \frac{\delta n_\rct}{2},
            \sigma_\rct^2 n_\rct
        \bigg).
    $$
    Thus, the type-\RN{1} error is given by
    \begin{align*}
        \bbP\bigg[
        N\bigg(
            \frac{\delta n_\rct}{2},
            \sigma_\rct^2 n_\rct
        \bigg) \leq 0
        \bigg] = \Phi \bigg(- \frac{\delta}{2 \sigma_\rct/\sqrt{n_\rct}}\bigg).
        % \bbP\bigg(N(n_{\rct, +} \delta^2, n_{\rct, +} \delta^2 \sigma_\rct^2) \leq 0\bigg)
        % & = \Phi\bigg(-\frac{\delta}{\sigma_{\rct}/\sqrt{n_{\rct, +}}}\bigg) 
        % \geq  \Phi\bigg(-\frac{\delta}{\sigma_{\rct}/\sqrt{C_1 n_{\rct}}}\bigg),
    \end{align*}
    % where the last inequality is by the fact that testing is conducted conditional on the event $\calE$. 
    A symmetric argument shows that the type-\RN{2} error also admits the above lower bound. Thus, we have
    \begin{align*}
        \inf_{\hat\beta} \sup_{(\beta^\star, \beta_\obs)\in \calP_{\overline\Delta}} \bbE [|\hat \beta - \beta^\star|^2] 
        & \gtrsim \delta^2 \Phi\bigg(-\frac{\delta}{2 \sigma_{\rct}/\sqrt{n_{\rct}}}\bigg)
    \end{align*}
    for any $\delta\leq \overline\Delta/2$. We consider the following two cases.
    \begin{enumerate}
        \item If $\overline\Delta^2 \geq \sigma_\rct^2/n_\rct$, we choose $\delta = \sigma_\rct/(2\sqrt{n_\rct})$, which gives 
        $$
        \inf_{\hat\beta} \sup_{(\beta^\star, \beta_\obs)\in \calP_{\overline\Delta}} \bbE [|\hat \beta - \beta^\star|^2] 
        \gtrsim \frac{\sigma_\rct^2}{n_\rct}.
        $$
        \item If $\overline\Delta^2 < \sigma_\rct^2/n_\rct$, we choose $\delta = \overline\Delta/2$, which gives 
        $$
        \inf_{\hat\beta} \sup_{(\beta^\star, \beta_\obs)\in \calP_{\overline\Delta}} \bbE [|\hat \beta - \beta^\star|^2] 
        \gtrsim \overline\Delta^2\Phi\bigg(-\frac{\overline\Delta}{2 \sigma_\rct/\sqrt{n_c}}\bigg) \gtrsim \overline\Delta^2 .
        $$
    \end{enumerate}
    % Note that in both cases above, the choice of $\delta$ makes $|\beta_\obs^\star| = \delta/2 = o(1)$, so that $\beta_\obs^\star$ satisfies the implicit constraints placed by our model for the observational data.
    Equation \eqref{eq:lb_1} follows from the above two cases. 

    We then show
    \begin{equation}
        \label{eq:lb_2}
        \inf_{\hat\beta} \sup_{(\beta^\star, \beta_\obs)\in \calP_{\overline\Delta}} \bbE [|\hat \beta - \beta^\star|^2] 
        \gtrsim \frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_\obs \sigma_\rct^2}.
    \end{equation}  
    If the above inequality holds, then we get
    $$
        \inf_{\hat\beta} \sup_{(\beta^\star, \beta_\obs)\in \calP_{\overline\Delta}} \bbE [|\hat \beta - \beta^\star|^2] 
        \gtrsim \bigg(\frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_\obs \sigma_\rct^2}\bigg) \lor  \bigg(\frac{\sigma_\rct^2}{n_\rct} \land \overline\Delta^2\bigg) 
        \gtrsim \frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_\obs \sigma_\rct^2} + \frac{\sigma_\rct^2}{n_\rct} \land \overline\Delta^2
        ,
    $$
    which is our desired result. To show \eqref{eq:lb_2}, we consider the prior distribution $\beta^\star = \beta_\obs = \delta v$, where $v$ is a symmetric Rademacher random variable and $\delta > 0$ is a constant whose value will be specified later. 
    Note that under this prior distribution, $|\beta^\star-\beta_\obs| = 0$, so $(\beta^\star, \beta_\obs)\in\calP(\bar\Delta)$ automatically holds. Using a nearly identical argument as what led to \eqref{eq:lb_reduction}, we have
    % \begin{align*}
    %   & \inf_{\hat\beta} \sup_{(\beta^\star, \beta_\obs)\in \calP(\bar\Delta)} \bbE [|\hat \beta - \beta^\star|^2] \\
    %   & \gtrsim \delta^2 \bbE_{\{A_i\}|\calE}\inf_{\hat v\in\{\pm 1\}} \frac{1}{2}\bigg(\bbP(\hat v = -1 ~|~ v = +1, \calE, \{A_i\}) + \bbP(\hat v = +1 ~|~ v = -1, \calE, \{A_i\})\bigg).
    % \end{align*}  
    \begin{align*}
        & \inf_{\hat\beta} \sup_{(\beta^\star, \beta_\obs)\in \calP_{\overline\Delta}} \bbE [|\hat \beta - \beta^\star|^2] \\
        & \gtrsim \delta^2 \bbE_{\{\bfX_i\}, \{A_i\}}\inf_{\hat v\in\{\pm 1\}} \frac{1}{2}\bigg(\bbP(\hat v= -1 ~|~ v = +1, \{A_i\}, \{\bfX_i\}) + \bbP(\hat v= +1 ~|~ v= -1, \{A_i\}, \{\bfX_i\})\bigg) ,
    \end{align*}
    The right-hand side above again amounts to a binary hypothesis testing problem between $H_0: v = +1$ and $H_1: v = -1$ given the knowledge of $\{A_i\}$ and $\{\bfX_i\}$. The likelihood functions can again be explicitly calculated, and with some algebra, we arrive at the following optimal test, which rejects $H_0$ when
    $$
        \frac{1}{\sigma_\rct^2} \sum_{i\in\Rct, A_i = 1} (Y_i - \bsgamma_\rct^\top \bfX_i) - \frac{1}{\sigma_\rct^2} \sum_{i\in\Rct, A_i = 0} (Y_i - \bsgamma_\rct^\top \bfX_i) + \frac{1}{\sigma_\obs^2} \sum_{i\in\Obs, A_i = 1} (Y_i - \bsgamma_\obs^\top \bfX_i) -  \frac{1}{\sigma_\obs^2} \sum_{i\in\Obs, A_i = 0} (Y_i - \bsgamma_\obs^\top \bfX_i) \leq 0.
    $$
    Under $H_0$, we have $Y_i- \bsgamma_\rct^\top \bfX_i \mid A_i, \bfX_i \overset{i.i.d.}\sim N( (A_i-1/2)\delta, \sigma_\rct^2)$ for $i \in \Rct$ and $Y_i - \bsgamma_\obs^\top \bfX_i\mid A_i, \bfX_i \overset{i.i.d.}\sim N((A_i - 1/2)\delta, \sigma_\obs^2)$ for $i \in \Obs$. Thus, 
    the type-\RN{1} error (and type-\RN{2} error as well by a symmetric argument) takes the following form:
    \begin{align*}
        \bbP\bigg[ N\bigg( \frac{\delta n_\rct}{2\sigma_\rct^2} + \frac{\delta n_{\obs}}{2\sigma_\obs^2}, \frac{n_{\rct} }{\sigma_\rct^2} + \frac{n_{\obs}}{\sigma_\obs^2}\bigg)  \leq 0\bigg] 
        & = \Phi\bigg({-\frac{\delta}{2}\sqrt{\frac{n_{\rct}}{\sigma_\rct^2} + \frac{n_{\obs}}{2\sigma_\obs^2}}}\bigg) .
        % \geq \Phi\bigg(- C\delta \cdot \sqrt{\frac{n_{\rct}}{\sigma_\rct^2} + \frac{n_{\obs}}{\sigma_\obs^2}}\bigg),
    \end{align*}
    Choosing $\delta = 1 / \sqrt{\frac{n_{\rct}}{\sigma_\rct^2} + \frac{n_{\obs}}{\sigma_\obs^2}}$, we get
    $$
        \inf_{\hat\beta} \sup_{(\beta^\star, \beta_\obs)\in \calP_{\overline\Delta}} \bbE [|\hat \beta - \beta^\star|^2] \gtrsim \frac{1}{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2},
    $$
    which is exactly \eqref{eq:lb_2}. The proof is concluded.




\subsection{Proof of Theorem \ref{thm:high_prob_bound_adaptive_estimator}} \label{prf:thm:high_prob_bound_adaptive_estimator}
% By the same arguments as those in the proof of Proposition \ref{prop:amse_convex_comb_alt_formula}, we have $n_\obs \asymp n_{\obs}$ and $\sigma_\rct^2/n_\rct \gtrsim \sigma_{\obs}^2/n_{\obs}$. Moreover, the assumption of $n_\rct \land n_\obs \to \infty$ is equivalent to $n_\rct \land n_{\obs} \to \infty$.

Similar to the proof of Theorem \ref{thm:oracle_estimator}, we write $\psi_\rct(X_i, A_i, Y_i) = \psi_{\rct, i}$ for $i\in\Rct$ and $\psi_\obs(X_i, A_i, Y_i) = \psi_{\obs, i}$ for $i\in\Obs$.
% We have shown in the Proof of Theorem \ref{thm:oracle_estimator} that $n_\obs \geq (1+\ep)n_\rct$ implies $n_{\obs}\gtrsim n_\obs$. Thus, $n_\rct \land n_\obs \to \infty$ is equivalent to $n_\rct \land n_{\obs}\to\infty$ and $\frac{\sigma_\rct^2}{n_\rct}\gtrsim \frac{\sigma_\obs^2}{n_\obs}$ is equivalent to $\frac{\sigma_\rct^2}{n_\rct}\gtrsim \frac{\sigma_\obs^2}{n_{\obs}}$.

We first show that $\Delta$ is feasible for \eqref{eq:est_delta} with high probability. By construction, we have
\begin{align*}
    \frac{\tilde \Delta - \Delta}{\sqrt{\frac{\sigma_\rct^2}{n_\rct} + \frac{\sigma_\obs^2}{n_{\obs}}}} 
    = \frac{n_\rct^{-1}\sum_{i\in\Rct} \psi_{\rct, i} - n_{\obs}^{-1}\sum_{i\in\Obs}\psi_{\obs, i}}{\sqrt{\frac{\sigma_\rct^2}{n_\rct} + \frac{\sigma_\obs^2}{n_{\obs}}}} + o_p(1).
\end{align*}
An application of Berry-Esseen theorem (see Theorem \ref{thm:berry_esseen}) gives
\begin{align*}
    \sup_{t\in\bbR}\bigg| \bbP\bigg( \frac{n_\rct^{-1}\sum_{i\in\Rct} \psi_{\rct, i} - n_{\obs}^{-1}\sum_{i\in\Obs}\psi_{\obs, i}}{\sqrt{\frac{\sigma_\rct^2}{n_\rct} + \frac{\sigma_\obs^2}{n_{\obs}}}} \leq t \bigg) -\Phi(t) \bigg| \leq 6 \cdot \frac{\frac{\rho_\rct}{n_\rct^2} + \frac{\rho_\obs}{n_{\obs}^2}}{(\frac{\sigma_\rct^2}{n_\rct} + \frac{\sigma_\obs^2}{n_{\obs}})^{3/2}} \leq 6 \bigg(\frac{\rho_\rct}{\sigma_\rct^3 \sqrt{n_\rct}} + \frac{\rho_\obs}{\sigma_\obs^3 \sqrt{n_{\obs}}}\bigg)  = o(1),
\end{align*}
where the last inequality is by $n_\rct \land n_{\obs} \to \infty$.
Thus, for any $t > 0$, we have
$$
    \bigg|\frac{n_\rct^{-1}\sum_{i\in\Rct} \psi_{\rct, i} - n_{\obs}^{-1}\sum_{i\in\Obs}\psi_{\obs, i}}{\sqrt{\frac{\sigma_\rct^2}{n_\rct} + \frac{\sigma_\obs^2}{n_{\obs}}}}\bigg| \leq t
$$
with probability at least $1-2\Phi(-t) - o(1)$. As long as $t \gtrsim 1$, the magnitude of the $o_p(1)$ term is at most $t$ with probability at least $1-o(1)$. Thus, a union bound gives that with probability at least $1-2\Phi(-t) - o(1)$, 
$$
    |\tilde\Delta - \Delta| \lesssim  t \sqrt{\frac{\sigma_\rct^2}{n_\rct} + \frac{\sigma_\obs^2}{n_{\obs}}}.
$$
Consider the event
$$
    \calE := \{0.9\sigma_\rct \leq \hat \sigma_\rct \leq 1.1\sigma_\rct\} \cap \{0.9\sigma_\obs \leq \hat \sigma_\obs \leq 1.1\sigma_\obs\}.
$$
Since $\hat\sigma_\rct\overset{p}{\to}{\sigma_\rct}$ and $\hat\sigma_\obs\overset{p}{\to}{\sigma_\obs}$, we know that $\bbP(\calE) \geq 1-o(1)$. Thus, we have
$$
    |\tilde\Delta - \Delta| \leq C t \sqrt{\frac{\hat\sigma_\rct^2}{n_\rct} + \frac{\hat\sigma_\obs^2}{n_{\obs}}}
$$
with probability $1-2\Phi(-t)-o(1)$, where $C>0$ is some absolute constant. Under the choice of $t = \lambda/C$, the above bound reads
\begin{align*}
    \bbP\bigg(|\tilde\Delta - \Delta| \leq \lambda \cdot \sqrt{\frac{\hat\sigma_\rct^2}{n_\rct} + \frac{\hat\sigma_\obs^2}{n_{\obs}}}\bigg) 
    & \geq 1 - 2\Phi(-{\lambda}/{C}) - o(1)\\
    & \geq 1 - \calO(e^{-\lambda^2/(2C^2)}) - o(1) \\
    \label{eq:high_prob_feasible}
    & \geq 1- e^{-\sfc \lambda^2} - o(1).\numberthis
\end{align*}    
Here, the second inequality above is by the Gaussian tail bound $\Phi(-t) \leq \frac{1}{t\sqrt{2\pi}}e^{-t^2/2}$ and $\lambda \gtrsim 1$, and $\sfc > 0$ is an absolute constant only depending on $C$. Thus, we have shown that $\Delta$ is feasible for for \eqref{eq:est_delta} with probability at least $1- e^{-\sfc \lambda^2} - o(1)$.
On this high probability event, we have $|\hat\Delta_\lambda|\leq |\Delta|$, which further yields
\begin{equation}
    \label{eq:ub_by_delta}
    |\hat\Delta_\lambda -\Delta| \leq 2|\Delta|.
\end{equation}
Meanwhile, on the same high probability event, we have
\begin{align*}
    |\hat\Delta_\lambda - \Delta| & \leq |\tilde \Delta - \Delta| + |\hat \Delta_\lambda - \tilde \Delta|  \\
    & \leq \lambda \cdot \sqrt{\frac{\hat\sigma_\rct^2}{n_\rct} + \frac{\hat\sigma_\obs^2}{n_{\obs}}} +  |\hat\Delta_\lambda - \tilde \Delta|\\
    & \leq 2\lambda \cdot \sqrt{\frac{\hat\sigma_\rct^2}{n_\rct} + \frac{\hat\sigma_\obs^2}{n_{\obs}}},
\end{align*}    
where the second inequality is by \eqref{eq:high_prob_feasible} and the last inequality is by the constraint in \eqref{eq:est_delta}. Recall that the high probability event in \eqref{eq:high_prob_feasible} is a superset of the event $\calE$, so we can further upper bound the right-hand side above by
\begin{equation}
    \label{eq:ub_by_sd}
    2\sqrt{1.1} \cdot \lambda \cdot \sqrt{\frac{\sigma_\rct^2}{n_\rct} + \frac{\sigma_\obs^2}{n_{\obs}}}.
\end{equation}  
Summarizing \eqref{eq:ub_by_delta} and \eqref{eq:ub_by_sd}, we arrive at
\begin{equation}
    \label{eq:est_err_delta}
    \bbP\bigg[|\hat\Delta_\lambda - \Delta| \lesssim \bigg(\lambda \cdot \sqrt{\frac{\sigma_\rct^2}{n_\rct} + \frac{\sigma_\obs^2}{n_{\obs}}}\bigg) \land |\Delta|\bigg]  \geq 1- e^{-\sfc \lambda^2} - o(1).
\end{equation}  
Denote $\tilde \beta = (1-\hat\weight)\hat\beta_\rct + \hat\weight \hat\beta_\obs$, so that $\hat\beta_\lambda = \tilde \beta + \hat\weight \hat\Delta_\lambda$.
To analyze $\hat\beta_\lambda$, we decompose
\begin{align*}
    |\hat \beta_\lambda - \beta^\star|^2 & \lesssim \bigg|\tilde \beta - \bigg(\hat\weight \cdot \beta_\obs + (1-\hat\weight) \cdot \beta^\star\bigg)\bigg|^2 + \bigg|\bigg(\hat\weight \cdot \beta_\obs + (1-\hat\weight) \cdot \beta^\star\bigg) - \beta^\star + \omega\hat \Delta_\lambda\bigg|^2 \\
    & = \bigg|\tilde \beta - \bigg(\hat\weight \cdot \beta_\obs + (1-\hat\weight) \cdot \beta^\star\bigg)\bigg|^2 + \hat\weight^2|\hat \Delta_\lambda - \Delta|^2 \\
    \label{eq:param_est_err_decomp}
    & \lesssim \bigg|\tilde \beta - \bigg(\hat\weight \cdot \beta_\obs + (1-\hat\weight) \cdot \beta^\star\bigg)\bigg|^2 + \bigg(\lambda^2 \cdot {\frac{\sigma_\rct^2}{n_\rct}}\bigg) \land \Delta^2,\numberthis
\end{align*}
where the last inequality happens with probability $1-e^{-\sfc \lambda^2} - o(1)$ by \eqref{eq:est_err_delta} and $\frac{\sigma_\rct^2}{n_\rct}\gtrsim \frac{\sigma_\obs^2}{n_{\obs}}$. On the event $\calE$, we have
\begin{align*}
    \hat\weight & =  \frac{\hat \sigma_\rct^2/n_\rct}{\hat \sigma_\rct^2/n_\rct + \hat\sigma_\obs^2/n_{\obs}} \in \Big[\frac{0.9\weight}{1.1} , \frac{1.1\weight}{0.9}\Big],\\
    1 - \hat\weight &  =  \frac{\hat \sigma_\obs^2/n_{\obs}}{\hat \sigma_\rct^2/n_\rct + \hat\sigma_\obs^2/n_{\obs}} \in \Big[\frac{0.9(1-\weight)}{1.1} , \frac{1.1(1-\weight)}{0.9}\Big].
\end{align*}    
Thus, on the event $\calE$, we can proceed by
\begin{align*}
    \bigg|\tilde \beta - \bigg(\hat\weight \cdot \beta_\obs + (1-\hat\weight) \cdot \beta^\star\bigg)\bigg|^2 
    & \lesssim (1-\weight)^2 |\hat\beta_\rct - \beta^\star|^2 + \weight^2 |\hat\beta_\obs - \beta_\obs|^2.
\end{align*}
Using Assumption \ref{assump:asymp_linear}, we write
\begin{align*}
    (1-\weight)|\hat\beta_\rct- \beta^\star| = (1-\weight) \cdot \bigg| \frac{1}{n_\rct}\sum_{i\in\Rct}\psi_{\rct, i} + o_p(n_\rct^{-1/2})\bigg|.
\end{align*}
By Berry-Esseen theorem (see Theorem \ref{thm:berry_esseen}), we have
$$
    \sup_{t\in\bbR} \bigg| \bbP\bigg(\frac{1}{n_\rct}\sum_{i\in\Rct}\psi_{\rct, i} \leq t \cdot \frac{\sigma_\rct}{\sqrt{n_\rct}}\bigg) - \Phi(t)\bigg| \leq \frac{6 \rho_\rct}{\sigma_\rct^3 \sqrt{n_\rct}},
$$
which further gives
$$
    \bbP\bigg(\frac{1}{n_\rct}\sum_{i\in\Rct}\psi_{\rct, i} \leq \lambda \cdot \frac{\sigma_\rct}{\sqrt{n_\rct}}\bigg) \geq 1 - \Phi(-\lambda)  - o(1) \geq 1 - \calO(e^{-\lambda^2/2}) - o(1),
$$
where the last inequality is by the Gaussian tail bound and $\lambda \gtrsim 1$.
The above display, along with $\lambda \gtrsim 1$, implies that with probability $1-e^{-\sfc \lambda^2} - o(1)$ for a potentially different absolute constant $\sfc >0$, we have
\begin{align*}
    (1-\weight)|\hat\beta_\rct- \beta^\star| 
    & \lesssim \lambda \cdot \frac{\sigma_\obs^2/n_{\obs}}{\sigma_\rct^2/n_\rct + \sigma_\obs^2/n_{\obs}} \cdot \frac{\sigma_\rct}{\sqrt{n_\rct}} \\
    & \leq \lambda \cdot \frac{\sigma_\obs^2/n_{\obs}}{\sigma_\rct^2/n_\rct} \cdot \frac{\sigma_\rct}{\sqrt{n_\rct}} \\
    & = \lambda \cdot \frac{\sigma_\obs}{\sqrt{n_{\obs}}} \cdot \sqrt{\frac{\sigma_\obs^2/n_{\obs}}{\sigma_\rct^2/n_\rct}} \\
    & \lesssim \lambda \cdot \frac{\sigma_\obs}{\sqrt{n_{\obs}}} \\
    & \lesssim \lambda \cdot \sqrt{\frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2}},
\end{align*}
where the last two inequalities are by $\sigma_\rct^2/n_\rct\gtrsim \sigma_\obs^2/n_{\obs}$. Using a nearly identical argument, we have
$$
    \bbP\bigg(\frac{1}{n_{\obs}}\sum_{i\in\Obs}\psi_{\obs, i} \leq \lambda \cdot \frac{\sigma_\obs}{\sqrt{n_{\obs}}}\bigg) \geq 1 - e^{-\sfc \lambda^2}-o(1),
$$
which further implies that,
\begin{align*}
    \weight |\hat\beta_\obs - \beta_\obs| 
    & \lesssim \lambda \cdot \frac{\sigma_\rct^2/n_\rct}{\sigma_\rct^2/n_\rct + \sigma_\obs^2/n_{\obs}} \cdot \frac{\sigma_\obs}{\sqrt{\sigma_\obs}} \\
    & \leq\lambda \cdot  \frac{\sigma_\obs}{\sqrt{\sigma_\obs}} \\
    & \lesssim \lambda \cdot \sqrt{\frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2}},
\end{align*}
where the last inequality is again by $\sigma_\rct^2/n_\rct\gtrsim \sigma_\obs^2/n_{\obs}$. A union bound then gives
$$
    \bigg|\tilde \beta - \bigg(\hat\weight \cdot \beta_\obs + (1-\hat\weight) \cdot \beta^\star\bigg)\bigg|^2  \lesssim \lambda^2\cdot \frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2}
$$
with probability $1-2 e^{-\sfc\lambda^2} - o(1)$. The proof is concluded by plugging the above display back to \eqref{eq:param_est_err_decomp}, invoking another union bound, and recalling that $\lambda\gtrsim 1$ and $|\Delta|\leq \overline\Delta$.






% \subsection{Proof of Equation \texorpdfstring{(\ref{eq:beta_obs_explicit_formula})}{}}\label{prf:eq:beta_obs_explicit_formula}
% For any $i\in\Obs$, we have
% \begin{align*}
% 	\bbE[Y_i~|~A_i = 1, \bfX_i] & = \bbE\bigg[ \bbE[Y_i(A_i) | A_i=1 , \bfX_i, U_i] ~\bigg|~ A_i=1, \bfX_i\bigg] \\
% 	& = \bbE[\beta^\star_\obs + U_i + \bsgamma_\obs^\top \bfX_i~|~ A_i=1, \bfX_i]\\
% 	& = \beta^\star_\obs + \bsgamma_\obs^\top \bfX_i + \bbP(U_i = 1 ~|~ A_i=1, \bfX_i) - \bbP(U_i = -1~|~A_i=1, \bfX_i).
% \end{align*}
% Note that
% \begin{align*}
% 	\bbP(U_i = 1 ~|~ A_i = 1, \bfX_i) & = \frac{\bbP(U_i = 1, A_i = 1 ~|~\bfX_i)}{\bbP(A_i = 1~|~\bfX_i)}\\
% 	& = \frac{\bbP(A_i=1~|~\bfX_i, U_i=1) \bbP(U_i=1~|~\bfX_i)}{\sum_{u\in\{\pm 1\}} \bbP(A_i=1~|~\bfX_i, U_i = u) \bbP(U_i = u~|~\bfX_i)} \\
% 	& = \frac{\pi_\obs(\bfX_i, 1)}{\pi_\obs(\bfX_i, 1) + \pi_\obs(\bfX_i, -1)},
% \end{align*}	
% where the last inequality is by $U_i\sim\textnormal{Rademacher}(1/2)$ and $U_i\indep \bfX_i$. Thus, we have
% $$
% 	\bbE[Y_i~|~ A_i = 1, \bfX_i] = \beta_\obs^\star + \bsgamma_\obs^\top \bfX_i + \frac{\pi_\obs(\bfX_i, 1) - \pi_\obs(\bfX_i, -1)}{\pi_\obs(\bfX_i, 1) + \pi_\obs(\bfX_i, -1)}.
% $$
% On the other hand, we have
% \begin{align*}
% 	\bbE[Y_i~|~A_i = 0, \bfX_i] & =   \bbE\bigg[ \bbE[Y_i(A_i) | A_i=0 , \bfX_i, U_i] ~\bigg|~ A_i=0, \bfX_i\bigg]  = \bbE[\bsgamma_\obs^\top \bfX_i ~|~ A_i = 0, \bfX_i] = \bsgamma_\obs^\top \bfX_i.
% \end{align*}
% % $$
% % 	\bbP(U_i = 1 ~|~ A_i = 0, \bfX_i)
% % 	= \frac{1- \pi_\obs(\bfX_i, 1)}{2 - \pi_\obs(\bfX_i, 1)- \pi_\obs(\bfX_i, -1)},
% % $$
% % which further gives
% % $$
% % 	\bbE[Y_i ~|~ A_i = 0, \bfX_i] = 
% % $$
% The proof is concluded by taking the difference of the above two displays and integrating over the randomness in $\bfX_i$.


\subsection{Proof of Theorem \ref{thm:oracle_ci}} \label{prf:thm:oracle_ci}
We first show the proposed oracle CI is asymptotically level $(1-\alpha)$. This conclusion is trivial for the $\overline\Delta \geq \sigma_\rct/\sqrt{n_\rct}$ case. When $\overline\Delta < \sigma_\rct/\sqrt{n_\rct}$, recall that we have shown in the proof of Theorem \ref{thm:oracle_estimator} that
$$
    {\hat\beta_\weight}\bigg/\bigg({\frac{\sigma_\rct\sigma_\obs}{\sqrt{n_\rct\sigma_\obs^2 + n_\obs\sigma_\rct^2}} }\bigg) \overset{d}{\to} N(0, 1).
$$
Hence, we have
$$
    \bbP\bigg( - \Phi^{-1}(1-\frac{\alpha}{2})\cdot \frac{\sigma_\rct\sigma_\obs}{\sqrt{n_\rct\sigma_\obs^2 + n_{\obs}\sigma_\rct^2}} + \hat\beta_\weight \leq (1-\weight)\beta^\star + \weight \beta_\obs \leq \hat\beta_\weight + \Phi^{-1}(1-\frac{\alpha}{2})\cdot \frac{\sigma_\rct\sigma_\obs}{\sqrt{n_\rct\sigma_\obs^2 + n_{\obs}\sigma_\rct^2}}\bigg) \geq 1 - \alpha - o(1).
$$
Since $\beta^\star = (1-\weight)\beta^\star + \weight \beta_\obs + \weight \Delta$ and $|\Delta|\leq \overline\Delta$, it follows that
\begin{align*}
    & \bbP\bigg( -\overline\Delta- \Phi^{-1}(1-\frac{\alpha}{2})\cdot \frac{\sigma_\rct\sigma_\obs}{\sqrt{n_\rct\sigma_\obs^2 + n_{\obs}\sigma_\rct^2}} + \hat\beta_\weight 
    \leq \beta^\star % (1-\weight)\beta^\star + \weight \beta_\obs 
    \leq \hat\beta_\weight + \Phi^{-1}(1-\frac{\alpha}{2})\cdot \frac{\sigma_\rct\sigma_\obs}{\sqrt{n_\rct\sigma_\obs^2 + n_{\obs}\sigma_\rct^2}} + \overline \Delta\bigg) \\
    & \geq \bbP\bigg( - \Phi^{-1}(1-\frac{\alpha}{2})\cdot \frac{\sigma_\rct\sigma_\obs}{\sqrt{n_\rct\sigma_\obs^2 + n_{\obs}\sigma_\rct^2}} + \hat\beta_\weight \leq (1-\weight)\beta^\star + \weight \beta_\obs \leq \hat\beta_\weight + \Phi^{-1}(1-\frac{\alpha}{2})\cdot \frac{\sigma_\rct\sigma_\obs}{\sqrt{n_\rct\sigma_\obs^2 + n_{\obs}\sigma_\rct^2}}\bigg)\\
    & \geq 1 - \alpha - o(1).
\end{align*} 
By construction, 
\begin{align*}
    \len([L_\alpha, U_\alpha])
     = 
    \begin{cases}
        2 \Phi^{-1}(1-\alpha/2) \frac{\sigma_\rct}{\sqrt{n_\rct}} & \textnormal{ if } \overline\Delta \geq \sigma_\rct/\sqrt{n_\rct} \\
        2 \Phi^{-1}(1-\alpha/2) \frac{\sigma_\rct\sigma_\obs}{\sqrt{n_\rct\sigma_\obs^2 + n_{\obs}\sigma_\rct^2}} + 2 \overline\Delta  & \textnormal{ otherwise}.
    \end{cases}
\end{align*}
As long as $\alpha \geq \ep\gtrsim 1$, we have $\Phi^{-1}(1-\alpha/2)\lesssim 1$. 
% Also, we have shown in the proof of Theorem \ref{thm:oracle_estimator} that $n_\obs \asymp n_{\obs}$ when $n_\obs \geq (1+\ep)n_\rct$. 
It follows that  
$$
    \len([L_\alpha, U_\alpha]) \lesssim \frac{\sigma_\rct\sigma_\obs}{\sqrt{n_\rct\sigma_\obs^2 + n_\obs\sigma_\rct^2}} + \frac{\sigma_\rct}{\sqrt{n_\rct}} \land \overline\Delta,
$$
and the proof is concluded by taking expectation at both sides.


\subsection{Proof of Theorem \ref{thm:minimax_adaptive_length}}\label{prf:thm:minimax_adaptive_length}
We first present two useful lemmas.
\begin{lemma}
    \label{lemma:minimax_length}
    Let $\pi_{\underline\Delta}$ and $\pi_{\overline\Delta}$ be prior distributions on $\calP_{\underline\Delta}$ and $\calP_{\overline\Delta}$, respectively. Let $f_{\pi_{\underline\Delta}}$ and $f_{\pi_{\overline\Delta}}$ be the marginal distribution of all the data, marginalized over $\pi_{\underline\Delta}$ and $\pi_{\overline\Delta}$, respectively.
    Assume the prior distributions are chosen so that $\beta^\star = \underline\beta$ under $\pi_{\underline\Delta}$ and $\beta^\star = \overline\beta$ under $\pi_{\overline\Delta}$. Then we have
    $$
        \len^\star_\alpha(\calP_{\underline\Delta}, \calP_{\overline\Delta}) \geq |\underline\beta - \overline\beta| \cdot \bigg[\bigg(1 - TV(f_{\pi_{\underline\Delta}}, f_{\pi_{\overline\Delta}}) - 2\alpha\bigg) \lor 0\bigg],
    $$
    where $TV(\cdot, \cdot)$ is the total variation distance.
\end{lemma}
\begin{proof}
    This is a direct corollary of Lemma 1 in \cite{cai2017confidence}.
\end{proof}

\begin{lemma}
    \label{lemma:tv_ineq}
    Let $X, Y, Z$ be random variables. Then
    $$
        TV(\textnormal{Law}(X), \textnormal{Law}(Y)) \leq \bbE_{Z}[TV(\textnormal{Law}(X|Z), \textnormal{Law}(Y|Z))].
    $$
\end{lemma}
\begin{proof}
    By definition, we have
    \begin{align*}
        TV(\textnormal{Law}(X), \textnormal{Law}(Y)) & = \sup_{\calE}|\bbP(X\in \calE) - \bbP(Y \in \calE)|\\
        & = \sup_{\calE} \bigg|\bbE_Z \bigg[\bbP(X\in\calE \mid Z) - \bbP(Y\in\calE \mid Z)\bigg] \bigg|\\
        & \leq \sup_{\calE} \bbE_Z \bigg| \bbP(X\in\calE \mid Z) - \bbP(Y\in\calE \mid Z)\bigg| \\
        & \leq \bbE_Z \sup_{\calE}\bigg| \bbP(X\in\calE \mid Z) - \bbP(Y\in\calE \mid Z)\bigg| \\
        & = \bbE_{Z}[TV(\textnormal{Law}(X|Z), \textnormal{Law}(Y|Z))],
    \end{align*}
    where the last two inequalities are by Jensen's inequality.
\end{proof}

We break the proof into three cases.

\paragraph{Case A. $\boldsymbol{\overline\Delta \geq \sigma_\rct/\sqrt{n_\rct}}$.}
In this case, we choose $\pi_{\underline\Delta}$ to be a point mass at $\beta^\star = 0, \beta_\obs = 0$ and we let $\pi_{\overline\Delta}$ be a point mass at $\beta^\star = \sigma_\rct/\sqrt{n_\rct}, \beta_\obs = 0$. By Lemmas \ref{lemma:minimax_length} and \ref{lemma:tv_ineq}, we have
\begin{align*}
    \len^\star_\alpha(\calP_{\underline\Delta}, \calP_{\overline\Delta}) 
    &\geq \frac{\sigma_\rct}{\sqrt{n_\rct}} \cdot \bigg[\bigg(1 - TV(f_{\pi_{\underline\Delta}}, f_{\pi_{\overline\Delta}}) - 2\alpha\bigg) \lor 0\bigg] \\
    & \geq \frac{\sigma_\rct}{\sqrt{n_\rct}} \cdot \bigg[\bigg( \bbE_{\{\bfX_i\}, \{A_i\}}[ 1 - TV(f_{\pi_{\underline\Delta}|\{\bfX_i\}, \{A_i\}}, f_{\pi_{\overline\Delta}|\{\bfX_i\}, \{A_i\}})] - 2\alpha\bigg) \lor 0\bigg],
\end{align*}
where $f_{\pi_{\underline\Delta}|\{\bfX_i\}, \{A_i\}}$ (resp.~$f_{\pi_{\overline\Delta}|\{\bfX_i\}, \{A_i\}}$) is the conditional distribution of $f_{\pi_{\underline\Delta}}$ (resp.~$f_{\pi_{\underline\Delta}}$) given $\{\bfX_i\}$ and $\{A_i\}$. 
By Neyman--Pearson lemma, the quantity $1 - TV(f_{\pi_{\underline\Delta}|\{\bfX_i\}, \{A_i\}}, f_{\pi_{\overline\Delta}|\{\bfX_i\}, \{A_i\}})$ is equal to the Type-I plus Type-II error of testing
$$
    H_0: \{Y_i\}\mid \{\bfX_i\}, \{A_i\} \sim f_{\pi_{\underline\Delta}|\{\bfX_i\}, \{A_i\}}
    ~~~
    \textnormal{v.s.}
    ~~~
    H_1: \{Y_i\}\mid \{\bfX_i\}, \{A_i\} \sim f_{\pi_{\overline\Delta}|\{\bfX_i\}, \{A_i\}},
$$
and the optimal test is given by the likelihood ratio test.
By construction, the likelihood function under $H_0$ is
\begin{align*}
    L_0 & = \bigg(\prod_{i\in\Rct, A_i = 1} \frac{1}{\sqrt{2\pi \sigma_\rct^2}} \exp\{-(Y_i - \bsgamma_\rct^\top \bfX_i)^2/(2\sigma_\rct^2)\}\bigg) \\
    & \qquad \times \bigg(\prod_{i\in\Rct, A_i = 0}\frac{1}{\sqrt{2\pi \sigma_\rct^2}} \exp\{-(Y_i - \bsgamma_\rct^\top \bfX_i)^2/(2\sigma_\rct^2)\}\bigg) \\
    & \qquad \times \bigg(\prod_{i\in\Obs, A_i = 1} \frac{1}{\sqrt{2\pi \sigma_\obs^2}} \exp\{-(Y_i -  \bsgamma_\obs^\top \bfX_i)^2/(2\sigma_\obs^2)\}\bigg) \\
    \label{eq:minimax_length_L0_caseA}
    & \qquad \times
    \bigg(\prod_{i\in\Obs, A_i = 0} \frac{1}{\sqrt{2\pi \sigma_\obs^2}} \exp\{-(Y_i -\bsgamma_\obs^\top \bfX_i)^2/(2\sigma_\obs^2)\}\bigg),\numberthis
\end{align*}    
whereas the likelihood function under $H_1$ is
\begin{align*}
    L_1 & = \bigg(\prod_{i\in\Rct, A_i = 1} \frac{1}{\sqrt{2\pi \sigma_\rct^2}} \exp\{-(Y_i - \sigma_\rct/(2\sqrt{n_\rct}) - \bsgamma_\rct^\top \bfX_i)^2/(2\sigma_\rct^2)\}\bigg) \\
    & \qquad \times \bigg(\prod_{i\in\Rct, A_i = 0}\frac{1}{\sqrt{2\pi \sigma_\rct^2}} \exp\{-(Y_i + \sigma_\rct/(2\sqrt{n_\rct}) - \bsgamma_\rct^\top \bfX_i)^2/(2\sigma_\rct^2)\}\bigg) \\
    & \qquad \times \bigg(\prod_{i\in\Obs, A_i = 1} \frac{1}{\sqrt{2\pi \sigma_\obs^2}} \exp\{-(Y_i -  \bsgamma_\obs^\top \bfX_i)^2/(2\sigma_\obs^2)\}\bigg) \\
    & \qquad \times
    \bigg(\prod_{i\in\Obs, A_i = 0} \frac{1}{\sqrt{2\pi \sigma_\obs^2}} \exp\{-(Y_i -\bsgamma_\obs^\top \bfX_i)^2/(2\sigma_\obs^2)\}\bigg).
\end{align*}    
The optimal test rejects $H_0$ in favor of $H_1$ when $L_1/L_0\geq 1$, which is equivalent to
\begin{align*}
    % \label{eq:minimax_length_opt_test_caseA}
    -\sum_{i\in\calC, A_i = 1} \bigg(2(Y_i - \gamma_\rct^\top \bfX_i) - \frac{\sigma_\rct}{2\sqrt{n_\rct}}\bigg) 
    + 
    \sum_{i\in\calC, A_i = 0} \bigg(2(Y_i - \gamma_\rct^\top \bfX_i) + \frac{\sigma_\rct}{2\sqrt{n_\rct}}\bigg)  \leq 0.
\end{align*} 
Under $H_0$, we have $Y_i-\gamma_\rct^\top \bfX_i \mid \bfX_i, A_i \overset{i.i.d.}{\sim} N(0, \sigma_\rct^2)$. Thus, the left-hand side above is distributed as
$
    N\left(\frac{\sigma_\rct \sqrt{n_\rct}}{2}, 4n_\rct\sigma_\rct^2\right),
$
and the type-I error is given by
$$
    \bbP\bigg( N\left(\frac{\sigma_\rct \sqrt{n_\rct}}{2}, 4n\sigma_\rct^2\right) \leq 0\bigg) = \Phi(-1/4).
$$
A nearly identical argument shows that the Type-II error is also given by $\Phi(-1/4)$.
Hence, we get
$$
    1 - TV(f_{\pi_{\underline\Delta}|\{\bfX_i\}, \{A_i\}}, f_{\pi_{\overline\Delta}|\{\bfX_i\}, \{A_i\}})] = 2 \Phi(-1/4),
$$
and it follows that
$$
    \len^\star_\alpha(\calP_{\underline\Delta}, \calP_{\overline\Delta}) 
    \geq 2\frac{\sigma_\rct}{\sqrt{n_\rct}} \cdot (\Phi(-1/4) - \alpha)\gtrsim \frac{\sigma_\rct}{\sqrt{n_\rct}},
$$
where the last inequality is by $\alpha \leq \Phi(-1/4)-\ep$.

\paragraph{Case B. $\boldsymbol{ 1/\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}\leq \overline \Delta \leq \sigma_\rct/\sqrt{n_\rct}}$.}
In this case, we choose $\pi_{\underline\Delta}$ to be a point mass at $\beta^\star =0, \beta_\obs = 0$, and we choose $\pi_{\overline\Delta}$ to be a point mass at $\beta^\star = \overline\Delta, \beta_\obs = 0$. By Lemmas \ref{lemma:minimax_length} and \ref{lemma:tv_ineq}, we have
\begin{align*}
    \len^\star_\alpha(\calP_{\underline\Delta}, \calP_{\overline\Delta}) 
    & \geq \overline\Delta \cdot \bigg[\bigg( \bbE_{\{\bfX_i\}, \{A_i\}}[ 1 - TV(f_{\pi_{\underline\Delta}|\{\bfX_i\}, \{A_i\}}, f_{\pi_{\overline\Delta}|\{\bfX_i\}, \{A_i\}})] - 2\alpha\bigg) \lor 0\bigg].
\end{align*}
Similar to Case A, we need to compute the optimal Type-I plus Type-II error of testing
$$
    H_0: \{Y_i\}\mid \{\bfX_i\}, \{A_i\} \sim f_{\pi_{\underline\Delta}|\{\bfX_i\}, \{A_i\}}
    ~~~
    \textnormal{v.s.}
    ~~~
    H_1: \{Y_i\}\mid \{\bfX_i\}, \{A_i\} \sim f_{\pi_{\overline\Delta}|\{\bfX_i\}, \{A_i\}}.
$$
The likelihood function under $H_0$ is given by \eqref{eq:minimax_length_L0_caseA}, and the likelihood function under $H_1$ is given by
\begin{align*}
    L_1 & = \bigg(\prod_{i\in\Rct, A_i = 1} \frac{1}{\sqrt{2\pi \sigma_\rct^2}} \exp\{-(Y_i - \overline\Delta/2 - \bsgamma_\rct^\top \bfX_i)^2/(2\sigma_\rct^2)\}\bigg) \\
    & \qquad \times \bigg(\prod_{i\in\Rct, A_i = 0}\frac{1}{\sqrt{2\pi \sigma_\rct^2}} \exp\{-(Y_i + \overline\Delta/2 - \bsgamma_\rct^\top \bfX_i)^2/(2\sigma_\rct^2)\}\bigg) \\
    & \qquad \times \bigg(\prod_{i\in\Obs, A_i = 1} \frac{1}{\sqrt{2\pi \sigma_\obs^2}} \exp\{-(Y_i -  \bsgamma_\obs^\top \bfX_i)^2/(2\sigma_\obs^2)\}\bigg) \\
    & \qquad \times
    \bigg(\prod_{i\in\Obs, A_i = 0} \frac{1}{\sqrt{2\pi \sigma_\obs^2}} \exp\{-(Y_i -\bsgamma_\obs^\top \bfX_i)^2/(2\sigma_\obs^2)\}\bigg).
\end{align*}    
The optimal test rejects $H_0$ in favor of $H_1$ when $L_1/L_0\geq 1$, which is equivalent to
\begin{align*}
    -\sum_{i\in\calC, A_i = 1} \bigg(2(Y_i - \gamma_\rct^\top \bfX_i) - {\overline\Delta}/{2}\bigg) 
    + 
    \sum_{i\in\calC, A_i = 0} \bigg(2(Y_i - \gamma_\rct^\top \bfX_i) +\overline\Delta/2\bigg)  \leq 0.
\end{align*} 
Under $H_0$, the left-hand side above is distributed as
$
N\left(\overline\Delta n_\rct/2, 4n_\rct \sigma_\rct^2\right),
$
and thus the type-I error is given by
$$
    \bbP\bigg(N\left(\overline\Delta n_\rct/2, 4n_\rct \sigma_\rct^2\right) \leq 0\bigg) = \Phi\bigg(-\frac{\overline\Delta}{4 \sigma_\rct/\sqrt{n_\rct}}\bigg) \geq \Phi(-1/4),
$$
where the last inequality is by $\overline\Delta \leq \sigma_\rct/\sqrt{n_\rct}$. A nearly identical argument shows that the type-I error is also lower bounded by $\Phi(-1/4)$. Thus, 
$$
1 - TV(f_{\pi_{\underline\Delta}|\{\bfX_i\}, \{A_i\}}, f_{\pi_{\overline\Delta}|\{\bfX_i\}, \{A_i\}})] \geq 2\Phi(-1/4),
$$
and
$$
    \len^\star_\alpha(\calP_{\underline\Delta}, \calP_{\overline\Delta}) 
    \geq 2 \overline\Delta \cdot (\Phi(-1/4) - \alpha)\gtrsim \overline\Delta,
$$
where the last inequality is by $\alpha \leq \Phi(-1/4)-\ep$.

\paragraph{Case C. $\boldsymbol{\overline\Delta \leq 1/\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}}$.}
In this case, we let $\pi_{\underline\Delta}$ be a point mass at $\beta^\star = 0, \beta_\obs = 0$ and $\pi_{\overline\Delta}$ be a point mass at $\beta^\star = \frac{1}{\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}}, \beta_\obs = \frac{1}{\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}}$.
By Lemmas \ref{lemma:minimax_length} and \ref{lemma:tv_ineq}, we have
\begin{align*}
    \len^\star_\alpha(\calP_{\underline\Delta}, \calP_{\overline\Delta}) 
    & \geq \frac{1}{\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}} \cdot \bigg[\bigg( \bbE_{\{\bfX_i\}, \{A_i\}}[ 1 - TV(f_{\pi_{\underline\Delta}|\{\bfX_i\}, \{A_i\}}, f_{\pi_{\overline\Delta}|\{\bfX_i\}, \{A_i\}})] - 2\alpha\bigg) \lor 0\bigg].
\end{align*}
Similar to the previous two cases, we need to compute the optimal Type-I plus Type-II error of testing
$$
    H_0: \{Y_i\}\mid \{\bfX_i\}, \{A_i\} \sim f_{\pi_{\underline\Delta}|\{\bfX_i\}, \{A_i\}}
    ~~~
    \textnormal{v.s.}
    ~~~
    H_1: \{Y_i\}\mid \{\bfX_i\}, \{A_i\} \sim f_{\pi_{\overline\Delta}|\{\bfX_i\}, \{A_i\}}.
$$
The likelihood function under $H_0$ is given by \eqref{eq:minimax_length_L0_caseA}, and the likelihood function under $H_1$ is given by
\begin{align*}
    L_1 & = \bigg(\prod_{i\in\Rct, A_i = 1} \frac{1}{\sqrt{2\pi \sigma_\rct^2}} \exp\{-(Y_i - (2\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2})^{-1} - \bsgamma_\rct^\top \bfX_i)^2/(2\sigma_\rct^2)\}\bigg) \\
    & \qquad \times \bigg(\prod_{i\in\Rct, A_i = 0}\frac{1}{\sqrt{2\pi \sigma_\rct^2}} \exp\{-(Y_i + (2\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2})^{-1} - \bsgamma_\rct^\top \bfX_i)^2/(2\sigma_\rct^2)\}\bigg) \\
    & \qquad \times \bigg(\prod_{i\in\Obs, A_i = 1} \frac{1}{\sqrt{2\pi \sigma_\obs^2}} \exp\{-(Y_i - (2\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2})^{-1} -  \bsgamma_\obs^\top \bfX_i)^2/(2\sigma_\obs^2)\}\bigg) \\
    & \qquad \times
    \bigg(\prod_{i\in\Obs, A_i = 0} \frac{1}{\sqrt{2\pi \sigma_\obs^2}} \exp\{-(Y_i + (2\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2})^{-1} -\bsgamma_\obs^\top \bfX_i)^2/(2\sigma_\obs^2)\}\bigg).
\end{align*}
The optimal test rejects $H_0$ in favor of $H_1$ when $L_1/L_0\geq 1$. With some algebra, such a test rejects $H_0$ in favor of $H_1$ when
\begin{align*}
    & \frac{-1}{\sigma_\rct^2} \sum_{i\in\Rct, A_i = 1} \bigg(2(Y_i - \gamma_\rct^\top \bfX_i) - \frac{1}{2 \sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}}\bigg)
    + 
    \frac{1}{\sigma_\rct^2} \sum_{i\in\Rct, A_i = 0} \bigg(2(Y_i - \gamma_\rct^\top \bfX_i) + \frac{1}{2 \sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}}\bigg) \\
    & ~ -\frac{1}{\sigma_\obs^2} \sum_{i\in\Obs, A_i = 1} \bigg(2(Y_i - \gamma_\obs^\top \bfX_i) - \frac{1}{2 \sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}}\bigg) 
    + \frac{1}{\sigma_\obs^2} \sum_{i\in\Obs, A_i = 0} \bigg(2(Y_i + \gamma_\obs^\top \bfX_i) - \frac{1}{2 \sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}}\bigg)\\
    & \leq 0.
\end{align*}
The left-hand side above is distributed as
$$
    \frac{1}{\sigma_\rct^2} \cdot N\bigg(\frac{n_\rct}{2\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}}, 4 n_\rct \sigma_\rct^2\bigg) \Conv
    \frac{1}{\sigma_\obs^2} \cdot N\bigg(\frac{n_\obs}{2\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}}, 4 n_\obs \sigma_\obs^2\bigg),
$$
where $\conv$ denotes the convolution of random variables. Thus, the type-I error is given by
\begin{align*}
    & \bbP\bigg[ \frac{n_\rct/\sigma_\rct^2}{2\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}} +  \frac{n_\obs/\sigma_\obs^2}{2\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}} + \bigg(\frac{2\sqrt{n_\rct}}{\sigma_\rct} \cdot N(0, 1)\bigg)\Conv\bigg(\frac{2\sqrt{n_\obs}}{\sigma_\obs} \cdot N(0, 1)\bigg)\leq 0 \bigg]\\
    & = \bbP\bigg[ \frac{\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}}{2} + 2 \cdot N \bigg(0, \frac{n_\rct}{\sigma_\rct^2} + \frac{n_\obs}{\sigma_\obs^2}\bigg)\leq 0\bigg] \\
    & = \Phi(-1/4).
\end{align*}
A nearly identical argument shows that the type-I error is also lower bounded by $\Phi(-1/4)$. Thus, 
$$
    \len^\star_\alpha(\calP_{\underline\Delta}, \calP_{\overline\Delta}) 
    \geq 2 \frac{1}{\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}} \cdot (\Phi(-1/4) - \alpha)\gtrsim \frac{1}{\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}},
$$
where the last inequality is by $\alpha \leq \Phi(-1/4)-\ep$.

\paragraph{Finishing the proof.}
Combining the above three cases, we get 
$$
    \len^\star_\alpha(\calP_{\underline\Delta}, \calP_{\overline\Delta})  \gtrsim \frac{1}{\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}} \lor \bigg(\frac{\sigma_\rct}{\sqrt{n_\rct}} \land \overline\Delta\bigg) 
    \asymp \frac{1}{\sqrt{n_\rct/\sigma_\rct^2 + n_\obs/\sigma_\obs^2}} +  \frac{\sigma_\rct}{\sqrt{n_\rct}} \land \overline\Delta,
$$
and the proof is finished.

\newpage
\section{Additional Simulation Results}\label{appx:more_simulation}
\begin{table}[ht]
\centering
\caption{Ratios of the mean squared error of each estimator to that of the oracle estimator $\widehat{\beta}_\weight$ when $n_o = 50,000$. Estimators considered in the table are the RCT-only estimator $\widehat{\beta}_c$, the observational-data-only estimator $\widehat{\beta}_o$, and the anchored thresholding estimator $\widehat{\beta}_{\lambda}$.% with $\lambda = \lambda_1 \cdot \sqrt{\log(n_c\land n_{o_2})}$.
}
% \label{tbl: extra simulation results}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccccc}
  
 &$\hat\beta_c$ & $\hat\beta_o$ &\multicolumn{2}{c}{$\hat\beta_{\lambda}$} & $\hat\beta_c$ & $\hat\beta_o$ &\multicolumn{2}{c}{$\hat\beta_{\lambda}$}\\
 \hline\hline
   \multicolumn{9}{c}{$\beta(X_1, X_2, X_3) = 2$} \\
   \hline
 \multirow{2}{*}{\begin{tabular}{c}b\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{IPW}\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{IPW}\end{tabular}} 
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.5$\end{tabular}}
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.6$\end{tabular}}
    &\multirow{2}{*}{\begin{tabular}{c}\textsf{AIPW}\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{AIPW}\end{tabular}} 
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.5$\end{tabular}}
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.6$\end{tabular}}
  \\  
  \\
  
   0.00 & 30.54 & 1.00 & 4.49 & 2.78 & 24.50 & 1.02 & 3.51 & 2.24 \\ 
   0.01 & 28.76 & 1.05 & 3.77 & 2.33 & 25.40 & 1.06 & 3.58 & 2.22 \\ 
  0.10 & 9.10 & 1.07 & 1.85 & 1.40 & 7.14 & 1.08 & 1.59 & 1.28 \\ 
   0.50 & 1.00 & 1.95 & 1.16 & 1.30 & 1.00 & 2.73 & 1.41 & 1.64 \\ 
   0.60 & 1.00 & 3.08 & 1.51 & 1.80 & 1.00 & 4.21 & 1.73 & 2.13 \\ 
   0.70 & 1.00 & 3.91 & 1.83 & 2.21 & 1.00 & 5.29 & 2.05 & 2.51 \\ 
   2.00 & 1.00 & 14.37 & 2.37 & 3.16 & 1.00 & 20.16 & 2.44 & 3.26 \\ 
  3.00 & 1.00 & 18.21 & 2.42 & 3.24 & 1.00 & 23.89 & 2.30 & 3.06 \\ 
  10.00 & 1.00 & 22.61 & 2.48 & 3.32 & 1.00 & 32.11 & 2.53 & 3.39 \\  
  \hline\hline
   \multicolumn{9}{c}{$\beta(X_1, X_2, X_3) = 2 - X_1 - X_2$} \\
   \hline

\multirow{2}{*}{\begin{tabular}{c}b\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{IPPW}\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{IPW}\end{tabular}} 
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.5$\end{tabular}}
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.6$\end{tabular}}
    &\multirow{2}{*}{\begin{tabular}{c}\textsf{AIPPW}\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{AIPW}\end{tabular}} 
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.5$\end{tabular}}
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.6$\end{tabular}}
  \\  \\  
   0.00 & 27.78 & 1.03 & 3.76 & 2.33 & 24.19 & 1.01 & 3.56 & 2.28 \\ 
   0.01 & 25.44 & 1.01 & 3.40 & 2.11 & 21.77 & 1.01 & 3.02 & 1.95 \\ 
   0.10 & 8.82 & 1.07 & 1.73 & 1.32 & 6.71 & 1.07 & 1.51 & 1.23 \\ 
   0.50 & 1.00 & 2.14 & 1.23 & 1.41 & 1.00 & 2.97 & 1.48 & 1.75 \\ 
   0.60 & 1.00 & 2.76 & 1.49 & 1.73 & 1.00 & 3.78 & 1.73 & 2.09 \\ 
   0.70 & 1.00 & 3.91 & 1.77 & 2.15 & 1.00 & 5.03 & 1.86 & 2.31 \\ 
   2.00 & 1.00 & 12.53 & 2.36 & 3.08 & 1.00 & 17.67 & 2.38 & 3.12 \\ 
   3.00 & 1.00 & 18.79 & 2.44 & 3.28 & 1.00 & 26.05 & 2.51 & 3.37 \\ 
   10.00 & 1.00 & 21.66 & 2.45 & 3.27 & 1.00 & 29.74 & 2.35 & 3.13 \\ 
\end{tabular}}
\end{table}


\begin{table}[ht]
\centering
\caption{Ratios of the mean squared error of each estimator to that of the oracle estimator $\widehat{\beta}_\weight$ when $n_o = 100,000$. Estimators considered in the table are the RCT-only estimator $\widehat{\beta}_c$, the observational-data-only estimator $\widehat{\beta}_o$, and the anchored thresholding estimator $\widehat{\beta}_{\lambda}$.% with $\lambda = \lambda_1 \cdot \sqrt{\log(n_c\land n_{o_2})}$.
}
% \label{tbl: simulation results}
\resizebox{\textwidth}{!}{ 
\begin{tabular}{ccccccccccc}
 &$\hat\beta_c$ & $\hat\beta_o$ &\multicolumn{2}{c}{$\hat\beta_{\lambda}$} & $\hat\beta_c$ & $\hat\beta_o$ &\multicolumn{2}{c}{$\hat\beta_{\lambda}$}\\
 \hline\hline
   \multicolumn{9}{c}{$\beta(X_1, X_2, X_3) = 2$} \\
   \hline
 \multirow{2}{*}{\begin{tabular}{c}b\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{IPW}\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{IPW}\end{tabular}} 
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.5$\end{tabular}}
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.6$\end{tabular}}
    &\multirow{2}{*}{\begin{tabular}{c}\textsf{AIPW}\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{AIPW}\end{tabular}} 
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.5$\end{tabular}}
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.6$\end{tabular}}
  \\  \\
  
   0.00 & 28.75 & 1.04 & 3.70 & 2.26 & 24.32 & 1.04 & 3.46 & 2.23 \\ 
   0.01 & 30.02 & 1.05 & 3.99 & 2.39 & 25.30 & 1.05 & 3.66 & 2.33 \\ 
  0.10 & 8.65 & 1.08 & 1.62 & 1.25 & 6.37 & 1.09 & 1.40 & 1.17 \\ 
   0.50 & 1.00 & 2.20 & 1.21 & 1.41 & 1.00 & 3.09 & 1.52 & 1.79 \\ 
   0.60 & 1.00 & 2.77 & 1.42 & 1.68 & 1.00 & 3.76 & 1.66 & 2.02 \\ 
   0.70 & 1.00 & 3.59 & 1.67 & 2.00 & 1.00 & 4.90 & 1.87 & 2.31 \\ 
   2.00 & 1.00 & 14.05 & 2.30 & 3.07 & 1.00 & 19.78 & 2.34 & 3.13 \\ 
   3.00 & 1.00 & 16.92 & 2.22 & 2.96 & 1.00 & 22.69 & 2.20 & 2.92 \\ 
   10.00 & 1.00 & 21.80 & 2.48 & 3.30 & 1.00 & 30.30 & 2.45 & 3.26 \\  \hline\hline 
   \multicolumn{9}{c}{$\beta(X_1, X_2, X_3) = 2 - X_1 - X_2$} \\ \hline

\multirow{2}{*}{\begin{tabular}{c}b\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{IPPW}\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{IPW}\end{tabular}} 
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.5$\end{tabular}}
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.6$\end{tabular}}
    &\multirow{2}{*}{\begin{tabular}{c}\textsf{AIPPW}\end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}{c}\textsf{AIPW}\end{tabular}} 
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.5$\end{tabular}}
   & \multirow{2}{*}{\begin{tabular}{c}$\lambda_1=0.6$\end{tabular}}
  \\  \\  
    0.00 & 28.75 & 1.04 & 3.70 & 2.26 & 24.32 & 1.04 & 3.46 & 2.23 \\ 
   0.01 & 30.02 & 1.05 & 3.99 & 2.39 & 25.30 & 1.05 & 3.66 & 2.33 \\ 
   0.10 & 8.65 & 1.08 & 1.62 & 1.25 & 6.37 & 1.09 & 1.40 & 1.17 \\ 
   0.50 & 1.00 & 2.20 & 1.21 & 1.41 & 1.00 & 3.09 & 1.52 & 1.79 \\ 
   0.60 & 1.00 & 2.77 & 1.42 & 1.68 & 1.00 & 3.76 & 1.66 & 2.02 \\ 
   0.70 & 1.00 & 3.59 & 1.67 & 2.00 & 1.00 & 4.90 & 1.87 & 2.31 \\ 
   2.00 & 1.00 & 14.05 & 2.30 & 3.07 & 1.00 & 19.78 & 2.34 & 3.13 \\ 
   3.00 & 1.00 & 16.92 & 2.22 & 2.96 & 1.00 & 22.69 & 2.20 & 2.92 \\ 
  10.00 & 1.00 & 21.80 & 2.48 & 3.30 & 1.00 & 30.30 & 2.45 & 3.26 \\
\end{tabular}}
\end{table}





==> combining clinical and observational datasets/history/02-setup_old2.tex <==
%!TEX root = 00-main.tex
\section{Set-up}
\textcolor{red}{We have approx 5 pages in set-up/review of two biases. We may want to trim it to three pages and put the rest to the supplement.}
\label{sec: setup}
\subsection{Notation, estimands and baseline estimators}
Suppose the existence of a binary treatment $ A\in \{0,1\} $, potential outcomes $\{Y(1), Y(0)\}$ and baseline observed covariates $\mathbf{X}$. 
We assume consistency so that the observed outcome $Y$ satisfies $Y= AY(1) + (1-A)Y(0)$. 
Our estimand of interest is the average treatment effect of the target population (PATE):
\begin{equation*}
    % \label{eq:PATE}
     \beta^\ast = \mathbb{E}[Y{(1)} - Y{(0)}],
\end{equation*}
where $\mathbb{E}[\cdot]$ is taken with respect to the joint distribution of $\{\mathbf{X}, Y(0), Y(1)\}$ over the target population. A random sample of size $n_c$ from the target population was selected into a RCT according to some sample selection protocol. 
We use $S = c$ to indicate selection into the RCT and let $\mathcal{C}$ denote the associated index set so that $|\mathcal{C}| = n_c$. Write the RCT data as \textcolor{red}{We may want to write less important expressions inline.}
\begin{equation*}
    \mathcal{D}_{c} = \{(Y_i, A_i, \mathbf{X}_i, S_i = c):~i \in \mathcal{C}\},
\end{equation*}
and denote the average treatment effect in the RCT population as
\begin{equation*}
    \beta^\ast_{c} = \mathbb{E}[Y(1) - Y(0) \mid S = c],
\end{equation*}
where $\mathbb{E}[\cdot]$ is taken with respect to the conditional joint distribution of $\{\mathbf{X}, Y(0), Y(1) \mid S = c\}$, i.e., over the RCT population. 
Assume that the data in $\mathcal{D}_{c}$ are independent and identically distributed according to the joint law of $\big(Y(1), Y(0), A, \mathbf{X}\big) \mid S = c$ and let $\pi_c(\mathbf{x}) = \bbP(A = 1 \mid \mathbf{X}=\mathbf{x}, S = c)>0$ denote the \emph{known} treatment assignment probability in the RCT. 
The average treatment effect in the RCT population $\beta^\ast_c$ is then identified from $\mathcal{D}_c$ and can be estimated via the following inverse probability weighting (IPW) estimator \citep{horvitz1952generalization}:
\begin{equation}
\label{eq:cipw}
\hat\beta_{c, \textsf{IPW}}  = \frac{1}{n_c} \sum_{i\in \mathcal{C}}  \bigg(\frac{A_i Y_i }{\pi_c(\mathbf{X}_i)} - \frac{(1-A_i) Y_i }{1- \pi_c(\mathbf{X}_i)}\bigg).
\end{equation}
Another estimator that is also commonly considered is the regression imputation or g-formula estimator, which fits a conditional outcome mean model for each treatment arm and then marginalizes over the RCT samples \citep{robins1986}. Because it is in general not fully robust to misspecification of the outcome-covariate relationship and thus does not exploit the full advantage of RCTs, this is not further considered in this article. \textcolor{red}{We may want to move some standard stuff into supplement.}


Alternatively, $\beta^\ast_c$ can be estimated via the following augmented inverse probability weighting (AIPW) estimator \citep{robins1994estimation, bang2005doubly} 
\begin{align*}
% \begin{split}
\hat\beta_{c, \textsf{AIPW}}
&  = \frac{1}{n_c} \sum_{i\in \mathcal{C}}\bigg(\frac{A_i (Y_i -\mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} ) )  }{\pi_c(\mathbf{X}_i)} - \frac{(1-A_i)(Y_i -\mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ) ) }{1- \pi_c(\mathbf{X}_i)} \\
\label{eq:caipw}
& \qquad \qquad \qquad +\mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} )   - \mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} )\bigg),\numberthis
% \end{split}
\end{align*}
where $ \mu_{ca}(\bfx; \bsalpha_{ca} ),a = 0, 1,$ are parametric specifications (parametrized by $\bsalpha_{c0}$ and $\bsalpha_{c1}$, respectively) of the conditional outcome means $\mu_{ca}(\bfx) = \mathbb{E}[Y \mid \bfX=\bfx, A = a, S = c]$ and $ \hat \bsalpha_{ca} $ are estimators of $ \bsalpha_{ca}$. 
In an RCT with known $\pi_c(\bfx)$, the AIPW estimator $ \hat\beta_{c, \textsf{AIPW}}$ is robust in the sense that it consistently estimates $\beta^\ast_c$ even when the parametric outcome regression models $\mu_{ca} (\bfx; \bsalpha_{ca})$ do not correctly specify $\mu_{ca}(\bfx)$ for $a = 0, 1$ (\citealp{bang2005doubly,tsiatis2007semiparametric}). 
Besides robustness, AIPW also enjoys desirable efficiency properties.
It is locally efficient if $\mu_{ca} (\bfx; \bsalpha_{ca})$ correctly specifies $\mu_{ca}(\bfx)$. 
It is also guaranteed to be more efficient than $\hat\beta_{c, \textsf{IPW}}$ when $\pi_c(\bfx)$ does not depend on the covariate vector $\bfx$ (i.e., random treatment assignment),  $\mu_{ca}(\bfx; \bsalpha_{ca})$ are linear parametric models of $\mu_{ca}(\bfx)$, and $ \hat \bsalpha_{ca}$ are the corresponding least squares estimators (\citealp{tsiatis2008covariate}). 

In parallel, a random sample of size $n_o$ from the target population was collected in an observational study, which is typically of a much larger size compared to the RCT. We use $S = o$ to indicate selection into the observational study and let $\mathcal{O}$ denote the associated index set so that $|\mathcal{O}| = n_o$. 
Write the observational data as
\begin{equation*}
    \mathcal{D}_{o} = \{(Y_i, A_i, \mathbf{X}_i, S_i = o):~i \in \mathcal{O}\}
\end{equation*}
and define the average treatment effect in the observational study population as
\begin{equation*}
    \beta^\ast_{o} = \mathbb{E}[Y(1) - Y(0) \mid S = o],
\end{equation*}
where $\mathbb{E}[\cdot]$ is taken with respect to the conditional joint distribution of $\big(\mathbf{X}, Y(0), Y(1) \big)\mid S = o$. Assume that the data in $\mathcal{D}_{o }$ are independent and identically distributed according to the joint law of $\big(Y(1), Y(0), A, \mathbf{X}\big) \mid S = o$.  
% According to Assumption \ref{assump: observational is target} stated later in Section \ref{subsec: external validity}, the observational study population is the same as the target population, so we have $\beta_o^\ast= \beta^\ast$.

Let $\pi_{o}(\bfx) = \bbP(A = 1 \mid \mathbf{X} = \bfx, S = o)>0$ denote the treatment assignment probability in the observational data, i.e., the propensity score (\citealp{rosenbaum1983central}), $\mu_{oa}(\bfx) = \mathbb{E}[Y \mid \mathbf{X}=\bfx, A = a, S = o]$ the conditional outcome means in the observational data, and  $\pi_{o}(\bfx; \bseta)$ and $\mu_{oa}(\bfx;  \bsalpha_{oa})$ their corresponding parametric specifications. The counterparts of $\cipw$ and $\caipw$ defined in \eqref{eq:cipw} and \eqref{eq:caipw} can then be formed as
\begin{align}
\label{eqn:oipw}
	\hat\beta_{o, \textsf{IPW}} &= \frac{1}{n_o} \sum_{i\in \mathcal{O}}  \bigg(\frac{A_i Y_i }{\pi_{o}(\mathbf{X}_i; \hat \bseta)} - \frac{(1-A_i) Y_i }{1- \pi_{o}(\mathbf{X}_i; \hat \bseta) }\bigg) ,\\
		\hat	\beta_{o, \textsf{AIPW}} &=  \frac{1}{n_o} \sum_{i\in \mathcal{O}}\bigg(\frac{A_i (Y_i -\mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} ) )  }{\pi_{o}(\mathbf{X}_i; \hat\bseta )} - \frac{(1-A_i)(Y_i -\mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} ) ) }{1- \pi_{o}(\mathbf{X}_i;\hat\bseta)}  \nonumber\\
\label{eqn:oaipw}
        & \qquad \qquad\qquad + \mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} )   - \mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} )\bigg),
\end{align}
where $\hat\bseta$ and $\hat\bsalpha_{oa}$ are estimates of $\bseta$ and $\bsalpha_{oa}$, respectively. 

Note that without further assumptions, neither $\beta^\star_\rct$ nor $\beta^\star_\obs$ agrees with our estimand of interest $\beta^\star$.

\subsection{Internal validity bias}
\label{subsec: internal validity}
Internal validity refers to an effect estimate being (asymptotically) unbiased for the causal effect. 
Constructing estimators that the internally valid for the RCT population (i.e., can consistently estimate $\beta^\star_\rct$) is a relatively easy task.
In particular, the following assumption holds by design.

\begin{assumption}[Design of RCT]\label{assump: design of RCT} \rm
For the RCT population, we assume $A \perp (Y(1), Y(0)) \mid \mathbf{X}, S=c$, the treatment assignment probability $ \pi_c(\mathbf{x}):= P(A=1\mid \mathbf{X}=\mathbf{x}, S=c) $ is known, and $\pi_c(\mathbf{X})>0$ with probability 1 with respect to the law of $\bfX\mid S = c$. 
\end{assumption}
Assumption \ref{assump: design of RCT} states that the treatment assignment in the RCT population is manipulated by the experimenter and depends only on the observed covariates. 
Under Assumption \ref{assump: design of RCT} and usual identification assumptions of consistency and the Stable Unit Treatment Value Assumption (SUTVA) (\citealp{Rubin1980}), both $\hat\beta_{c, \textsf{IPW}}$ and $\hat\beta_{c, \textsf{AIPW}}$ defined in \eqref{eq:cipw} and \eqref{eq:caipw} are internally valid: they are consistent and asymptotically normal estimators for the causal estimand $\beta^{\ast}_c$. 


On the other hand, constructing internally valid estimators for the observational population is typically an impossible task due to confounding bias from unobserved covariates. 
Consequently, the two estimators $\hat\beta_{o, \textsf{IPW}}$ and $\hat\beta_{o, \textsf{AIPW}}$ defined in \eqref{eqn:oipw} and \eqref{eqn:oaipw} are not necessarily estimating $\beta^\ast_o$, the causal estimand defined based on the observational data. 

To further understand how the internal validity bias arises from unobserved covariates, we consider an unmeasured confounder $U$ such that the treatment assignment becomes ignorable once conditional on $(\mathbf{X}, U)$ \citep{rosenbaum1983central, rosenbaum1983sens, Imbens2003}, i.e., $ A  \indep ( Y(1), Y(0)) \mid \mathbf{X}, U, S=o$ but $ A \nindep ( Y(1), Y(0)) \mid \mathbf{X}, S=o$. 
Meanwhile, we make the following standard positivity assumption.
\begin{assumption}[Positivity of Treatment Assignment in Observational Study]\label{assump: positivity obs} 
Assume the treatment assignment probability $\pi_o(\mathbf{X}):= P(A=1\mid \bfX, S=o)>0$ with probability 1 with respect to the law of $\bfX \mid S = \obs$.
\end{assumption}
Under the above assumption, even when $\pi_o(\mathbf{x}; \bseta)$ and $\mu_{oa}(\mathbf{x}; \bsalpha_{oa})$ correctly specify  $\pi_o(\mathbf{x})$ and $\mu_{oa}(\mathbf{x})$, the estimators $ \hat\beta_{o, \textsf{IPW}}$ and $\hat\beta_{o, \textsf{AIPW}}$ are still estimating a non-causal quantity 
$$
\beta_o=\mathbb{E}\left[Y\mid  S = o, A=1\right] - \mathbb{E}\left[Y\mid  S = o, A=0\right],
$$
because they fail to adjust for the presence of $U$. 

The difference between the causal $\beta^\ast_o$ and the non-causal counterpart $\beta_{o}$ takes the following form (see Appendix \textcolor{red}{XX} for a detailed derivation):
\begin{align*}
% \begin{split}
  \Delta  =\beta^\ast_{o} - \beta_{o}
  &=  \mathbb{E}\left[ \frac{(1-A) Y\pi_{o}(\mathbf{X})}{1-\pi_{o}(\mathbf{X})} \left\{  1-\gamma(\mathbf{X}, U)  \right\}  \mid S= o \right]\\
  \label{eqn: Obs data internal validity bias}
  & \qquad - \mathbb{E}\left[ \frac{AY(1-\pi_{o}(\mathbf{X}))}{\pi_{o}(\mathbf{X})  } \left\{   1- \frac{1}{\gamma (\mathbf{X}, U)}  \right\}  \mid S= o \right], \numberthis
% \end{split}
\end{align*}
where $\gamma(\mathbf{X}, U)$ represents the odds ratio of the true propensity score $\pi_{o}(\mathbf{X}, U) = P(A= 1 \mid \mathbf{X}, U, S = o)$ that takes into account the unobserved covariate $U$ and the observed propensity score $\pi_{o}(\mathbf{X}) = \bbP(A = 1 \mid \mathbf{X}, S = o)$, i.e.,
\begin{equation*}
  \gamma(\mathbf{X}, U)
  % = \text{OR} \{\pi_{o}(\mathbf{X}, U), \pi_{o}(\mathbf{X}) \} 
  = \frac{\pi_{o}(\mathbf{X}, U)/[1-\pi_{o}(\mathbf{X}, U)]}{\pi_{o}(\mathbf{X})/[1- \pi_{o}(\mathbf{X})]}. 
\end{equation*}
Namely, $\Delta$ measures the internal validity bias from the observational data. 
There are other ways to parametrize and represent the bias $\Delta$. Our method and theory developed in Section \ref{sec: method} does \emph{not} depend on the particular parametrization or the correct specification of the nuisance models $\pi_o(\mathbf{x})$ and $\mu_{oa}(\mathbf{x})$. 
In other words, the estimator based on the observational data can have arbitrary bias. 




\subsection{External validity bias}
\label{subsec: external validity}
External validity is concerned with how well the effect estimates generalize to other contexts \citep{degtiar2021review}.
It can arise from various sources, such as the difference in subject characteristics, study setting, etc.
% \citet{degtiar2021review} discussed multiple sources of external validity bias (e.g., difference in subject characteristics, study setting, etc); we focus on the bias arising from the variation in sample selection probability, the treatment effect heterogeneity, and the interplay between these two factors. 
To have a fine-grained characterization of the external validity bias, one need to specify the target population of interest.

In the main manuscript, we focus on the setting where the observational data represent our target population, as formalized in the following assumption.
\begin{assumption}[Target Population]\label{assump:target}
Assume 
% either one of the following holds:
% \begin{itemize}
    % \item[(a)] The RCT data represent the target population, so that $(\mathbf{X}, Y(0), Y(1)\mid S=c) \overset{d}{=} ( \mathbf{X}, Y(0), Y(1))$;
    % \item[(b)] 
    $\bbE[Y(a)\mid \bfX, S = \obs] = \bbE[Y(a)\mid \bfX]$ for any $a\in\{0, 1\}$.
% \end{itemize}
\end{assumption}

It is clear that under the above assumption, we have $\beta^\star = \beta^\star_\obs$.
% , wheres under the latter setting, we have $\beta^\star = \beta^\star_\obs$.
% Either setting could be of interest to the investigator.
% The latter 
Such a setting is prevalent in practice, as participants in RCT are typically highly selected and thus the population it represents can differ significantly from the ultimate population of interest.
We remark that our method and theory developed in Section \ref{sec: method} can be extended in a \emph{mutatis mutandis} fashion to accommodate other settings, such as when the RCT data represent the target population, or even when there is a separate target population that is distinct from either RCT or observational data. For ease of exposition, we defer the discussion of such extensions to Appendix \ref{appx:rct_as_target}.

% In contrast, the former setting is relevant when the investigator is interested only in the subjects with a particular set of characteristics.
% Before proceed further, we remark that our method and theory developed in Section \ref{sec: method} could be extended in a \emph{mutatis mutandis} fashion to handle the case where there is a separate target population that is different from the population represented by either the RCT or the observational data. But we do not pursue this direction in this article. 
% \paragraph{The observational population is the target.}
When the observational data represent the target population, the two RCT-based estimators, namely $\cipw$ and $\caipw$, albeit being internally valid, do not converge to the correct target $\beta^\star$ asymptotically.
Fortunately, their external validity bias can be eliminated under the following \emph{conditional mean exchangeability} assumption, also known as the \emph{generalizability} assumption \citep{Stuart:2011aa, Dahabreh:2019aa, degtiar2021review}. 

\begin{assumption}[Conditional Mean Exchangeability]\label{assump: study selection exchangeability}
For any $a\in\{0, 1\}$, assume
$\mathbb{E}[Y(a) \mid \mathbf{X}, S = c] = \mathbb{E}[Y(a) \mid \mathbf{X}]$.
\end{assumption}
The above assumption states that participating in the RCT does not affect the potential outcome means and is a standard assumption that allows for generalizing the causal estimand in the RCT population to the target population.
Under this assumption, the PATE $\beta^\star$ can be identified from the RCT data via inverse probability weighting on the participation probability $e_\rct(\bfx) = \bbP(S = \rct\mid \bfX =\bfx, S \in \{\rct, \obs\})$, where we use $S \in \{\rct, \obs\}$ to indicate that the probability is taken with respect to the law of $\bfX$ marginalized over the RCT and the observational data.

In practice, the participation probability $e_\rct$ is unknown and thus must be estimated from the data. To make this task possible, we impose the following assumption.
% In Assumption \ref{assump: bdd density ratio}, we also require common support of the observed covariates with respect to study selection.
\begin{assumption}[Bounded Density Ratio]\label{assump: bdd density ratio}
Assume $\bbP(\mathbf{X}= \mathbf{x}\mid S=o) / \bbP( \mathbf{X}= \mathbf{x} \mid S=c)<\infty$ for all $\mathbf{x}$ with positive density with respect to the law of $(\bfX \mid S \in \{\rct, \obs\})$. 
\end{assumption}

%\begin{assumption}[Decaying Probability of Selection into RCT]\label{assump: sample selection positivity for Obs}\rm
%$P(S = s \mid \mathbf{X} = \mathbf{x}) > 0$ for $s = o, t$, and every $\mathbf{x}$ with positive density. 
%\end{assumption}
 
%Recall that $\beta_o$ denotes the probability limit of the observational studies estimators $\hat\beta_{o, \textsf{IPW}}$ and $\hat\beta_{o, \textsf{AIPW}}$ in \eqref{eqn: IPW and AIPW for obs}. The bias of both estimators with respect to the target parameter $\beta^\ast$ can be decomposed into an internal validity bias term and an external validity bias term as follows:
%\begin{equation}
%\begin{split}
%    \Delta := \beta_o - \beta^\ast = \underbrace{\beta_o- \beta^\ast_o}_{\text{internal validity bias}} + \underbrace{\beta^\ast_o - \beta^\ast}_{\text{external validity bias}}.
%\end{split}
%\end{equation}

%In the absence of the internal validity bias, one may eliminate the external validity bias by adopting an inverse probability of participation weighting (IPPW) or augmented inverse probability of participation weighting (AIPPW) approach (\citealp{Stuart:2011aa, Dahabreh:2019aa}) and form the following re-weighted estimators:
%\begin{align*}
%\hat\beta_{o, \textsf{IPPW}}  &= \frac{1}{n_t} \sum_{i\in \mathcal{O}} \bigg[ \frac{A_i Y_i }{\pi_{o}(\mathbf{X}_i; \hat\bseta)} - \frac{(1-A_i) Y_i }{1- \pi_{o}(\mathbf{X}_i;\hat\bseta)}\bigg] \frac{ e_{{t}}(\mathbf{X}_i; \hat \omega_{{t}} )  }{e_{{o}}(\mathbf{X}_i; \hat \omega_{{c}} )    }\\
%\hat\beta_{o, \textsf{AIPPW}}   & = \frac{1}{n_t} \sum_{i\in \mathcal{O}} \bigg[\frac{A_i (Y_i -\mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} ) )  }{\pi_{o}(\mathbf{X}_i; \hat\bseta)} - \frac{(1-A_i)(Y_i -\mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} ) ) }{1- \pi_{o}(\mathbf{X}_i; \hat\bseta)}  \bigg] \frac{ e_{{t}}(\mathbf{X}_i; \hat \omega_{{t}} ) }{e_{{o}}(\mathbf{X}_i; \hat \omega_{{c}} )  } \\
%&\qquad + \frac{1}{n_t} \sum_{i\in \mathcal{T}} \mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} )   - \mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} ).
%\end{align*}

%In the above display, $\pi_o > 0$ for all $\mathbf{x}$ by the treatment assignment positivity assumption in observational study and $e_o > 0$ for all $\mathbf{x}$ by Assumption \ref{assump: sample selection positivity for Obs}. In the finite sample, both estimators may be unstable as weights may be very close to $0$ for some $\mathbf{x}$. To alleviate this issue, one may further adopt a stabilized version of both estimators.

%In the presence of the internal validity bias, both IPPW and AIPPW estimators change the covariate distribution over which the internal validity bias is evaluated and there is no decisive conclusion whether inverse participation probability weighting would mitigate or amplifies the internal validity bias of $\hat\beta_{o, \textsf{IPW}}$ or $\hat\beta_{o, \textsf{AIPW}}$.


Commonly in existing works, the positivity of RCT participation (i.e., $\bbP(S=c\mid \mathbf{X}=\mathbf{x}, S\in \{o_1,c\} )$ is strictly bounded away from zero and one almost surely) is imposed \citep{Stuart:2011aa, Dahabreh:2019aa, lu2019causal, degtiar2021review}. Under positivity of RCT participation, plus Assumptions \ref{assump:target} and \ref{assump: study selection exchangeability}, \citet{Stuart:2011aa} and \citet{Dahabreh:2019aa} showed that one can adopt an inverse probability of participation weighting (IPPW) or augmented inverse probability of participation weighting (AIPPW) approach to generalize the RCT-based estimators to the target population.

However, the positivity of RCT participation is much stronger than Assumption \ref{assump: bdd density ratio} and almost never hold in practice. 
To see this, let us note that the observational data is typically of a much larger size compared to the RCT (this is also why we would like to use the observational data despite its potential internal validity bias).
The fact that $n_\obs\gg n_\rct$ signifies that the RCT participation probability must decay to zero as the sample size goes to infinity, and thus the positivity of RCT participation is naturally violated.

Our Assumption \ref{assump: bdd density ratio} does not assume away decaying probability of RCT participation. 
One approach to tackle this challenge is to use the technique developed in \cite{zhang2021double}. However, their estimation procedure is complicated and the convergence rate of the resulting estimator is typically slower than $n_c^{-1/2}$. 
In this article, we propose a simple procedure that restores the usual $n_c^{-1/2}$ rate: we randomly sample a subset of size $n_c$ from the observational data, denoted as $\mathcal{D}_{\mathcal{O}_1}$, then we use $\mathcal{D}_{\mathcal{C}}\cup\mathcal{D}_{\mathcal{O}_1} $ to
 adjust for the external validity bias of the RCT-based estimators using IPPW or AIPPW. This leads to the following RCT-based estimators for PATE $\beta^* = \beta^\star_\obs$:
\begin{align*}
\begin{split}
    \hat\beta_{c, \textsf{IPPW}}  &= \frac{1}{n_c} \sum_{i\in \mathcal{C}} \bigg[ \frac{A_i Y_i }{\pi_c(\mathbf{X}_i)} - \frac{(1-A_i) Y_i }{1- \pi_c(\mathbf{X}_i)}\bigg] \frac{ 1-e_{{c}}(\mathbf{X}_i; \hat \xi )  }{e_{{c}}(\mathbf{X}_i; \hat \xi )    },\\
\hat\beta_{c, \textsf{AIPPW}}   & = \frac{1}{n_c} \sum_{i\in \mathcal{C}} \bigg[\frac{A_i (Y_i -\mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} ) )  }{\pi_c(\mathbf{X}_i)} - \frac{(1-A_i)(Y_i -\mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ) ) }{1- \pi_c(\mathbf{X}_i)}  \bigg] \frac{ 1-e_{{c}}(\mathbf{X}_i; \hat \xi )  }{e_{{c}}(\mathbf{X}_i; \hat \xi )  } \\
&\qquad + \frac{1}{n_c} \sum_{i\in \mathcal{O}_1} \mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} )   - \mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ),
\end{split}
\end{align*}
where $e_{{c}}(\mathbf{x};  \xi )$ is a parametric specification of the ground truth participation probability $e_\rct(\bfx)$, and $\hat\xi$ is an estimator of $\xi$ obtained from $\mathcal{D}_{\mathcal{C}}\cup\mathcal{D}_{\mathcal{O}_1} $. 
It can be shown that when $e_{{c}}(\mathbf{X}_i; \xi )$ is correct, the probability limit of $\hat\beta_{c, \textsf{IPPW}} $ is $\beta^\star_\obs = \beta^\star$; when either  $e_{{c}}(\mathbf{X}_i; \xi )$ or $ \{\mu_{c1} (\mathbf{X}_i;  \bsalpha_{c1} ),  \mu_{c0} (\mathbf{X}_i;  \bsalpha_{c0} )\}$ is correct,  the probability limit of $\hat\beta_{c, \textsf{AIPPW}} $ is $\beta^\star_\obs = \beta^\star$. 

We use the remaining observational data $\mathcal{D}_{\mathcal{O}_2} = \mathcal{D}_{\mathcal{O}}\setminus\mathcal{D}_{\mathcal{O}_1}$ to construct the observational-data-based estimators $\hat\beta_{o_2,\textsf{IPW}}$ and $\hat\beta_{o_2,\textsf{AIPW}}$, whose formal definitions are given below: 
\begin{align*}
    	\hat\beta_{o_2, \textsf{IPW}} &= \frac{1}{n_{o_2} } \sum_{i\in \mathcal{O}_2}  \bigg(\frac{A_i Y_i }{\pi_{o}(\mathbf{X}_i; \hat \bseta)} - \frac{(1-A_i) Y_i }{1- \pi_{o}(\mathbf{X}_i; \hat \bseta) }\bigg) ,\\
		\hat	\beta_{o_2, \textsf{AIPW}} &=  \frac{1}{n_{o_2}} \sum_{i\in \mathcal{O}_2}\bigg(\frac{A_i (Y_i -\mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} ) )  }{\pi_{o}(\mathbf{X}_i; \hat\bseta )} - \frac{(1-A_i)(Y_i -\mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} ) ) }{1- \pi_{o}(\mathbf{X}_i;\hat\bseta)} \\
        & \qquad \qquad \qquad + \mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} )   - \mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o1} )\bigg),
\end{align*}
where (with slight abuse of notation) $\hat\bseta$ and $\hat\bsalpha_{oa}$ are estimators of $\bseta$ and $\bsalpha_{oa}$ obtained from $\mathcal{D}_{\mathcal{O}_2}$. 
Under Assumption \ref{assump:target}(b), the two estimators given above do not suffer from external validity bias, and their only source of bias is the internal validity bias $\Delta_\inter$.
% \begin{assumption}[Observational/Target Population]\label{assump: observational is target}
% $\bbP(\mathbf{X}, Y(0), Y(1)\mid S=o) = \bbP( \mathbf{X}, Y(0), Y(1))$. 
% \end{assumption}

It is well know that IPW-type estimators like $\cippw, \caippw, \ooipw$, and $\ooaipw$ can be unstable when the (estimated) weights are close to zero. To alleviate this issue, one can apply the stabilization method by normalizing the weights to sum to 1 \citep{robins2007comment}.  For example, the stabilized version of $\caippw$ is 
\begin{align*}
        \hat\beta_{c, \textsf{sAIPPW}} &= \bigg[  \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{A_i(1-e_{{c}}(\mathbf{X}_i; \hat \xi )) }{\pi_c(\mathbf{X}_i)e_{{c}}(\mathbf{X}_i; \hat \xi ) }\bigg]^{-1} \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{A_i(1-e_{{c}}(\mathbf{X}_i; \hat \xi )) (Y_i -\mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} ) )  }{\pi_c(\mathbf{X}_i)e_{{c}}(\mathbf{X}_i; \hat \xi ) } \\
        & \qquad - \bigg[  \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{(1-A_i)(1-e_{{c}}(\mathbf{X}_i; \hat \xi ))}{(1- \pi_c(\mathbf{X}_i))e_{{c}}(\mathbf{X}_i; \hat \xi )} \bigg]^{-1}\frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{(1-A_i)(1-e_{{c}}(\mathbf{X}_i; \hat \xi ))(Y_i -\mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ) ) }{(1- \pi_c(\mathbf{X}_i))e_{{c}}(\mathbf{X}_i; \hat \xi )}   \\
         \label{eqn: c,sAIPPW}
&\qquad + \frac{1}{n_c} \sum_{i\in \mathcal{O}_1} \mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} )   - \mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ). \numberthis
\end{align*}
% Finally, it is well know that estimators like $\hat\beta_{o_2, \textsf{IPW}}, \hat\beta_{o_2, \textsf{AIPW}}, \hat\beta_{c, \textsf{IPPW}},$ and $ \hat\beta_{c, \textsf{AIPPW}}$ can be unstable when the treatment assignment and study selection probability $\pi_o(\mathbf{x}), 1-\pi_o(\mathbf{x}),$ and $ e_c(\mathbf{x})$, or their parametric specifications are close to 0 for some $\mathbf{x}$. To alleviate this issue, one can apply the stabilization method by normalizing the weights to sum to 1 \citep{robins2007comment}.  For example, the stabilized RCT-based AIPPW estimator $\hat\beta_{c, \textsf{sAIPPW}}$ is 
% \begin{align} \label{eqn: c,sAIPPW}
% \begin{split}
%     	\hat\beta_{c, \textsf{sAIPPW}} &= \bigg[  \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{A_i(1-e_{{c}}(\mathbf{X}_i; \hat \xi )) }{\pi_c(\mathbf{X}_i)e_{{c}}(\mathbf{X}_i; \hat \xi ) }\bigg]^{-1} \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{A_i(1-e_{{c}}(\mathbf{X}_i; \hat \xi )) (Y_i -\mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} ) )  }{\pi_c(\mathbf{X}_i)e_{{c}}(\mathbf{X}_i; \hat \xi ) } \\
%     	& \qquad - \bigg[  \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{(1-A_i)(1-e_{{c}}(\mathbf{X}_i; \hat \xi ))}{(1- \pi_c(\mathbf{X}_i))e_{{c}}(\mathbf{X}_i; \hat \xi )} \bigg]^{-1}\frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{(1-A_i)(1-e_{{c}}(\mathbf{X}_i; \hat \xi ))(Y_i -\mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ) ) }{(1- \pi_c(\mathbf{X}_i))e_{{c}}(\mathbf{X}_i; \hat \xi )}   \\
% &\qquad + \frac{1}{n_c} \sum_{i\in \mathcal{O}_1} \mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} )   - \mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ); 
% \end{split}
% \end{align}
and the stabilized AIPW estimator version of $\ooaipw$ is given by 
\begin{align*}
% \begin{split}
    	\hat\beta_{o_2, \textsf{sAIPW}} &=
    	\bigg[\frac{1}{n_{o_2}} \sum_{i\in \mathcal{O}_2}\frac{A_i  }{\pi_{o}(\mathbf{X}_i; \hat\bseta )} \bigg]^{-1}\frac{1}{n_{o_2}} \sum_{i\in \mathcal{O}_2} \frac{A_i (Y_i -\mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} ) )  }{\pi_{o}(\mathbf{X}_i; \hat\bseta )}  \\
    	& \qquad - \bigg[\frac{1}{n_{o_2}} \sum_{i\in \mathcal{O}_2}\frac{1-A_i  }{1-\pi_{o}(\mathbf{X}_i; \hat\bseta )} \bigg]^{-1}\frac{1}{n_{o_2}} \sum_{i\in \mathcal{O}_2}\frac{(1-A_i)(Y_i -\mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} ) ) }{1- \pi_{o}(\mathbf{X}_i;\hat\bseta)}\\
         \label{eqn: o2,sAIPW}
        &    \qquad   +\frac{1}{n_{o_2}} \sum_{i\in \mathcal{O}_2} \mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} )   - \mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} ). \numberthis
% \end{split}
\end{align*}
Note that the stabilized estimators are asymptotically equivalent to their unstabilized counterparts. \textcolor{red}{give ref?}
The consistency, asymptotic normality, and influence function representation of the introduced estimators are standard and can be immediately obtained from \citet[Chapter 6.1]{newey1994}. 
In the following, because of their appealing properties, we will use $\hat\beta_{c, \textsf{sAIPPW}}$ defined in \eqref{eqn: c,sAIPPW} and  $\hat\beta_{o_2, \textsf{sAIPW}}$ defined in \eqref{eqn: o2,sAIPW} as our default estimators, and we write $\hat \beta_\rct = \hat\beta_{c, \textsf{sAIPPW}}, \hat\beta_{\obs} = \hat\beta_{o_2, \textsf{sAIPW}}$  for notational simplicity.




% \begin{table}[]
% \centering
% \begin{tabular}{lll}
% Target population      & RCT & OBS \\ \hline
% Sources of bias for RCT-based estimators & None    &   External  \\
% Sources of bias for OBS-data-based estimators &  Internal+External   &    Internal \\
% Recommended RCT-based estimators          &   $\csaipw$  &  $\csaippw$   \\
% Recommended OBS-based estimators          &  $\osaipw$   &   $\oosaipw$  \\ \hline
% \end{tabular}
% \caption{Sources of bias and recommended choice of estimators based on the target population.}
% \label{table:choice_of_estimators}
% \end{table}


% Table \ref{table:choice_of_estimators} summarizes the sources of bias and the recommended choice of RCT-based and observational-data-based estimators for the PATE $\beta^\star$ based on the target population.










==> combining clinical and observational datasets/history/04-method_old.tex <==
%!TEX root = 00-main.tex

\section{Methodology}
\label{sec: method}
\subsection{An oracle procedure and its optimality}
% Let $\hat \beta_\rct$ be a generic estimator constructed using the RCT data and let $\hat \beta_\obs$ be another generic estimator constructed using the observational data. 
We have seen in Section \ref{subsec: external validity} that despite the presence of external validity bias, it is possible (under relatively weak assumptions) for $\hat\beta_\rct = \hat\beta_{c, \textsf{sAIPPW}}$ to consistently estimate the ground truth PATE $\beta^\star$.
In contrast, as demonstrated in Section \ref{subsec: internal validity}, constructing an estimator that consistently estimates $\beta^\star$ is in general impossible due to the potential internal validity bias in the observational data.
Rather, the best one could hope is the convergence of $\hat\beta_\obs = \hat\beta_{o_2, \textsf{sAIPW}}$ to some $\beta_\obs$ that is close to $\beta^\star$,
% Note that $\hat\beta_\rct$ (resp. $\hat\beta_\obs$) is unbiased for $\beta^\star_\rct$ (resp. $\beta_\obs$), and let $\sigma^2_\rct$ (resp. $\sigma^2_\obs$) be the asymptotic variance of $\hat\beta_\rct$ (resp. $\hat\beta_\obs$). 
and the discrepancy is quantified by
$$
\Delta =  \beta^\star - \beta_\obs.
$$

If the data analyst has prior knowledge on the magnitude of $\Delta$, a natural attempt to combine the two estimators (or two data sources) is to taking their convex combination:
\begin{equation}
	\label{eq:cvx_comb}
	\hat \beta_\weight := (1-\weight)  \hat\beta_\rct + \weight \hat\beta_\obs,
\end{equation}
where the weight $\omega$ may depend on $\Delta$.
Indeed, if $\Delta$ is excessively large, then incorporating the observational data can only hurt the performance of the final estimator, and the optimal strategy in this case is arguably only using the RCT data, i.e., setting $\omega = 0$.
In the other extreme, if $\Delta$ is negligibly small, then the optimal strategy becomes pooling the two data sources together (with proper weighting to adjust for the covariate shift). When $\hat\beta_\rct$ and $\hat \beta_\obs$ both admit asymptotic linear expansions, this pooling strategy corresponds to setting $\omega$ to a non-zero value that depends on the sample sizes.

In this subsection, we give a precise analysis on the performance of the estimator \eqref{eq:cvx_comb}.
 % and demonstrates its minimax optimality under a toy causal model. 
Unsurprisingly, the optimal choice of $\omega$ indeed depends on $\Delta$, rendering \eqref{eq:cvx_comb} an oracle procedure that is barely applicable in practice.
Nevertheless, such an analysis is still meaningful in that it serves as a benchmark on the rate of convergence we shall aim for when we design data-adaptive procedures in Section \ref{subsec: adaptive_procedure}.

\paragraph{The asymptotic mean squared error of $\boldsymbol{\hat \beta_\omega}$.}
% To keep the analysis versatile, 
We assume both $\hat\beta_\rct$ and $\hat\beta_\obs$ admit asymptotic linear expansions, as detailed below.
\begin{assumption}[Existence of asymptotic linear expansions]
\label{assump:asymp_linear}
Suppose there exist influence functions $\psi_\rct(X, A, Y)$, $\psi_\obs(X, A, Y)$ such that as $n_\rct \land n_{\obs_2} \to \infty$,
\begin{align*}
	\sqrt{n_\rct}(\hat\beta_\rct - \beta^\star) &  = \frac{1}{\sqrt{n_\rct}} \sum_{i\in \Rct}  \psi_\rct(\bfX_i, A_i, Y_i) +  o_p(1),\\
	\sqrt{n_{\obs_2}}(\hat\beta_\obs - \beta_\obs) &  = \frac{1}{\sqrt{n_{\obs_2}}} \sum_{i\in\Obs_2}  \psi_\obs(\bfX_i, A_i, Y_i) +  o_p(1).
\end{align*}
Moreover, the influence functions are mean zero with finite second and third moments given by
\begin{align*}
	\bbE[(\psi_\rct(\bfX_i, A_i, Y_i))^2] & = \sigma_\rct^2, \qquad
	\bbE[|\psi_\rct(\bfX_i, A_i, Y_i)|^3] = \rho_\rct, \qquad \forall i \in \Rct,\\
	\bbE[(\psi_\obs(\bfX_i, A_i, Y_i))^2] & = \sigma_\obs^2, \qquad
	\bbE[|\psi_\obs(\bfX_i, A_i, Y_i)|^3] = \rho_\obs, \qquad \forall i \in \Obs_2.
\end{align*}	
\end{assumption}
Based on the exposition in Section \ref{subsec: internal validity} and \ref{subsec: external validity}, the above assumption is satisfied by our default estimators $\hat \beta_\rct = \hat\beta_{c, \textsf{sAIPPW}}, \hat\beta_{\obs} = \hat\beta_{o_2, \textsf{sAIPW}}$.
We remark that there are other estimators for which the above assumption holds and our analysis is versatile enough to accommodate them. 

We assume the existence of finite third moments because our analysis takes advantage of Berry-Essen theorem. 
While this assumption could be relaxed, e.g., by invoking generalizations of Berry-Esseen theorem that only requires finite fractional moment \citep[Chapter 16]{feller2008introduction}, we do not pursue it in the current manuscript.

The following theorem characterizes the asymptotic mean squared error of $\hat\beta_\omega$.
\begin{theorem}[Performance of the oracle estimator]
\label{thm:amse_convex_comb}
Under Assumption \ref{assump:asymp_linear}, the estimator $\hat\beta_\weight$ satisfies
\begin{equation}
	\label{eq:amse_convergence_convex_comb}
	\sup_{\weight\in[0, 1]} \bigg|\frac{\bbE[|\hat\beta_\weight - \beta^\star|^2]}{\amse(\hat\beta_\weight)} - 1\bigg| \to 0 \qquad \textnormal{as }  n_\rct \land n_{\obs_2} \to \infty,
\end{equation}	
where the asymptotic mean squared error is given by
\begin{equation}
	\label{eq:amse_formula_convex_comb}
	\amse(\hat\beta_\weight) = 
	\frac{(1-\weight)^2 \sigma_\rct^2}{n_\rct} + \frac{\weight^2 \sigma_\obs^2}{n_{\obs_2}} + \weight^2\Delta^2.
\end{equation}	
Meanwhile, the optimal weight is given by
$
	\weight^\star = \frac{\sigma_\rct^2/n_\rct}{\sigma_\rct^2/n_\rct + \sigma_\obs^2/n_{\obs_2} + \Delta^2},
$
in which case the optimal asymptotic mean squared error becomes
\begin{equation}
	\label{eq:opt_amse_convex_comb}
	\min_{\weight\in[0, 1]} \amse(\hat\beta_\weight) = \amse(\hat\beta_{\weight^\star}) = \frac{\sigma_\rct^2}{n_\rct} \cdot \frac{\sigma_\obs^2 / n_{\obs_2} + \Delta^2}{\sigma_\rct^2/n_\rct + \sigma_\obs^2/n_{\obs_2} + \Delta^2}.
\end{equation}	
\end{theorem}
\begin{proof}
	See Appendix \ref{prf:thm:amse_convex_comb}.
\end{proof}

The optimal weight $\omega^\star$ is a function of $\Delta$ with a form that well matches our intuition. If $\Delta$ is large, then $\omega^\star$ is close to zero, meaning the optimal convex combination is close to using $\hat\beta_\rct$ alone. If $\Delta$ is small, then $\omega^\star$ becomes a function of the noise levels and the effective sample sizes. In the latter case, if we additionally assume $\sigma_\obs^2/n_{\obs_2} \ll \sigma_\rct^2/n_\rct$ (i.e., the observational data are much more abundant than the RCT data), then $\weight^\star$ is close to $1$, meaning that the optimal convex combination is close to using $\hat\beta_\obs$ alone.

The following proposition re-expresses the rate of convergence \eqref{eq:opt_amse_convex_comb} into a more interpretable form.
\begin{proposition}[Alternative representation for the optimal \amse]
\label{prop:amse_convex_comb_alt_formula}
	Assume $\sigma_\rct^2/n_\rct \gtrsim \sigma_\obs^2/n_{\obs}$ and $n_\obs \geq (1+\ep)n_\rct$ for some absolute constant $\ep > 0$ (i.e., the observational data are more abundant than the RCT data), then 
	\begin{equation}
		\label{eq:amse_convex_comb_alt_formula}
		\amse(\hat\beta_{\weight^\star}) \asymp \frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} + \frac{\sigma_\rct^2}{n_\rct} \land \Delta^2 
		\asymp
		\begin{cases}
			\frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} & \textnormal{if } \Delta^2 \lesssim \frac{\sigma_\rct^2}{n_\rct}
			\\[5pt]
			\frac{\sigma_\rct^2}{n_\rct} &  \textnormal{ if} \Delta^2 \gtrsim \frac{\sigma_\rct^2}{n_\rct}
		\end{cases}
	\end{equation}	
\end{proposition}
\begin{proof}
	See Appendix \ref{prf:prop:amse_convex_comb_alt_formula}. 
\end{proof}
The formula \eqref{eq:amse_convex_comb_alt_formula} gives a characterization on the role of $\Delta$ in the asymptotic mean squared error of $\hat\beta_{\weight^\star}$. 
When $\Delta^2 \lesssim \sigma_\rct^2/n_\rct$, the right-hand side of \eqref{eq:amse_convex_comb_alt_formula} becomes $\Theta\left(\frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2}\right)$, a rate that is of the same order as $\amse(\beta_{\hat\omega^\star})$ \emph{as if} $\Delta = 0$.
When $\Delta^2 \gtrsim \sigma_\rct^2/n_\rct$, then the right-hand side of \eqref{eq:amse_convex_comb_alt_formula} becomes $\Theta\left(\frac{\sigma_\rct^2}{n_\rct}\right)$, a rate  that is of the same order as $\amse(\hat \beta_{\omega^\star})$ \emph{as if} $\Delta = \infty$.
Recall that when $\Delta = 0$, the estimator $\hat \beta_{\omega^\star}$ is constructed essentially by pooling the two data sources together, whereas when $\Delta = \infty$, it is constructed by using $\hat\beta_\rct$ alone.
Disregarding the constant factors, the above proposition gives a curious phase transition between two extreme strategies: if $\Delta^2\lesssim \sigma_\rct^2/n_\rct$, then pooling the two data sources together can achieve the same performance as the optimal convex combination $\hat\beta_{\weight^\star}$; if $\Delta^2\gtrsim \sigma_\rct^2/n_\rct$, then using the RCT data alone can achieve the same performance as $\hat\beta_{\weight^\star}$.
Such a phase transition has been identified in other statistical problems that involve multiple data sources \citep{chen2021theorem}.




Curious readers may wonder if the rate \eqref{eq:amse_convex_comb_alt_formula}, achieved by the best convex combination, is information-theoretically optimal among all algorithms.
In fact, we can construct a simple data-generating process, under which \emph{any} algorithm that attempts to estimate $\beta^\star$ must suffer from a mean-squared error of order $\Omega\left( \frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} + \frac{\sigma_\rct^2}{n_\rct} \land \Delta^2\right)$. This confirms the minimax optimality of the best convex combination. For brevity, we defer the lower bound arguments to Appendix \ref{appx:lb}.




\subsection{An adaptive procedure: NAME}\label{subsec: adaptive_procedure}
% We consider an algorithm that achieves the same rate as the best convex combination.
% Notably this algorithm does not require a correct specification of $\Delta = \beta_\rct^\star - \beta^\star_\rct|$.
In this section, we design a fully adaptive estimator and prove that it achieves nearly the same performance as the best convex combination $\hat\beta_{\weight^\star}$, up to poly-log factors.

We start by constructing an preliminary estimator that pools all the data together:
$$
	\tilde \beta : =  (1-\hat\weight) \hat\beta_\rct + \hat\weight  \hat \beta_\obs, \qquad \hat \weight = \frac{\hat \sigma_\rct^2/n_\rct}{\hat \sigma_\rct^2/n_\rct + \sigma_\obs^2/n_{\obs_2}},
$$
where $\hat\sigma_\rct$ and $\hat\sigma_\obs$ are estimators of $\sigma_\rct$ and $\sigma_\obs$, respectively.
Since $\beta_\obs \neq \beta^\star$, the above estimator is biased, and the magnitude of the bias is $\hat \weight |\Delta|$.
We then try to de-bias $\tilde\beta$ by estimating $\Delta$. 
A natural estimator is given by
$$
	\tilde \Delta = \hat \beta_\rct - \hat \beta_\obs.
$$
If we use the above estimator to de-bias $\tilde \beta$, the final estimator would be $\hat\beta = \tilde \beta + \hat\weight\tilde\Delta$, i.e., we get back to $\hat\beta_\rct$, leading to no efficiency gain. Thus, we need more work.

Let us make two observations. First, we know that $\tilde \Delta$, after a proper scaling, is asymptotically Gaussian as $n_\rct \land n_{\obs_2}\to\infty$, and the asymptotic mean and variance of $\tilde \Delta$ are given by $\Delta$ and ${\sigma_\rct^2}/{n_\rct} + {\sigma_\obs^2}/{n_{\obs_2}}$, respectively. A standard concentration of measure argument gives that $|\Delta - \tilde \Delta| \lesssim \sqrt{\log(n_\rct \land n_{\obs_2}) \cdot ({\sigma_\rct^2}/{n_\rct} + {\sigma_\obs^2}/{n_{\obs_2}})}$ with high probability.
Second, we know that to potentially take advantage of the observational data, we need $\Delta$ to be relatively small. The above two observations motivate the following procedure:
% This looks like estimating a sparse Gaussian signal, so we can use Lasso-type algorithms to adapt to unknown $\Delta$. More concretely, let us consider
\begin{equation}
	\label{eq:est_delta}
    \hat \Delta = \argmin_{\delta} |\delta| \qquad \textnormal{subject to } |\delta - \tilde \Delta| \leq \sfc \sqrt{\log (n_\rct\land n_{\obs_2})} \cdot
    \sqrt{\frac{\hat\sigma_\rct^2}{n_\rct} + \frac{\hat\sigma_\obs^2}{n_{\obs_2}}},
\end{equation} 
where $\sfc > 0$ is a hyperparameter. Intuitively, the above procedure selects a $\hat\Delta$ with the minimum absolute value (based on our second observation), among all ``plausible'' candidates, where the ``plausibility'' is quantified by our first observation.

Such a procedure is reminiscent of many well-known methods in high-dimensional statistics, such as the Dantzig selector in sparse linear models \citep{candes2007dantzig} and nuclear norm minimization in matrix completion \citep{candes2009exact,candes2010power}, where one seeks for an estimator that minimizes certain complexity measures (in our case, the absolute value) subject to a constraint that ensures the error control.

Note that \eqref{eq:est_delta} can be solved via soft-thresholding: 
$$
	\hat \Delta = 
	\begin{cases}
		\textnormal{sgn}(\tilde \Delta) \cdot \bigg(|\tilde \Delta| - \sfc \sqrt{\log (n_\rct\land n_{\obs_2})} \cdot
    	\sqrt{\frac{\hat\sigma_\rct^2}{n_\rct} + \frac{\hat\sigma_\obs^2}{n_{\obs_2}}}\bigg)
    	& \textnormal{ if } 
    	|\tilde \Delta| \geq \sfc \sqrt{\log (n_\rct\land n_{\obs_2})} \cdot
    	\sqrt{\frac{\hat\sigma_\rct^2}{n_\rct} + \frac{\hat\sigma_\obs^2}{n_{\obs_2}}},\\
    	0
    	& \textnormal{ otherwise}.
	\end{cases}
$$
Thus, one can alternatively think of \eqref{eq:est_delta} as a LASSO-type estimator \citep{tibshirani1996regression} that minimizes $|\tilde \Delta - \delta|^2 + \lambda |\delta|$ for a particular choice of $\lambda$.

Once $\hat\Delta$ is obtained, the final estimator for $\beta^\star$ is given by 
\begin{equation}
	\label{eq:final_estimator}
	\hat \beta = \tilde \beta + \hat\weight  \hat \Delta.
\end{equation}	
The following theorem shows that $\hat\beta$ achieves nearly the same performance as the best convex combination $\hat\beta_{\weight^\star}$ with high probability, up to poly-log factors.
% \sxc{Another route is to assume stronger tail behaviors of the response and the covariates, e.g., sub-gaussian. And this route will give us stronger results, e.g., in expectation bound}.
% that only assumes $\hat \beta_\obs$ and $\hat \beta_\rct$ both exhibit a central limit behavior.
% \begin{assump}[Central limit behavior]
% Assume that for any $t\in \bbR$, we have
% $$
% 	\bigg|\bbP\bigg( \frac{\sqrt{n_\rct}|\hat \beta_\rct - \beta_\rct^\star|}{\sigma_\rct} \leq t\bigg) - \Phi(t)\bigg| \leq  \sfC_\rct n_\rct^{-\sfc_\rct}, 
% 	\qquad 
% 	\bigg|\bbP\bigg( \frac{\sqrt{n_\rct}|\hat \beta_\obs - \beta_\obs^\star|}{\sigma_\obs} \leq t\bigg) - \Phi(t)\bigg| \leq  \sfC_\obs n_{\obs_2}^{-\sfc_\obs},
% $$
% where $\Phi(t)$ is the CDF of $N(0, 1)$.
% \end{assump}
% For simplicity, we assume the propensity scores are exactly known, so that both estimators $\hat\beta_\rct$ and $\hat\beta_\obs$ are simply the average of i.i.d.~random variables. 
% Say $\hat \beta_\rct = \sum_{i=1}^{n_\rct} \phi_i/n_\rct$ and $\hat \beta_\obs = \sum_{i=1}^{n_{\obs_2}}\psi_i/n_{\obs_2}$.
% Let $\rho_\rct = \bbE|\phi_i - \beta_\rct^\star|^3$ and $\rho_\obs = \bbE |\psi_i - \beta_\obs^\star|^3$.
% \sxc{when propensity scores are estimated, arguments largely remain the same but we need to make assumptions on the rate of convergence.}

\begin{theorem}[Performance of the adaptive estimator]
\label{thm:high_prob_bound_adaptive_estimator}
Let Assumption \ref{assump:asymp_linear} hold. In addition, assume $\sigma_\rct^2/n_\rct\gtrsim \sigma_\obs^2/n_{\obs}$ and $n_\obs \geq (1+\ep)n_\rct$ for some absolute constant $\ep > 0$. If $\hat\sigma_\rct \overset{p}{\to} \sigma_\rct$ and $\hat\sigma_\obs \overset{p}{\to} \sigma_\obs$ as $n_\rct \land n_\obs \to \infty$, then with probability at least $1-o(1)$, we have
\begin{equation}
	\label{eq:high_prob_bound_adaptive_estimator}
	 |\hat\beta - \beta^\star|^2 \lesssim  \log(n_\rct\land n_{\obs_2})\cdot \bigg(\frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} + \frac{\sigma_\rct^2}{n_\rct} \land \Delta^2\bigg).
\end{equation} 
\end{theorem}


\begin{proof}
	See Appendix \ref{prf:thm:high_prob_bound_adaptive_estimator}.
\end{proof}

Inspecting the proof, one can readily check that the probability that the above bound holds is of the form $1 - (n_\rct\land n_{\obs})^{-\sfc'} - o(1)$, where $\sfc'$ is some absolute constant depending on $\sfc$ and the $o(1)$ depends on the rate of convergence of $\hat\sigma_\rct$ and $\hat\sigma_\obs$, as well as the two $o_p(1)$ terms appeared in the asymptotic linear expansion of $\hat\beta_\rct$ and $\hat\beta_\obs$. 
Meanwhile, the $\log(n_\rct \land n_\obs)$ term in the right-hand side of \eqref{eq:high_prob_bound_adaptive_estimator} can be replaced by any sequence that slowly diverges to infinity without hurting the validity of the above theorem.










% \textcolor{blue}{
% OLD: 
% Consider the following estimator:
% $$
% 	\hat\beta \in \argmin_{\beta} |\beta - \hat\beta_\rct| \qquad \textnormal{s.t. } |\beta - \hat \beta_\obs| \leq |\Delta| + \frac{\sfc \cdot \sigma_\obs}{\sqrt{n_{\obs_2}}},
% $$
% where $\sfc$ is any constant strictly greater than $1$. Then, the \amse~of this estimator is of the same order as the best convex combination and the pool-and-debias estimator. The proof is based on the fact that $\hat\beta$ is close to $\hat\beta_\obs$ and that $\beta^\star_\rct$ is a feasible solution. 
% }



\subsection{Post-transfer/post-integration inference}

\paragraph{Inverting hypothesis tests with 1-D grid search and Bonferroni correction.}
Let $\sigma_\Delta = \sqrt{\frac{\sigma_\rct^2}{n_\rct} + \frac{\sigma_\obs^2}{n_{\obs_2}}}$.
Note that the asymptotic distribution of $\tilde \Delta$ is known:
$
    \frac{\tilde \Delta - \Delta}{\sigma_\Delta} \Rightarrow N(0, 1).
$
Fix a constant $\delta \in \bbR$ and consider testing the hypothesis $H_0: \Delta = \delta$. 
Since the asymptotic distribution of $\tilde\Delta$ is known, we can construct the null distribution of $\hat \Delta$ by Monte Carlo and construct a valid $p$-value.
Running this procedure multiple times and collecting all $\delta$'s for which the null cannot be rejected, we get a valid confidence interval for $\Delta$.  \sxc{this now looks a bit spurious to me because the transformation from $\tilde\Delta$ to $\hat\Delta$ depends on the sample sizes.}

We are dealing with an 1-D parameter, so doing simulation won't be too costly. If our original parameter of interest were a vector, then we would need tools from post selection inference \citep{berk2013valid,lee2016exact} because we are essentially doing ``dataset selection'' as opposed to variable selection.

On the other hand, constructing a valid confidence interval for $\weight \beta_\obs + (1-\weight) \beta_\rct$ from $\tilde \beta$ is easy, as $\tilde\beta$ is asymptotically normal after re-scaling. Thus, we can construct a valid confidence interval for $\beta_\rct^\star = \weight \beta_\obs + (1-\weight) \beta_\rct + \weight \Delta$ using Bonferroni correction.

\paragraph{Inverting hypothesis tests with 2-D grid search.}
Fix two constants $b_\rct, b_\obs$ and consider the null hypothesis $H_0: \beta_\rct^\star = b_\rct, \beta_\obs = b_\obs$. Under $H_0$, the asymptotic distributions of all quantities involved in the construction of $\hat\beta$, namely $\tilde\beta, \tilde\Delta, \hat \Delta$, are known by Monte Carlo. We can then construct a histogram of the null distribution of $\hat\beta$, and compare it with the observed $\hat\beta$ to get a valid $p$-value for testing $H_0$. Run this procedure multiple times and collect all pairs of $(b_\rct, b_\obs)$ for which the null cannot be rejected. We then project this ``plausible'' region of values of $(b_\rct, b_\obs)$ to the first coordinate to get a valid confidence interval of $\beta^\star_\rct$. \sxc{This also looks spurious to me for the same reason as above.}

% This construction of confidence intervals is valid because of the following reason.
% Consider a random variable $Z$ which is asymptotically $N(0, 1)$. We essentially want the quantiles of $f(Z)$ to be well-approximated by the quantiles of $f(N(0, 1))$, where $f$ is a mapping representing our algorithm. Our algorithm, albeit non-smooth, is still continuous. So the continuous mapping theorem applies and we get $f(Z)$ has $f(N(0, 1))$ as its weak limit. In particular, all quantiles of $f(Z)$ can be approximated by $f(N(0, 1))$. \
% sxc{If we were using hard threshold, we may run into some trouble because of the discontinuity.}



\paragraph{Inverting hypothesis tests with 2-D grid search and the oracle test statistic.}
Fix two constants $b_\rct, b_\obs$ and again consider the null hypothesis $H_0: \beta_\rct^\star = b_\rct, \beta_\obs = b_\obs$. Under $H_0$, we know the value of $\Delta$ and we can thus construct a test statistic $\hat\beta_\Delta$ using the best convex combination, where we use the subscript $\Delta$ to emphasize that this estimate depends on $\Delta$. Moreover, the null distribution of $\hat\beta_\Delta$ is also known. So we can construct a valid $p$-value for $H_0$ with $\hat\beta_\Delta$ being the test statistic (as opposed to $\hat\beta$ in the previous approach). Inverting this test with 2-D grid search and projecting the confidence region to the $\beta^\star_\rct$ direction, we get a valid confidence interval for $\beta^\star_\rct$.
This approach is also valid --- it is just using a different test statistic every time we construct a confidence region. It has an additional benefit that we do not worry about the non-smoothness of the soft-thresholding operation. \sxc{The validity of this method is easy to prove. Not sure how long this interval will be. Also it looks like a form of sensitivity analysis to me.}

==> combining clinical and observational datasets/history/bias_old.tex <==


The $ \beta_o $ defined in \eqref{eq: beta o} is not necessarily equal to the target causal parameter  $ \beta_c^\star $ for two reasons: (i) there may be unmeasured confounding in the observational study, i.e., $ \beta_o\neq E( Y {(1)} -Y {(0)}   \mid S=o)$; (ii)  $ E( Y {(1)} -Y {(0)}   \mid S=o ) $ may not equal to $ \beta_c^\star $ due to nontransportability. How close $ \beta_o  $ is to $ \beta_c^\star $ depends on the magnitude of these two sources of bias. In the following, we give a theoretical analysis of the bias $ \beta_o-\beta_c^\star $.   

For reason (i), suppose there exists an unmeasured confounder $ U  $ that satisfies $ A  \perp ( Y(1), Y(0)) \mid U, X, S=o$. Let $ \pi_o(X, U) = P(A=1\mid X, U, S=o) $ and $  \gamma(X, U)= \text{OR} \{\pi_o(X, U), \pi_o(X) \} $, 
where 
\[
\text{OR} \{p_1, p_2\} =\frac{p_1/(1-p_1)}{p_2/(1-p_2)}. 
\]
 Then the bias from unmeasured confounding $  \beta_o -E( Y {(1)} - Y {(0)}  \mid S=o ) $ equals 
 \begin{align*}
 E\left[ \frac{AY(1-\pi_o(X))}{\pi_o(X)  } \left\{   1- \frac{1}{\gamma (X, U)}  \right\}  \mid S= o \right]  - E\left[ \frac{(1-A) Y\pi_o(X)}{1-\pi_o(X)} \left\{  1-\gamma(X, U)  \right\}  \mid S= o \right]     .
 \end{align*}
When $ \gamma(x, u)=1 $, it means no unmeasured confounding, and thus the bias due to unmeasured confounding equals zero. 

For reason (ii), for $ a\in \{0,1\} $, let 
\[
\lambda_a(y, x) = \frac{f_{Y(a)\mid X, S=o} (y\mid x, s=o)}{f_{Y(a)\mid X, S=c} (y\mid x, s=c)} = \text{OR} \{ P(S=o\mid Y(a), X=x), P(S=o\mid  X=x) \}. 
\]
Then the bias from nontransportability  $ E( Y {(1)}  -Y {(0)}   \mid S=o ) - \beta_c^\star $ equals 
\begin{align*}
 E( Y {(1)} (\lambda_1(Y(1), X) - 1) \mid S=c ) -  E( Y {(0)} (\lambda_0(Y(0), X)  -1) \mid S=c )  . 
\end{align*}
When $ \lambda_0(x, u)=\lambda_1(x, u)=1 $, it means that the transportability assumption holds, and thus the bias due to nontransportability equals zero. 


Combining both, we know that the bias of $ \beta_o $  can be written as  
\begin{align*}
 &  \beta_o - \beta_c^\star  =  \beta_o -E( Y {(1)} - Y {(0)}   \mid S=o )  + E( Y {(1)}  -Y {(0)}   \mid S=o ) - \beta_c^\star   \\
&=  E\left[ \frac{AY(1-\pi_o(X))}{\pi_o(X)  } \left\{   1- \frac{1}{\gamma (X, U)}  \right\}  \mid S= o \right]  - E\left[ \frac{(1-A) Y\pi_o(X)}{1-\pi_o(X)} \left\{  1-\gamma(X, U)  \right\}  \mid S= o \right]     \\
& \qquad  + E( Y {(1)} (\lambda_1(Y(1), X) - 1) \mid S=c ) -  E( Y {(0)} (\lambda_0(Y(0), X)  -1) \mid S=c )  . 
\end{align*}
Using Cauchy-Schwartz inequality,  we can bound $  \beta_o - \beta_c^\star $ as follows 
\begin{align}
	\begin{split}
	(\beta_o - \beta_c^\star)^2  & \lesssim E\left[ Y {(1)}^2  \mid S=c \right] E\left[ \{\lambda_1(Y(1), X) -1 \}^2\mid S=c \right]   \label{eq: bias} \\
	&\qquad +  E\left[ Y {(0)}^2  \mid S=c \right] E\left[ \{\lambda_0(Y(0), X)-1 \}^2\mid S=c \right]  \\
	&\qquad +   E\left[ \left\{\frac{AY(1-\pi_o(X))}{\pi_o(X)  }\right\}^2   \mid S= o \right] E\left[ \left\{ 1-\frac{1}{\gamma (X, U)}    \right\}^2\mid S=o\right]  \\
	&\qquad + E\left[ \left\{\frac{(1-A) Y \pi_o(X)}{1- \pi_o(X)  }\right\}^2   \mid S= o \right] E\left[ \left\{  1-\gamma(X, U) \right\}^2\mid S=o\right].  
\end{split}
\end{align}
where $ a\lesssim b  $ denotes that  there exists a constant $ C<\infty $ such that $ a\leq C b $.  \textcolor{red}{TY: I will clean up  the above equations.}



\emph{Remark.}  The analysis of bias is related to the sensitivity analysis that is a popular device to assess the sensitivity of the study conclusion to untestable assumptions. In particular, the  marginal  sensitivity analysis framework uses the supremum norm of $ \gamma(x, u) $ to quantify the deviation from the no unmeasured confounding assumption (Dorn and Guo, 2021), which may overstate the effect of unmeasured confounding in our analysis. Therefore, we instead use the integral norm  of $ \gamma(x, u) $. 



==> combining clinical and observational datasets/history/intro_old.tex <==

Randomized clinical trials (RCTs) have been considered the gold standard approach that generates the highest level evidence  for evaluating the causal effect of new medical products.  However, the traditional paradigm of assessing new treatments based on running large RCTs has become ever more expensive and time-consuming, which calls for new innovations and advances to accelerate medical product developments.  In the meantime, there is a proliferation of observational data that are collected for research or administrative purposes, such as disease registries, biobanks, administrative claims and electronic health records. Such massive and rich datasets and the exciting potentials of augmenting the current clinical development paradigm  have generated strong interest among industry, regulatory \citep{fda2018rwd}, and academia \citep{di2020real}. However, without proper randomization, there is often concern about confounding bias, in particular unmeasured confounding bias,  in  causal inference based on observational data \citep{Franklin:2021aa}. Therefore, an important question  is how to transfer knowledge from observational studies to improve  causal inference using only RCTs  without introducing bias. 

We consider the potential outcomes framework to formalize the causal inference question \citep{neyman1923application,rubin1974estimating}. Suppose that there exist a binary treatment indicator $ A $, baseline covariates $ X $, and a study indicator $ S$ which equals $ c $ if the subject is from the RCT, equals $ o $ if the subject is from the OS.  Let $ Y(a) $ be the potential outcome if $ A=a $, for $ a=0, 1 $.  


Much of the statistical literature on combining RCTs and  observational studies to better estimate casual effects 
can be divided into four main categories depending on the settings considered. The first category considers that the RCT and  observational study differs only in the covariate distribution $ (X\not \perp S) $ whereas the structural relationships between outcomes and covariates are the same ($ (Y(0), Y(1))\perp S\mid X $). Moreover, there is no unmeasured confounding in the observational study  ($ (Y(0), Y(1))\perp A\mid X, S=o $). This is so far the primary research setting and 




\begin{itemize}
    \item Setting 1: Let $P_X := P(X \mid S = 1)$ and $Q_X := P(X \mid S = 0)$ denote the marginal distribution in the clinical and observational dataset, and we have:
\[
f(Y(0), Y(1) \mid X) \mid S = 1 \quad = \quad f(Y(0), Y(1) \mid X) \mid S = 0,
\]
i.e., there is covariate shift and some version of the transportability assumption holds (i.e., the potential outcome distributions in the clinical dataset (S = 1) are the same as those in the observational dataset (S = 0)). There is no unmeasured confounding in observational dataset.

It seems the simplest approach in this case is importance weighting, and this is so far the primary research setting.

\item Setting 2: let $P = f(Y(0), Y(1), X \mid S = 1)$ and $Q = f(Y(0), Y(1), X \mid S = 0)$, $P \neq Q$, and there exists some high-level measure that quantifies the discrepancy between $P$ and $Q$. In other words, there may be both covariate shift ($X$ different) and posterior drift ($Y(\cdot)|X$ different). \sxc{label shift means $Y(\cdot)$s are different.}

\item Setting 3: There is covariate shift so that $P_X \neq Q_X$; for the moment, let us assume the transportability assumption holds so that $f(Y(0), Y(1), X \mid S = 1) = f(Y(0), Y(1), X \mid S = 0)$. However, there may exist unmeasured confounding in the observational dataset, i.e., $S = 0$, so that the usual IPWE does not estimate the average potential outcome over $Q_X$, i.e.,
\[
\sum_{i = 1}^{n_Q} \frac{A_i Y_i}{e(X_i)} \not\rightarrow \mathbb{E}_{X \sim Q_X, Y(0)\sim Q}[Y(1)]
\]
even as $n_Q \rightarrow \infty$. This setting is technically similar to, but conceptually different from Setting $2$. We can also think of Setting 3 as if the transportability assumption fails.  \citep{Kallus2018, yang2020improved}. 

\item Setting 4: There is covariate shift, the transportability assumption does not hold, and there is unmeasured confounding in observational dataset. Again, we may think of the failure of the transportability assumption and the unmeausred confounding under one unified framework.

\end{itemize}

Different from our goal of using observational data to improve causal inference based on RCTs, we note that there is also a large literature on knowledge transfer from the other direction. That is,  generalizing or transporting the RCT conclusion to a more representative patient population using observational data \citep{Stuart:2001aa, Buchanan:2018aa, Dahabreh:2019aa, colnet2020causal, degtiar2021review}. 



==> combining clinical and observational datasets/history/setup_old.tex <==

From the target population, we obtain a random sample selected into the randomized clinical trial (RCT), indexed by $ S=c $, and a random sample selected into the observational study, indexed by $ S=o $ {\color{red} (do two datasets overlap?)}. Subjects that are not directly sampled into the study from the target population are indexed by $ S=t $.    
Specifically,  we obtain random samples $ \{(Y_i(1), Y_i(0), A_i, X_i, S_i=c ), i \in \mathcal{C}\}$ of size $ n_c= |\mathcal{C}| $ from the RCT, which are independent and identically distributed  according to $ P(Y(1), Y(0), A, X, S\mid S=c ) $, and random samples $ \{(Y_i(1), Y_i(0), A_i, X_i, S_i=o ), i  \in \mathcal{O}\} $  of size  $ n_o= |\mathcal{O}| $ from the  observational study, which are  independent and identically distributed according to $ P(Y(1), Y(0), A, X, S\mid S=o ) $. For every unit $ i $, the observed outcome is $ Y_i= Y_i(A_i) $. To simplify the notation, we drop the subscript $ i $ when referring to a general unit from the population. 


The following assumption is guaranteed by the random treatment assignment in the RCT and is crucial for the identification of $ \beta_c $.  

\begin{assumption}[Design of  RCT]  \label{assumption: rct}
$ A  \perp ( Y(1), Y(0), X) \mid S=c$ and $ P(A=1\mid S=c) $ is known. 
\end{assumption}


We first consider the case with no covariate shift, as stated by the following assumption.  The general situation with covariate shift will be considered later in Section 4. 
\begin{assumption}[No covariate shift]  \label{assumption: no covariate shift}
$ S\perp X $. 
\end{assumption}


\subsection{Review: Fully Robust Estimators in RCT and Their Counterparts in OS}


Let  the known probability of receiving treatment in RCT be $ \pi_c = P(A=1\mid S=c)$, the conditional probability of receiving  treatment in OS be $ \pi_o(X)= P(A=1\mid X, S=o ) $,  and the conditional means of the outcome in study $ s $ be $ \mu_{sa}(X)=E(Y\mid X, A=a, S=s) $ for $ a\in \{0,1\} $ and $ s \in \{c, o\}  $.  


There are many methods to identify the causal effect in the RCT. In this article, we consider two commonly used ones that are fully robust in RCT, the inverse probability weighting (IPW), and the augmented inverse probability weighting (AIPW).   Specifically, the method of IPW identifies $ \beta_c^\star $ from 
\begin{align}
 \beta_c^\star  = E \left[ \frac{AY }{\pi_c }   -  \frac{(1-A)Y}{1- \pi_c}  \mid S=c\right],   \label{eq: ipw}
\end{align}
and this gives the IPW estimator 
\begin{align}
\hat	\beta_{c, \text{IPW}}  = \frac{1}{n_c} \sum_{i\in \mathcal{C}}  \frac{A_i Y_i }{\pi_c} - \frac{(1-A_i) Y_i }{1- \pi_c} .  \nonumber
\end{align}
The method of  AIPW identifies $ \beta_c^\star $ from 
\begin{align}
\beta_c^\star  = E \left[ \frac{A(Y- \mu_{c1}(X) ) }{\pi_c }   -  \frac{(1-A)(Y-\mu_{c0}(X))}{1- \pi_c} + \mu_{c1}(X)-   \mu_{c0}(X) \mid S=c\right],  \label{eq: aipw}
\end{align}
and this gives the  AIPW estimator 
\begin{align}
\hat	\beta_{c, \text{AIPW}}    = \frac{1}{n_c} \sum_{i\in \mathcal{C}}\frac{A_i (Y_i -\mu_{c1} (X_i; \hat \alpha_{c1} ) )  }{\pi_c} - \frac{(1-A_i)(Y_i -\mu_{c0} (X_i; \hat \alpha_{c0} ) ) }{1- \pi_c} + \mu_{c1} (X_i; \hat \alpha_{c1} )   - \mu_{c1} (X_i; \hat \alpha_{c0} ) .  \nonumber
\end{align}
where $ \mu_{ca}(X; \alpha_{ca} ) $ is a parametric specification of the outcome mean model $  \mu_{ca}(X; \alpha_{ca} ) $, and $ \hat \alpha_{ca} $ is an estimator of $ \alpha_{ca} $. 
 
In RCT where  subjects are randomly assigned to two treatment arms as in Assumption \ref{assumption: rct},  the IPW estimator $ \hat	\beta_{c, \text{IPW}}  $  is fully robust in the sense that \eqref{eq: ipw} holds regardless of outcome generating process.  

We also define the IPW and AIPW counterparts based on OS.  We denote the parameter identified by IPW and AIPW in OS as $ \beta_{o} $, and the identification formulas are respectively as follows
\begin{align}
	\begin{split}
	\beta_o &= E \left[ \frac{AY }{\pi_o(X) }   -  \frac{(1-A)Y}{1- \pi_o(X)}  \mid S=o\right],  \label{eq: beta o}\\
  \beta_o  &= E \left[ \frac{A(Y- \mu_{o1}(X) ) }{\pi_o(X) }   -  \frac{(1-A)(Y-\mu_{o0}(X))}{1- \pi_o(X)} + \mu_{o1}(X)-   \mu_{o0}(X) \mid S=o \right]. 
\end{split}
\end{align} 
The corresponding IPW and AIPW estimators are  
\begin{align}
	\hat	\beta_{o, \text{IPW}} &= \frac{1}{n_o} \sum_{i\in \mathcal{O}}  \frac{A_i Y_i }{\pi_o(X_i; \hat \eta)} - \frac{(1-A_i) Y_i }{1- \pi_o(X_i; \hat \eta) } ,\nonumber\\
		\hat	\beta_{o, \text{AIPW}} &=  \frac{1}{n_o} \sum_{i\in \mathcal{O}}\frac{A_i (Y_i -\mu_{o1} (X_i; \hat \alpha_{o1} ) )  }{\pi_o(X_i; \hat\eta )} - \frac{(1-A_i)(Y_i -\mu_{o0} (X_i; \hat \alpha_{o0} ) ) }{1- \pi_o(X_i;\hat\eta)} + \mu_{o1} (X_i; \hat \alpha_{o1} )   - \mu_{o0} (X_i; \hat \alpha_{o1} ) , \nonumber
\end{align}
where $ \mu_{oa}(X; \alpha_{oa} ) $ is a parametric specification of the outcome mean model $  \mu_{oa}(X; \alpha_{oa} ) $, and $ \hat \alpha_{oa} $ is an estimator of $ \alpha_{oa} $. It is important to note that $ \beta_o $ has no causal interpretation under Assumptions \ref{assumption: rct}-\ref{assumption: no covariate shift}; it is also not necessarily equal or close to the target causal parameter $\beta_c^\star  $. 

{\color{red}Variance formulas}

(i) When $ \mu_{ca}(x; \alpha_{ca} )  $ are linear models, then $ \sqrt{n} (\hat\beta_{c,\text{AIPW} } - \beta_c^\star) $ is asymptotically normal, with mean 0 and variance 
\begin{align*}
	\frac{{\rm var} (Y(1) - X^T \alpha_{c1} )}{\pi_c} +  	\frac{{\rm var} (Y(0) - X^T \alpha_{c0} )}{1- \pi_c}  +  {\rm var} (X^T( \alpha_{c1} - \alpha_{c0}))
\end{align*} 

(ii)  When $ \mu_{oa}(x; \alpha_{oa} )  $ are linear models, $ \pi_o (X_i; \eta) $ is a logistic model,
  then $ \sqrt{n} (\hat\beta_{o,\text{AIPW} } - \beta_o) $ is asymptotically normal, with mean 0 and variance 

==> history/02-setup_old2.tex <==
%!TEX root = 00-main.tex
\section{Set-up}
\textcolor{red}{We have approx 5 pages in set-up/review of two biases. We may want to trim it to three pages and put the rest to the supplement.}
\label{sec: setup}
\subsection{Notation, estimands and baseline estimators}
Suppose the existence of a binary treatment $ A\in \{0,1\} $, potential outcomes $\{Y(1), Y(0)\}$ and baseline observed covariates $\mathbf{X}$. 
We assume consistency so that the observed outcome $Y$ satisfies $Y= AY(1) + (1-A)Y(0)$. 
Our estimand of interest is the average treatment effect of the target population (PATE):
\begin{equation*}
    % \label{eq:PATE}
     \beta^\ast = \mathbb{E}[Y{(1)} - Y{(0)}],
\end{equation*}
where $\mathbb{E}[\cdot]$ is taken with respect to the joint distribution of $\{\mathbf{X}, Y(0), Y(1)\}$ over the target population. A random sample of size $n_c$ from the target population was selected into a RCT according to some sample selection protocol. 
We use $S = c$ to indicate selection into the RCT and let $\mathcal{C}$ denote the associated index set so that $|\mathcal{C}| = n_c$. Write the RCT data as \textcolor{red}{We may want to write less important expressions inline.}
\begin{equation*}
    \mathcal{D}_{c} = \{(Y_i, A_i, \mathbf{X}_i, S_i = c):~i \in \mathcal{C}\},
\end{equation*}
and denote the average treatment effect in the RCT population as
\begin{equation*}
    \beta^\ast_{c} = \mathbb{E}[Y(1) - Y(0) \mid S = c],
\end{equation*}
where $\mathbb{E}[\cdot]$ is taken with respect to the conditional joint distribution of $\{\mathbf{X}, Y(0), Y(1) \mid S = c\}$, i.e., over the RCT population. 
Assume that the data in $\mathcal{D}_{c}$ are independent and identically distributed according to the joint law of $\big(Y(1), Y(0), A, \mathbf{X}\big) \mid S = c$ and let $\pi_c(\mathbf{x}) = \bbP(A = 1 \mid \mathbf{X}=\mathbf{x}, S = c)>0$ denote the \emph{known} treatment assignment probability in the RCT. 
The average treatment effect in the RCT population $\beta^\ast_c$ is then identified from $\mathcal{D}_c$ and can be estimated via the following inverse probability weighting (IPW) estimator \citep{horvitz1952generalization}:
\begin{equation}
\label{eq:cipw}
\hat\beta_{c, \textsf{IPW}}  = \frac{1}{n_c} \sum_{i\in \mathcal{C}}  \bigg(\frac{A_i Y_i }{\pi_c(\mathbf{X}_i)} - \frac{(1-A_i) Y_i }{1- \pi_c(\mathbf{X}_i)}\bigg).
\end{equation}
Another estimator that is also commonly considered is the regression imputation or g-formula estimator, which fits a conditional outcome mean model for each treatment arm and then marginalizes over the RCT samples \citep{robins1986}. Because it is in general not fully robust to misspecification of the outcome-covariate relationship and thus does not exploit the full advantage of RCTs, this is not further considered in this article. \textcolor{red}{We may want to move some standard stuff into supplement.}


Alternatively, $\beta^\ast_c$ can be estimated via the following augmented inverse probability weighting (AIPW) estimator \citep{robins1994estimation, bang2005doubly} 
\begin{align*}
% \begin{split}
\hat\beta_{c, \textsf{AIPW}}
&  = \frac{1}{n_c} \sum_{i\in \mathcal{C}}\bigg(\frac{A_i (Y_i -\mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} ) )  }{\pi_c(\mathbf{X}_i)} - \frac{(1-A_i)(Y_i -\mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ) ) }{1- \pi_c(\mathbf{X}_i)} \\
\label{eq:caipw}
& \qquad \qquad \qquad +\mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} )   - \mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} )\bigg),\numberthis
% \end{split}
\end{align*}
where $ \mu_{ca}(\bfx; \bsalpha_{ca} ),a = 0, 1,$ are parametric specifications (parametrized by $\bsalpha_{c0}$ and $\bsalpha_{c1}$, respectively) of the conditional outcome means $\mu_{ca}(\bfx) = \mathbb{E}[Y \mid \bfX=\bfx, A = a, S = c]$ and $ \hat \bsalpha_{ca} $ are estimators of $ \bsalpha_{ca}$. 
In an RCT with known $\pi_c(\bfx)$, the AIPW estimator $ \hat\beta_{c, \textsf{AIPW}}$ is robust in the sense that it consistently estimates $\beta^\ast_c$ even when the parametric outcome regression models $\mu_{ca} (\bfx; \bsalpha_{ca})$ do not correctly specify $\mu_{ca}(\bfx)$ for $a = 0, 1$ (\citealp{bang2005doubly,tsiatis2007semiparametric}). 
Besides robustness, AIPW also enjoys desirable efficiency properties.
It is locally efficient if $\mu_{ca} (\bfx; \bsalpha_{ca})$ correctly specifies $\mu_{ca}(\bfx)$. 
It is also guaranteed to be more efficient than $\hat\beta_{c, \textsf{IPW}}$ when $\pi_c(\bfx)$ does not depend on the covariate vector $\bfx$ (i.e., random treatment assignment),  $\mu_{ca}(\bfx; \bsalpha_{ca})$ are linear parametric models of $\mu_{ca}(\bfx)$, and $ \hat \bsalpha_{ca}$ are the corresponding least squares estimators (\citealp{tsiatis2008covariate}). 

In parallel, a random sample of size $n_o$ from the target population was collected in an observational study, which is typically of a much larger size compared to the RCT. We use $S = o$ to indicate selection into the observational study and let $\mathcal{O}$ denote the associated index set so that $|\mathcal{O}| = n_o$. 
Write the observational data as
\begin{equation*}
    \mathcal{D}_{o} = \{(Y_i, A_i, \mathbf{X}_i, S_i = o):~i \in \mathcal{O}\}
\end{equation*}
and define the average treatment effect in the observational study population as
\begin{equation*}
    \beta^\ast_{o} = \mathbb{E}[Y(1) - Y(0) \mid S = o],
\end{equation*}
where $\mathbb{E}[\cdot]$ is taken with respect to the conditional joint distribution of $\big(\mathbf{X}, Y(0), Y(1) \big)\mid S = o$. Assume that the data in $\mathcal{D}_{o }$ are independent and identically distributed according to the joint law of $\big(Y(1), Y(0), A, \mathbf{X}\big) \mid S = o$.  
% According to Assumption \ref{assump: observational is target} stated later in Section \ref{subsec: external validity}, the observational study population is the same as the target population, so we have $\beta_o^\ast= \beta^\ast$.

Let $\pi_{o}(\bfx) = \bbP(A = 1 \mid \mathbf{X} = \bfx, S = o)>0$ denote the treatment assignment probability in the observational data, i.e., the propensity score (\citealp{rosenbaum1983central}), $\mu_{oa}(\bfx) = \mathbb{E}[Y \mid \mathbf{X}=\bfx, A = a, S = o]$ the conditional outcome means in the observational data, and  $\pi_{o}(\bfx; \bseta)$ and $\mu_{oa}(\bfx;  \bsalpha_{oa})$ their corresponding parametric specifications. The counterparts of $\cipw$ and $\caipw$ defined in \eqref{eq:cipw} and \eqref{eq:caipw} can then be formed as
\begin{align}
\label{eqn:oipw}
	\hat\beta_{o, \textsf{IPW}} &= \frac{1}{n_o} \sum_{i\in \mathcal{O}}  \bigg(\frac{A_i Y_i }{\pi_{o}(\mathbf{X}_i; \hat \bseta)} - \frac{(1-A_i) Y_i }{1- \pi_{o}(\mathbf{X}_i; \hat \bseta) }\bigg) ,\\
		\hat	\beta_{o, \textsf{AIPW}} &=  \frac{1}{n_o} \sum_{i\in \mathcal{O}}\bigg(\frac{A_i (Y_i -\mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} ) )  }{\pi_{o}(\mathbf{X}_i; \hat\bseta )} - \frac{(1-A_i)(Y_i -\mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} ) ) }{1- \pi_{o}(\mathbf{X}_i;\hat\bseta)}  \nonumber\\
\label{eqn:oaipw}
        & \qquad \qquad\qquad + \mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} )   - \mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} )\bigg),
\end{align}
where $\hat\bseta$ and $\hat\bsalpha_{oa}$ are estimates of $\bseta$ and $\bsalpha_{oa}$, respectively. 

Note that without further assumptions, neither $\beta^\star_\rct$ nor $\beta^\star_\obs$ agrees with our estimand of interest $\beta^\star$.

\subsection{Internal validity bias}
\label{subsec: internal validity}
Internal validity refers to an effect estimate being (asymptotically) unbiased for the causal effect. 
Constructing estimators that the internally valid for the RCT population (i.e., can consistently estimate $\beta^\star_\rct$) is a relatively easy task.
In particular, the following assumption holds by design.

\begin{assumption}[Design of RCT]\label{assump: design of RCT} \rm
For the RCT population, we assume $A \perp (Y(1), Y(0)) \mid \mathbf{X}, S=c$, the treatment assignment probability $ \pi_c(\mathbf{x}):= P(A=1\mid \mathbf{X}=\mathbf{x}, S=c) $ is known, and $\pi_c(\mathbf{X})>0$ with probability 1 with respect to the law of $\bfX\mid S = c$. 
\end{assumption}
Assumption \ref{assump: design of RCT} states that the treatment assignment in the RCT population is manipulated by the experimenter and depends only on the observed covariates. 
Under Assumption \ref{assump: design of RCT} and usual identification assumptions of consistency and the Stable Unit Treatment Value Assumption (SUTVA) (\citealp{Rubin1980}), both $\hat\beta_{c, \textsf{IPW}}$ and $\hat\beta_{c, \textsf{AIPW}}$ defined in \eqref{eq:cipw} and \eqref{eq:caipw} are internally valid: they are consistent and asymptotically normal estimators for the causal estimand $\beta^{\ast}_c$. 


On the other hand, constructing internally valid estimators for the observational population is typically an impossible task due to confounding bias from unobserved covariates. 
Consequently, the two estimators $\hat\beta_{o, \textsf{IPW}}$ and $\hat\beta_{o, \textsf{AIPW}}$ defined in \eqref{eqn:oipw} and \eqref{eqn:oaipw} are not necessarily estimating $\beta^\ast_o$, the causal estimand defined based on the observational data. 

To further understand how the internal validity bias arises from unobserved covariates, we consider an unmeasured confounder $U$ such that the treatment assignment becomes ignorable once conditional on $(\mathbf{X}, U)$ \citep{rosenbaum1983central, rosenbaum1983sens, Imbens2003}, i.e., $ A  \indep ( Y(1), Y(0)) \mid \mathbf{X}, U, S=o$ but $ A \nindep ( Y(1), Y(0)) \mid \mathbf{X}, S=o$. 
Meanwhile, we make the following standard positivity assumption.
\begin{assumption}[Positivity of Treatment Assignment in Observational Study]\label{assump: positivity obs} 
Assume the treatment assignment probability $\pi_o(\mathbf{X}):= P(A=1\mid \bfX, S=o)>0$ with probability 1 with respect to the law of $\bfX \mid S = \obs$.
\end{assumption}
Under the above assumption, even when $\pi_o(\mathbf{x}; \bseta)$ and $\mu_{oa}(\mathbf{x}; \bsalpha_{oa})$ correctly specify  $\pi_o(\mathbf{x})$ and $\mu_{oa}(\mathbf{x})$, the estimators $ \hat\beta_{o, \textsf{IPW}}$ and $\hat\beta_{o, \textsf{AIPW}}$ are still estimating a non-causal quantity 
$$
\beta_o=\mathbb{E}\left[Y\mid  S = o, A=1\right] - \mathbb{E}\left[Y\mid  S = o, A=0\right],
$$
because they fail to adjust for the presence of $U$. 

The difference between the causal $\beta^\ast_o$ and the non-causal counterpart $\beta_{o}$ takes the following form (see Appendix \textcolor{red}{XX} for a detailed derivation):
\begin{align*}
% \begin{split}
  \Delta  =\beta^\ast_{o} - \beta_{o}
  &=  \mathbb{E}\left[ \frac{(1-A) Y\pi_{o}(\mathbf{X})}{1-\pi_{o}(\mathbf{X})} \left\{  1-\gamma(\mathbf{X}, U)  \right\}  \mid S= o \right]\\
  \label{eqn: Obs data internal validity bias}
  & \qquad - \mathbb{E}\left[ \frac{AY(1-\pi_{o}(\mathbf{X}))}{\pi_{o}(\mathbf{X})  } \left\{   1- \frac{1}{\gamma (\mathbf{X}, U)}  \right\}  \mid S= o \right], \numberthis
% \end{split}
\end{align*}
where $\gamma(\mathbf{X}, U)$ represents the odds ratio of the true propensity score $\pi_{o}(\mathbf{X}, U) = P(A= 1 \mid \mathbf{X}, U, S = o)$ that takes into account the unobserved covariate $U$ and the observed propensity score $\pi_{o}(\mathbf{X}) = \bbP(A = 1 \mid \mathbf{X}, S = o)$, i.e.,
\begin{equation*}
  \gamma(\mathbf{X}, U)
  % = \text{OR} \{\pi_{o}(\mathbf{X}, U), \pi_{o}(\mathbf{X}) \} 
  = \frac{\pi_{o}(\mathbf{X}, U)/[1-\pi_{o}(\mathbf{X}, U)]}{\pi_{o}(\mathbf{X})/[1- \pi_{o}(\mathbf{X})]}. 
\end{equation*}
Namely, $\Delta$ measures the internal validity bias from the observational data. 
There are other ways to parametrize and represent the bias $\Delta$. Our method and theory developed in Section \ref{sec: method} does \emph{not} depend on the particular parametrization or the correct specification of the nuisance models $\pi_o(\mathbf{x})$ and $\mu_{oa}(\mathbf{x})$. 
In other words, the estimator based on the observational data can have arbitrary bias. 




\subsection{External validity bias}
\label{subsec: external validity}
External validity is concerned with how well the effect estimates generalize to other contexts \citep{degtiar2021review}.
It can arise from various sources, such as the difference in subject characteristics, study setting, etc.
% \citet{degtiar2021review} discussed multiple sources of external validity bias (e.g., difference in subject characteristics, study setting, etc); we focus on the bias arising from the variation in sample selection probability, the treatment effect heterogeneity, and the interplay between these two factors. 
To have a fine-grained characterization of the external validity bias, one need to specify the target population of interest.

In the main manuscript, we focus on the setting where the observational data represent our target population, as formalized in the following assumption.
\begin{assumption}[Target Population]\label{assump:target}
Assume 
% either one of the following holds:
% \begin{itemize}
    % \item[(a)] The RCT data represent the target population, so that $(\mathbf{X}, Y(0), Y(1)\mid S=c) \overset{d}{=} ( \mathbf{X}, Y(0), Y(1))$;
    % \item[(b)] 
    $\bbE[Y(a)\mid \bfX, S = \obs] = \bbE[Y(a)\mid \bfX]$ for any $a\in\{0, 1\}$.
% \end{itemize}
\end{assumption}

It is clear that under the above assumption, we have $\beta^\star = \beta^\star_\obs$.
% , wheres under the latter setting, we have $\beta^\star = \beta^\star_\obs$.
% Either setting could be of interest to the investigator.
% The latter 
Such a setting is prevalent in practice, as participants in RCT are typically highly selected and thus the population it represents can differ significantly from the ultimate population of interest.
We remark that our method and theory developed in Section \ref{sec: method} can be extended in a \emph{mutatis mutandis} fashion to accommodate other settings, such as when the RCT data represent the target population, or even when there is a separate target population that is distinct from either RCT or observational data. For ease of exposition, we defer the discussion of such extensions to Appendix \ref{appx:rct_as_target}.

% In contrast, the former setting is relevant when the investigator is interested only in the subjects with a particular set of characteristics.
% Before proceed further, we remark that our method and theory developed in Section \ref{sec: method} could be extended in a \emph{mutatis mutandis} fashion to handle the case where there is a separate target population that is different from the population represented by either the RCT or the observational data. But we do not pursue this direction in this article. 
% \paragraph{The observational population is the target.}
When the observational data represent the target population, the two RCT-based estimators, namely $\cipw$ and $\caipw$, albeit being internally valid, do not converge to the correct target $\beta^\star$ asymptotically.
Fortunately, their external validity bias can be eliminated under the following \emph{conditional mean exchangeability} assumption, also known as the \emph{generalizability} assumption \citep{Stuart:2011aa, Dahabreh:2019aa, degtiar2021review}. 

\begin{assumption}[Conditional Mean Exchangeability]\label{assump: study selection exchangeability}
For any $a\in\{0, 1\}$, assume
$\mathbb{E}[Y(a) \mid \mathbf{X}, S = c] = \mathbb{E}[Y(a) \mid \mathbf{X}]$.
\end{assumption}
The above assumption states that participating in the RCT does not affect the potential outcome means and is a standard assumption that allows for generalizing the causal estimand in the RCT population to the target population.
Under this assumption, the PATE $\beta^\star$ can be identified from the RCT data via inverse probability weighting on the participation probability $e_\rct(\bfx) = \bbP(S = \rct\mid \bfX =\bfx, S \in \{\rct, \obs\})$, where we use $S \in \{\rct, \obs\}$ to indicate that the probability is taken with respect to the law of $\bfX$ marginalized over the RCT and the observational data.

In practice, the participation probability $e_\rct$ is unknown and thus must be estimated from the data. To make this task possible, we impose the following assumption.
% In Assumption \ref{assump: bdd density ratio}, we also require common support of the observed covariates with respect to study selection.
\begin{assumption}[Bounded Density Ratio]\label{assump: bdd density ratio}
Assume $\bbP(\mathbf{X}= \mathbf{x}\mid S=o) / \bbP( \mathbf{X}= \mathbf{x} \mid S=c)<\infty$ for all $\mathbf{x}$ with positive density with respect to the law of $(\bfX \mid S \in \{\rct, \obs\})$. 
\end{assumption}

%\begin{assumption}[Decaying Probability of Selection into RCT]\label{assump: sample selection positivity for Obs}\rm
%$P(S = s \mid \mathbf{X} = \mathbf{x}) > 0$ for $s = o, t$, and every $\mathbf{x}$ with positive density. 
%\end{assumption}
 
%Recall that $\beta_o$ denotes the probability limit of the observational studies estimators $\hat\beta_{o, \textsf{IPW}}$ and $\hat\beta_{o, \textsf{AIPW}}$ in \eqref{eqn: IPW and AIPW for obs}. The bias of both estimators with respect to the target parameter $\beta^\ast$ can be decomposed into an internal validity bias term and an external validity bias term as follows:
%\begin{equation}
%\begin{split}
%    \Delta := \beta_o - \beta^\ast = \underbrace{\beta_o- \beta^\ast_o}_{\text{internal validity bias}} + \underbrace{\beta^\ast_o - \beta^\ast}_{\text{external validity bias}}.
%\end{split}
%\end{equation}

%In the absence of the internal validity bias, one may eliminate the external validity bias by adopting an inverse probability of participation weighting (IPPW) or augmented inverse probability of participation weighting (AIPPW) approach (\citealp{Stuart:2011aa, Dahabreh:2019aa}) and form the following re-weighted estimators:
%\begin{align*}
%\hat\beta_{o, \textsf{IPPW}}  &= \frac{1}{n_t} \sum_{i\in \mathcal{O}} \bigg[ \frac{A_i Y_i }{\pi_{o}(\mathbf{X}_i; \hat\bseta)} - \frac{(1-A_i) Y_i }{1- \pi_{o}(\mathbf{X}_i;\hat\bseta)}\bigg] \frac{ e_{{t}}(\mathbf{X}_i; \hat \omega_{{t}} )  }{e_{{o}}(\mathbf{X}_i; \hat \omega_{{c}} )    }\\
%\hat\beta_{o, \textsf{AIPPW}}   & = \frac{1}{n_t} \sum_{i\in \mathcal{O}} \bigg[\frac{A_i (Y_i -\mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} ) )  }{\pi_{o}(\mathbf{X}_i; \hat\bseta)} - \frac{(1-A_i)(Y_i -\mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} ) ) }{1- \pi_{o}(\mathbf{X}_i; \hat\bseta)}  \bigg] \frac{ e_{{t}}(\mathbf{X}_i; \hat \omega_{{t}} ) }{e_{{o}}(\mathbf{X}_i; \hat \omega_{{c}} )  } \\
%&\qquad + \frac{1}{n_t} \sum_{i\in \mathcal{T}} \mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} )   - \mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} ).
%\end{align*}

%In the above display, $\pi_o > 0$ for all $\mathbf{x}$ by the treatment assignment positivity assumption in observational study and $e_o > 0$ for all $\mathbf{x}$ by Assumption \ref{assump: sample selection positivity for Obs}. In the finite sample, both estimators may be unstable as weights may be very close to $0$ for some $\mathbf{x}$. To alleviate this issue, one may further adopt a stabilized version of both estimators.

%In the presence of the internal validity bias, both IPPW and AIPPW estimators change the covariate distribution over which the internal validity bias is evaluated and there is no decisive conclusion whether inverse participation probability weighting would mitigate or amplifies the internal validity bias of $\hat\beta_{o, \textsf{IPW}}$ or $\hat\beta_{o, \textsf{AIPW}}$.


Commonly in existing works, the positivity of RCT participation (i.e., $\bbP(S=c\mid \mathbf{X}=\mathbf{x}, S\in \{o_1,c\} )$ is strictly bounded away from zero and one almost surely) is imposed \citep{Stuart:2011aa, Dahabreh:2019aa, lu2019causal, degtiar2021review}. Under positivity of RCT participation, plus Assumptions \ref{assump:target} and \ref{assump: study selection exchangeability}, \citet{Stuart:2011aa} and \citet{Dahabreh:2019aa} showed that one can adopt an inverse probability of participation weighting (IPPW) or augmented inverse probability of participation weighting (AIPPW) approach to generalize the RCT-based estimators to the target population.

However, the positivity of RCT participation is much stronger than Assumption \ref{assump: bdd density ratio} and almost never hold in practice. 
To see this, let us note that the observational data is typically of a much larger size compared to the RCT (this is also why we would like to use the observational data despite its potential internal validity bias).
The fact that $n_\obs\gg n_\rct$ signifies that the RCT participation probability must decay to zero as the sample size goes to infinity, and thus the positivity of RCT participation is naturally violated.

Our Assumption \ref{assump: bdd density ratio} does not assume away decaying probability of RCT participation. 
One approach to tackle this challenge is to use the technique developed in \cite{zhang2021double}. However, their estimation procedure is complicated and the convergence rate of the resulting estimator is typically slower than $n_c^{-1/2}$. 
In this article, we propose a simple procedure that restores the usual $n_c^{-1/2}$ rate: we randomly sample a subset of size $n_c$ from the observational data, denoted as $\mathcal{D}_{\mathcal{O}_1}$, then we use $\mathcal{D}_{\mathcal{C}}\cup\mathcal{D}_{\mathcal{O}_1} $ to
 adjust for the external validity bias of the RCT-based estimators using IPPW or AIPPW. This leads to the following RCT-based estimators for PATE $\beta^* = \beta^\star_\obs$:
\begin{align*}
\begin{split}
    \hat\beta_{c, \textsf{IPPW}}  &= \frac{1}{n_c} \sum_{i\in \mathcal{C}} \bigg[ \frac{A_i Y_i }{\pi_c(\mathbf{X}_i)} - \frac{(1-A_i) Y_i }{1- \pi_c(\mathbf{X}_i)}\bigg] \frac{ 1-e_{{c}}(\mathbf{X}_i; \hat \xi )  }{e_{{c}}(\mathbf{X}_i; \hat \xi )    },\\
\hat\beta_{c, \textsf{AIPPW}}   & = \frac{1}{n_c} \sum_{i\in \mathcal{C}} \bigg[\frac{A_i (Y_i -\mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} ) )  }{\pi_c(\mathbf{X}_i)} - \frac{(1-A_i)(Y_i -\mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ) ) }{1- \pi_c(\mathbf{X}_i)}  \bigg] \frac{ 1-e_{{c}}(\mathbf{X}_i; \hat \xi )  }{e_{{c}}(\mathbf{X}_i; \hat \xi )  } \\
&\qquad + \frac{1}{n_c} \sum_{i\in \mathcal{O}_1} \mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} )   - \mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ),
\end{split}
\end{align*}
where $e_{{c}}(\mathbf{x};  \xi )$ is a parametric specification of the ground truth participation probability $e_\rct(\bfx)$, and $\hat\xi$ is an estimator of $\xi$ obtained from $\mathcal{D}_{\mathcal{C}}\cup\mathcal{D}_{\mathcal{O}_1} $. 
It can be shown that when $e_{{c}}(\mathbf{X}_i; \xi )$ is correct, the probability limit of $\hat\beta_{c, \textsf{IPPW}} $ is $\beta^\star_\obs = \beta^\star$; when either  $e_{{c}}(\mathbf{X}_i; \xi )$ or $ \{\mu_{c1} (\mathbf{X}_i;  \bsalpha_{c1} ),  \mu_{c0} (\mathbf{X}_i;  \bsalpha_{c0} )\}$ is correct,  the probability limit of $\hat\beta_{c, \textsf{AIPPW}} $ is $\beta^\star_\obs = \beta^\star$. 

We use the remaining observational data $\mathcal{D}_{\mathcal{O}_2} = \mathcal{D}_{\mathcal{O}}\setminus\mathcal{D}_{\mathcal{O}_1}$ to construct the observational-data-based estimators $\hat\beta_{o_2,\textsf{IPW}}$ and $\hat\beta_{o_2,\textsf{AIPW}}$, whose formal definitions are given below: 
\begin{align*}
    	\hat\beta_{o_2, \textsf{IPW}} &= \frac{1}{n_{o_2} } \sum_{i\in \mathcal{O}_2}  \bigg(\frac{A_i Y_i }{\pi_{o}(\mathbf{X}_i; \hat \bseta)} - \frac{(1-A_i) Y_i }{1- \pi_{o}(\mathbf{X}_i; \hat \bseta) }\bigg) ,\\
		\hat	\beta_{o_2, \textsf{AIPW}} &=  \frac{1}{n_{o_2}} \sum_{i\in \mathcal{O}_2}\bigg(\frac{A_i (Y_i -\mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} ) )  }{\pi_{o}(\mathbf{X}_i; \hat\bseta )} - \frac{(1-A_i)(Y_i -\mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} ) ) }{1- \pi_{o}(\mathbf{X}_i;\hat\bseta)} \\
        & \qquad \qquad \qquad + \mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} )   - \mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o1} )\bigg),
\end{align*}
where (with slight abuse of notation) $\hat\bseta$ and $\hat\bsalpha_{oa}$ are estimators of $\bseta$ and $\bsalpha_{oa}$ obtained from $\mathcal{D}_{\mathcal{O}_2}$. 
Under Assumption \ref{assump:target}(b), the two estimators given above do not suffer from external validity bias, and their only source of bias is the internal validity bias $\Delta_\inter$.
% \begin{assumption}[Observational/Target Population]\label{assump: observational is target}
% $\bbP(\mathbf{X}, Y(0), Y(1)\mid S=o) = \bbP( \mathbf{X}, Y(0), Y(1))$. 
% \end{assumption}

It is well know that IPW-type estimators like $\cippw, \caippw, \ooipw$, and $\ooaipw$ can be unstable when the (estimated) weights are close to zero. To alleviate this issue, one can apply the stabilization method by normalizing the weights to sum to 1 \citep{robins2007comment}.  For example, the stabilized version of $\caippw$ is 
\begin{align*}
        \hat\beta_{c, \textsf{sAIPPW}} &= \bigg[  \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{A_i(1-e_{{c}}(\mathbf{X}_i; \hat \xi )) }{\pi_c(\mathbf{X}_i)e_{{c}}(\mathbf{X}_i; \hat \xi ) }\bigg]^{-1} \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{A_i(1-e_{{c}}(\mathbf{X}_i; \hat \xi )) (Y_i -\mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} ) )  }{\pi_c(\mathbf{X}_i)e_{{c}}(\mathbf{X}_i; \hat \xi ) } \\
        & \qquad - \bigg[  \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{(1-A_i)(1-e_{{c}}(\mathbf{X}_i; \hat \xi ))}{(1- \pi_c(\mathbf{X}_i))e_{{c}}(\mathbf{X}_i; \hat \xi )} \bigg]^{-1}\frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{(1-A_i)(1-e_{{c}}(\mathbf{X}_i; \hat \xi ))(Y_i -\mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ) ) }{(1- \pi_c(\mathbf{X}_i))e_{{c}}(\mathbf{X}_i; \hat \xi )}   \\
         \label{eqn: c,sAIPPW}
&\qquad + \frac{1}{n_c} \sum_{i\in \mathcal{O}_1} \mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} )   - \mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ). \numberthis
\end{align*}
% Finally, it is well know that estimators like $\hat\beta_{o_2, \textsf{IPW}}, \hat\beta_{o_2, \textsf{AIPW}}, \hat\beta_{c, \textsf{IPPW}},$ and $ \hat\beta_{c, \textsf{AIPPW}}$ can be unstable when the treatment assignment and study selection probability $\pi_o(\mathbf{x}), 1-\pi_o(\mathbf{x}),$ and $ e_c(\mathbf{x})$, or their parametric specifications are close to 0 for some $\mathbf{x}$. To alleviate this issue, one can apply the stabilization method by normalizing the weights to sum to 1 \citep{robins2007comment}.  For example, the stabilized RCT-based AIPPW estimator $\hat\beta_{c, \textsf{sAIPPW}}$ is 
% \begin{align} \label{eqn: c,sAIPPW}
% \begin{split}
%     	\hat\beta_{c, \textsf{sAIPPW}} &= \bigg[  \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{A_i(1-e_{{c}}(\mathbf{X}_i; \hat \xi )) }{\pi_c(\mathbf{X}_i)e_{{c}}(\mathbf{X}_i; \hat \xi ) }\bigg]^{-1} \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{A_i(1-e_{{c}}(\mathbf{X}_i; \hat \xi )) (Y_i -\mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} ) )  }{\pi_c(\mathbf{X}_i)e_{{c}}(\mathbf{X}_i; \hat \xi ) } \\
%     	& \qquad - \bigg[  \frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{(1-A_i)(1-e_{{c}}(\mathbf{X}_i; \hat \xi ))}{(1- \pi_c(\mathbf{X}_i))e_{{c}}(\mathbf{X}_i; \hat \xi )} \bigg]^{-1}\frac{1}{n_c} \sum_{i\in \mathcal{C}} \frac{(1-A_i)(1-e_{{c}}(\mathbf{X}_i; \hat \xi ))(Y_i -\mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ) ) }{(1- \pi_c(\mathbf{X}_i))e_{{c}}(\mathbf{X}_i; \hat \xi )}   \\
% &\qquad + \frac{1}{n_c} \sum_{i\in \mathcal{O}_1} \mu_{c1} (\mathbf{X}_i; \hat \bsalpha_{c1} )   - \mu_{c0} (\mathbf{X}_i; \hat \bsalpha_{c0} ); 
% \end{split}
% \end{align}
and the stabilized AIPW estimator version of $\ooaipw$ is given by 
\begin{align*}
% \begin{split}
    	\hat\beta_{o_2, \textsf{sAIPW}} &=
    	\bigg[\frac{1}{n_{o_2}} \sum_{i\in \mathcal{O}_2}\frac{A_i  }{\pi_{o}(\mathbf{X}_i; \hat\bseta )} \bigg]^{-1}\frac{1}{n_{o_2}} \sum_{i\in \mathcal{O}_2} \frac{A_i (Y_i -\mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} ) )  }{\pi_{o}(\mathbf{X}_i; \hat\bseta )}  \\
    	& \qquad - \bigg[\frac{1}{n_{o_2}} \sum_{i\in \mathcal{O}_2}\frac{1-A_i  }{1-\pi_{o}(\mathbf{X}_i; \hat\bseta )} \bigg]^{-1}\frac{1}{n_{o_2}} \sum_{i\in \mathcal{O}_2}\frac{(1-A_i)(Y_i -\mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} ) ) }{1- \pi_{o}(\mathbf{X}_i;\hat\bseta)}\\
         \label{eqn: o2,sAIPW}
        &    \qquad   +\frac{1}{n_{o_2}} \sum_{i\in \mathcal{O}_2} \mu_{o1} (\mathbf{X}_i; \hat \bsalpha_{o1} )   - \mu_{o0} (\mathbf{X}_i; \hat \bsalpha_{o0} ). \numberthis
% \end{split}
\end{align*}
Note that the stabilized estimators are asymptotically equivalent to their unstabilized counterparts. \textcolor{red}{give ref?}
The consistency, asymptotic normality, and influence function representation of the introduced estimators are standard and can be immediately obtained from \citet[Chapter 6.1]{newey1994}. 
In the following, because of their appealing properties, we will use $\hat\beta_{c, \textsf{sAIPPW}}$ defined in \eqref{eqn: c,sAIPPW} and  $\hat\beta_{o_2, \textsf{sAIPW}}$ defined in \eqref{eqn: o2,sAIPW} as our default estimators, and we write $\hat \beta_\rct = \hat\beta_{c, \textsf{sAIPPW}}, \hat\beta_{\obs} = \hat\beta_{o_2, \textsf{sAIPW}}$  for notational simplicity.




% \begin{table}[]
% \centering
% \begin{tabular}{lll}
% Target population      & RCT & OBS \\ \hline
% Sources of bias for RCT-based estimators & None    &   External  \\
% Sources of bias for OBS-data-based estimators &  Internal+External   &    Internal \\
% Recommended RCT-based estimators          &   $\csaipw$  &  $\csaippw$   \\
% Recommended OBS-based estimators          &  $\osaipw$   &   $\oosaipw$  \\ \hline
% \end{tabular}
% \caption{Sources of bias and recommended choice of estimators based on the target population.}
% \label{table:choice_of_estimators}
% \end{table}


% Table \ref{table:choice_of_estimators} summarizes the sources of bias and the recommended choice of RCT-based and observational-data-based estimators for the PATE $\beta^\star$ based on the target population.










==> history/04-method_old.tex <==
%!TEX root = 00-main.tex

\section{Methodology}
\label{sec: method}
\subsection{An oracle procedure and its optimality}
% Let $\hat \beta_\rct$ be a generic estimator constructed using the RCT data and let $\hat \beta_\obs$ be another generic estimator constructed using the observational data. 
We have seen in Section \ref{subsec: external validity} that despite the presence of external validity bias, it is possible (under relatively weak assumptions) for $\hat\beta_\rct = \hat\beta_{c, \textsf{sAIPPW}}$ to consistently estimate the ground truth PATE $\beta^\star$.
In contrast, as demonstrated in Section \ref{subsec: internal validity}, constructing an estimator that consistently estimates $\beta^\star$ is in general impossible due to the potential internal validity bias in the observational data.
Rather, the best one could hope is the convergence of $\hat\beta_\obs = \hat\beta_{o_2, \textsf{sAIPW}}$ to some $\beta_\obs$ that is close to $\beta^\star$,
% Note that $\hat\beta_\rct$ (resp. $\hat\beta_\obs$) is unbiased for $\beta^\star_\rct$ (resp. $\beta_\obs$), and let $\sigma^2_\rct$ (resp. $\sigma^2_\obs$) be the asymptotic variance of $\hat\beta_\rct$ (resp. $\hat\beta_\obs$). 
and the discrepancy is quantified by
$$
\Delta =  \beta^\star - \beta_\obs.
$$

If the data analyst has prior knowledge on the magnitude of $\Delta$, a natural attempt to combine the two estimators (or two data sources) is to taking their convex combination:
\begin{equation}
	\label{eq:cvx_comb}
	\hat \beta_\weight := (1-\weight)  \hat\beta_\rct + \weight \hat\beta_\obs,
\end{equation}
where the weight $\omega$ may depend on $\Delta$.
Indeed, if $\Delta$ is excessively large, then incorporating the observational data can only hurt the performance of the final estimator, and the optimal strategy in this case is arguably only using the RCT data, i.e., setting $\omega = 0$.
In the other extreme, if $\Delta$ is negligibly small, then the optimal strategy becomes pooling the two data sources together (with proper weighting to adjust for the covariate shift). When $\hat\beta_\rct$ and $\hat \beta_\obs$ both admit asymptotic linear expansions, this pooling strategy corresponds to setting $\omega$ to a non-zero value that depends on the sample sizes.

In this subsection, we give a precise analysis on the performance of the estimator \eqref{eq:cvx_comb}.
 % and demonstrates its minimax optimality under a toy causal model. 
Unsurprisingly, the optimal choice of $\omega$ indeed depends on $\Delta$, rendering \eqref{eq:cvx_comb} an oracle procedure that is barely applicable in practice.
Nevertheless, such an analysis is still meaningful in that it serves as a benchmark on the rate of convergence we shall aim for when we design data-adaptive procedures in Section \ref{subsec: adaptive_procedure}.

\paragraph{The asymptotic mean squared error of $\boldsymbol{\hat \beta_\omega}$.}
% To keep the analysis versatile, 
We assume both $\hat\beta_\rct$ and $\hat\beta_\obs$ admit asymptotic linear expansions, as detailed below.
\begin{assumption}[Existence of asymptotic linear expansions]
\label{assump:asymp_linear}
Suppose there exist influence functions $\psi_\rct(X, A, Y)$, $\psi_\obs(X, A, Y)$ such that as $n_\rct \land n_{\obs_2} \to \infty$,
\begin{align*}
	\sqrt{n_\rct}(\hat\beta_\rct - \beta^\star) &  = \frac{1}{\sqrt{n_\rct}} \sum_{i\in \Rct}  \psi_\rct(\bfX_i, A_i, Y_i) +  o_p(1),\\
	\sqrt{n_{\obs_2}}(\hat\beta_\obs - \beta_\obs) &  = \frac{1}{\sqrt{n_{\obs_2}}} \sum_{i\in\Obs_2}  \psi_\obs(\bfX_i, A_i, Y_i) +  o_p(1).
\end{align*}
Moreover, the influence functions are mean zero with finite second and third moments given by
\begin{align*}
	\bbE[(\psi_\rct(\bfX_i, A_i, Y_i))^2] & = \sigma_\rct^2, \qquad
	\bbE[|\psi_\rct(\bfX_i, A_i, Y_i)|^3] = \rho_\rct, \qquad \forall i \in \Rct,\\
	\bbE[(\psi_\obs(\bfX_i, A_i, Y_i))^2] & = \sigma_\obs^2, \qquad
	\bbE[|\psi_\obs(\bfX_i, A_i, Y_i)|^3] = \rho_\obs, \qquad \forall i \in \Obs_2.
\end{align*}	
\end{assumption}
Based on the exposition in Section \ref{subsec: internal validity} and \ref{subsec: external validity}, the above assumption is satisfied by our default estimators $\hat \beta_\rct = \hat\beta_{c, \textsf{sAIPPW}}, \hat\beta_{\obs} = \hat\beta_{o_2, \textsf{sAIPW}}$.
We remark that there are other estimators for which the above assumption holds and our analysis is versatile enough to accommodate them. 

We assume the existence of finite third moments because our analysis takes advantage of Berry-Essen theorem. 
While this assumption could be relaxed, e.g., by invoking generalizations of Berry-Esseen theorem that only requires finite fractional moment \citep[Chapter 16]{feller2008introduction}, we do not pursue it in the current manuscript.

The following theorem characterizes the asymptotic mean squared error of $\hat\beta_\omega$.
\begin{theorem}[Performance of the oracle estimator]
\label{thm:amse_convex_comb}
Under Assumption \ref{assump:asymp_linear}, the estimator $\hat\beta_\weight$ satisfies
\begin{equation}
	\label{eq:amse_convergence_convex_comb}
	\sup_{\weight\in[0, 1]} \bigg|\frac{\bbE[|\hat\beta_\weight - \beta^\star|^2]}{\amse(\hat\beta_\weight)} - 1\bigg| \to 0 \qquad \textnormal{as }  n_\rct \land n_{\obs_2} \to \infty,
\end{equation}	
where the asymptotic mean squared error is given by
\begin{equation}
	\label{eq:amse_formula_convex_comb}
	\amse(\hat\beta_\weight) = 
	\frac{(1-\weight)^2 \sigma_\rct^2}{n_\rct} + \frac{\weight^2 \sigma_\obs^2}{n_{\obs_2}} + \weight^2\Delta^2.
\end{equation}	
Meanwhile, the optimal weight is given by
$
	\weight^\star = \frac{\sigma_\rct^2/n_\rct}{\sigma_\rct^2/n_\rct + \sigma_\obs^2/n_{\obs_2} + \Delta^2},
$
in which case the optimal asymptotic mean squared error becomes
\begin{equation}
	\label{eq:opt_amse_convex_comb}
	\min_{\weight\in[0, 1]} \amse(\hat\beta_\weight) = \amse(\hat\beta_{\weight^\star}) = \frac{\sigma_\rct^2}{n_\rct} \cdot \frac{\sigma_\obs^2 / n_{\obs_2} + \Delta^2}{\sigma_\rct^2/n_\rct + \sigma_\obs^2/n_{\obs_2} + \Delta^2}.
\end{equation}	
\end{theorem}
\begin{proof}
	See Appendix \ref{prf:thm:amse_convex_comb}.
\end{proof}

The optimal weight $\omega^\star$ is a function of $\Delta$ with a form that well matches our intuition. If $\Delta$ is large, then $\omega^\star$ is close to zero, meaning the optimal convex combination is close to using $\hat\beta_\rct$ alone. If $\Delta$ is small, then $\omega^\star$ becomes a function of the noise levels and the effective sample sizes. In the latter case, if we additionally assume $\sigma_\obs^2/n_{\obs_2} \ll \sigma_\rct^2/n_\rct$ (i.e., the observational data are much more abundant than the RCT data), then $\weight^\star$ is close to $1$, meaning that the optimal convex combination is close to using $\hat\beta_\obs$ alone.

The following proposition re-expresses the rate of convergence \eqref{eq:opt_amse_convex_comb} into a more interpretable form.
\begin{proposition}[Alternative representation for the optimal \amse]
\label{prop:amse_convex_comb_alt_formula}
	Assume $\sigma_\rct^2/n_\rct \gtrsim \sigma_\obs^2/n_{\obs}$ and $n_\obs \geq (1+\ep)n_\rct$ for some absolute constant $\ep > 0$ (i.e., the observational data are more abundant than the RCT data), then 
	\begin{equation}
		\label{eq:amse_convex_comb_alt_formula}
		\amse(\hat\beta_{\weight^\star}) \asymp \frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} + \frac{\sigma_\rct^2}{n_\rct} \land \Delta^2 
		\asymp
		\begin{cases}
			\frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} & \textnormal{if } \Delta^2 \lesssim \frac{\sigma_\rct^2}{n_\rct}
			\\[5pt]
			\frac{\sigma_\rct^2}{n_\rct} &  \textnormal{ if} \Delta^2 \gtrsim \frac{\sigma_\rct^2}{n_\rct}
		\end{cases}
	\end{equation}	
\end{proposition}
\begin{proof}
	See Appendix \ref{prf:prop:amse_convex_comb_alt_formula}. 
\end{proof}
The formula \eqref{eq:amse_convex_comb_alt_formula} gives a characterization on the role of $\Delta$ in the asymptotic mean squared error of $\hat\beta_{\weight^\star}$. 
When $\Delta^2 \lesssim \sigma_\rct^2/n_\rct$, the right-hand side of \eqref{eq:amse_convex_comb_alt_formula} becomes $\Theta\left(\frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2}\right)$, a rate that is of the same order as $\amse(\beta_{\hat\omega^\star})$ \emph{as if} $\Delta = 0$.
When $\Delta^2 \gtrsim \sigma_\rct^2/n_\rct$, then the right-hand side of \eqref{eq:amse_convex_comb_alt_formula} becomes $\Theta\left(\frac{\sigma_\rct^2}{n_\rct}\right)$, a rate  that is of the same order as $\amse(\hat \beta_{\omega^\star})$ \emph{as if} $\Delta = \infty$.
Recall that when $\Delta = 0$, the estimator $\hat \beta_{\omega^\star}$ is constructed essentially by pooling the two data sources together, whereas when $\Delta = \infty$, it is constructed by using $\hat\beta_\rct$ alone.
Disregarding the constant factors, the above proposition gives a curious phase transition between two extreme strategies: if $\Delta^2\lesssim \sigma_\rct^2/n_\rct$, then pooling the two data sources together can achieve the same performance as the optimal convex combination $\hat\beta_{\weight^\star}$; if $\Delta^2\gtrsim \sigma_\rct^2/n_\rct$, then using the RCT data alone can achieve the same performance as $\hat\beta_{\weight^\star}$.
Such a phase transition has been identified in other statistical problems that involve multiple data sources \citep{chen2021theorem}.




Curious readers may wonder if the rate \eqref{eq:amse_convex_comb_alt_formula}, achieved by the best convex combination, is information-theoretically optimal among all algorithms.
In fact, we can construct a simple data-generating process, under which \emph{any} algorithm that attempts to estimate $\beta^\star$ must suffer from a mean-squared error of order $\Omega\left( \frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} + \frac{\sigma_\rct^2}{n_\rct} \land \Delta^2\right)$. This confirms the minimax optimality of the best convex combination. For brevity, we defer the lower bound arguments to Appendix \ref{appx:lb}.




\subsection{An adaptive procedure: NAME}\label{subsec: adaptive_procedure}
% We consider an algorithm that achieves the same rate as the best convex combination.
% Notably this algorithm does not require a correct specification of $\Delta = \beta_\rct^\star - \beta^\star_\rct|$.
In this section, we design a fully adaptive estimator and prove that it achieves nearly the same performance as the best convex combination $\hat\beta_{\weight^\star}$, up to poly-log factors.

We start by constructing an preliminary estimator that pools all the data together:
$$
	\tilde \beta : =  (1-\hat\weight) \hat\beta_\rct + \hat\weight  \hat \beta_\obs, \qquad \hat \weight = \frac{\hat \sigma_\rct^2/n_\rct}{\hat \sigma_\rct^2/n_\rct + \sigma_\obs^2/n_{\obs_2}},
$$
where $\hat\sigma_\rct$ and $\hat\sigma_\obs$ are estimators of $\sigma_\rct$ and $\sigma_\obs$, respectively.
Since $\beta_\obs \neq \beta^\star$, the above estimator is biased, and the magnitude of the bias is $\hat \weight |\Delta|$.
We then try to de-bias $\tilde\beta$ by estimating $\Delta$. 
A natural estimator is given by
$$
	\tilde \Delta = \hat \beta_\rct - \hat \beta_\obs.
$$
If we use the above estimator to de-bias $\tilde \beta$, the final estimator would be $\hat\beta = \tilde \beta + \hat\weight\tilde\Delta$, i.e., we get back to $\hat\beta_\rct$, leading to no efficiency gain. Thus, we need more work.

Let us make two observations. First, we know that $\tilde \Delta$, after a proper scaling, is asymptotically Gaussian as $n_\rct \land n_{\obs_2}\to\infty$, and the asymptotic mean and variance of $\tilde \Delta$ are given by $\Delta$ and ${\sigma_\rct^2}/{n_\rct} + {\sigma_\obs^2}/{n_{\obs_2}}$, respectively. A standard concentration of measure argument gives that $|\Delta - \tilde \Delta| \lesssim \sqrt{\log(n_\rct \land n_{\obs_2}) \cdot ({\sigma_\rct^2}/{n_\rct} + {\sigma_\obs^2}/{n_{\obs_2}})}$ with high probability.
Second, we know that to potentially take advantage of the observational data, we need $\Delta$ to be relatively small. The above two observations motivate the following procedure:
% This looks like estimating a sparse Gaussian signal, so we can use Lasso-type algorithms to adapt to unknown $\Delta$. More concretely, let us consider
\begin{equation}
	\label{eq:est_delta}
    \hat \Delta = \argmin_{\delta} |\delta| \qquad \textnormal{subject to } |\delta - \tilde \Delta| \leq \sfc \sqrt{\log (n_\rct\land n_{\obs_2})} \cdot
    \sqrt{\frac{\hat\sigma_\rct^2}{n_\rct} + \frac{\hat\sigma_\obs^2}{n_{\obs_2}}},
\end{equation} 
where $\sfc > 0$ is a hyperparameter. Intuitively, the above procedure selects a $\hat\Delta$ with the minimum absolute value (based on our second observation), among all ``plausible'' candidates, where the ``plausibility'' is quantified by our first observation.

Such a procedure is reminiscent of many well-known methods in high-dimensional statistics, such as the Dantzig selector in sparse linear models \citep{candes2007dantzig} and nuclear norm minimization in matrix completion \citep{candes2009exact,candes2010power}, where one seeks for an estimator that minimizes certain complexity measures (in our case, the absolute value) subject to a constraint that ensures the error control.

Note that \eqref{eq:est_delta} can be solved via soft-thresholding: 
$$
	\hat \Delta = 
	\begin{cases}
		\textnormal{sgn}(\tilde \Delta) \cdot \bigg(|\tilde \Delta| - \sfc \sqrt{\log (n_\rct\land n_{\obs_2})} \cdot
    	\sqrt{\frac{\hat\sigma_\rct^2}{n_\rct} + \frac{\hat\sigma_\obs^2}{n_{\obs_2}}}\bigg)
    	& \textnormal{ if } 
    	|\tilde \Delta| \geq \sfc \sqrt{\log (n_\rct\land n_{\obs_2})} \cdot
    	\sqrt{\frac{\hat\sigma_\rct^2}{n_\rct} + \frac{\hat\sigma_\obs^2}{n_{\obs_2}}},\\
    	0
    	& \textnormal{ otherwise}.
	\end{cases}
$$
Thus, one can alternatively think of \eqref{eq:est_delta} as a LASSO-type estimator \citep{tibshirani1996regression} that minimizes $|\tilde \Delta - \delta|^2 + \lambda |\delta|$ for a particular choice of $\lambda$.

Once $\hat\Delta$ is obtained, the final estimator for $\beta^\star$ is given by 
\begin{equation}
	\label{eq:final_estimator}
	\hat \beta = \tilde \beta + \hat\weight  \hat \Delta.
\end{equation}	
The following theorem shows that $\hat\beta$ achieves nearly the same performance as the best convex combination $\hat\beta_{\weight^\star}$ with high probability, up to poly-log factors.
% \sxc{Another route is to assume stronger tail behaviors of the response and the covariates, e.g., sub-gaussian. And this route will give us stronger results, e.g., in expectation bound}.
% that only assumes $\hat \beta_\obs$ and $\hat \beta_\rct$ both exhibit a central limit behavior.
% \begin{assump}[Central limit behavior]
% Assume that for any $t\in \bbR$, we have
% $$
% 	\bigg|\bbP\bigg( \frac{\sqrt{n_\rct}|\hat \beta_\rct - \beta_\rct^\star|}{\sigma_\rct} \leq t\bigg) - \Phi(t)\bigg| \leq  \sfC_\rct n_\rct^{-\sfc_\rct}, 
% 	\qquad 
% 	\bigg|\bbP\bigg( \frac{\sqrt{n_\rct}|\hat \beta_\obs - \beta_\obs^\star|}{\sigma_\obs} \leq t\bigg) - \Phi(t)\bigg| \leq  \sfC_\obs n_{\obs_2}^{-\sfc_\obs},
% $$
% where $\Phi(t)$ is the CDF of $N(0, 1)$.
% \end{assump}
% For simplicity, we assume the propensity scores are exactly known, so that both estimators $\hat\beta_\rct$ and $\hat\beta_\obs$ are simply the average of i.i.d.~random variables. 
% Say $\hat \beta_\rct = \sum_{i=1}^{n_\rct} \phi_i/n_\rct$ and $\hat \beta_\obs = \sum_{i=1}^{n_{\obs_2}}\psi_i/n_{\obs_2}$.
% Let $\rho_\rct = \bbE|\phi_i - \beta_\rct^\star|^3$ and $\rho_\obs = \bbE |\psi_i - \beta_\obs^\star|^3$.
% \sxc{when propensity scores are estimated, arguments largely remain the same but we need to make assumptions on the rate of convergence.}

\begin{theorem}[Performance of the adaptive estimator]
\label{thm:high_prob_bound_adaptive_estimator}
Let Assumption \ref{assump:asymp_linear} hold. In addition, assume $\sigma_\rct^2/n_\rct\gtrsim \sigma_\obs^2/n_{\obs}$ and $n_\obs \geq (1+\ep)n_\rct$ for some absolute constant $\ep > 0$. If $\hat\sigma_\rct \overset{p}{\to} \sigma_\rct$ and $\hat\sigma_\obs \overset{p}{\to} \sigma_\obs$ as $n_\rct \land n_\obs \to \infty$, then with probability at least $1-o(1)$, we have
\begin{equation}
	\label{eq:high_prob_bound_adaptive_estimator}
	 |\hat\beta - \beta^\star|^2 \lesssim  \log(n_\rct\land n_{\obs_2})\cdot \bigg(\frac{\sigma_\rct^2 \sigma_\obs^2}{n_\rct \sigma_\obs^2 + n_{\obs} \sigma_\rct^2} + \frac{\sigma_\rct^2}{n_\rct} \land \Delta^2\bigg).
\end{equation} 
\end{theorem}


\begin{proof}
	See Appendix \ref{prf:thm:high_prob_bound_adaptive_estimator}.
\end{proof}

Inspecting the proof, one can readily check that the probability that the above bound holds is of the form $1 - (n_\rct\land n_{\obs})^{-\sfc'} - o(1)$, where $\sfc'$ is some absolute constant depending on $\sfc$ and the $o(1)$ depends on the rate of convergence of $\hat\sigma_\rct$ and $\hat\sigma_\obs$, as well as the two $o_p(1)$ terms appeared in the asymptotic linear expansion of $\hat\beta_\rct$ and $\hat\beta_\obs$. 
Meanwhile, the $\log(n_\rct \land n_\obs)$ term in the right-hand side of \eqref{eq:high_prob_bound_adaptive_estimator} can be replaced by any sequence that slowly diverges to infinity without hurting the validity of the above theorem.










% \textcolor{blue}{
% OLD: 
% Consider the following estimator:
% $$
% 	\hat\beta \in \argmin_{\beta} |\beta - \hat\beta_\rct| \qquad \textnormal{s.t. } |\beta - \hat \beta_\obs| \leq |\Delta| + \frac{\sfc \cdot \sigma_\obs}{\sqrt{n_{\obs_2}}},
% $$
% where $\sfc$ is any constant strictly greater than $1$. Then, the \amse~of this estimator is of the same order as the best convex combination and the pool-and-debias estimator. The proof is based on the fact that $\hat\beta$ is close to $\hat\beta_\obs$ and that $\beta^\star_\rct$ is a feasible solution. 
% }



\subsection{Post-transfer/post-integration inference}

\paragraph{Inverting hypothesis tests with 1-D grid search and Bonferroni correction.}
Let $\sigma_\Delta = \sqrt{\frac{\sigma_\rct^2}{n_\rct} + \frac{\sigma_\obs^2}{n_{\obs_2}}}$.
Note that the asymptotic distribution of $\tilde \Delta$ is known:
$
    \frac{\tilde \Delta - \Delta}{\sigma_\Delta} \Rightarrow N(0, 1).
$
Fix a constant $\delta \in \bbR$ and consider testing the hypothesis $H_0: \Delta = \delta$. 
Since the asymptotic distribution of $\tilde\Delta$ is known, we can construct the null distribution of $\hat \Delta$ by Monte Carlo and construct a valid $p$-value.
Running this procedure multiple times and collecting all $\delta$'s for which the null cannot be rejected, we get a valid confidence interval for $\Delta$.  \sxc{this now looks a bit spurious to me because the transformation from $\tilde\Delta$ to $\hat\Delta$ depends on the sample sizes.}

We are dealing with an 1-D parameter, so doing simulation won't be too costly. If our original parameter of interest were a vector, then we would need tools from post selection inference \citep{berk2013valid,lee2016exact} because we are essentially doing ``dataset selection'' as opposed to variable selection.

On the other hand, constructing a valid confidence interval for $\weight \beta_\obs + (1-\weight) \beta_\rct$ from $\tilde \beta$ is easy, as $\tilde\beta$ is asymptotically normal after re-scaling. Thus, we can construct a valid confidence interval for $\beta_\rct^\star = \weight \beta_\obs + (1-\weight) \beta_\rct + \weight \Delta$ using Bonferroni correction.

\paragraph{Inverting hypothesis tests with 2-D grid search.}
Fix two constants $b_\rct, b_\obs$ and consider the null hypothesis $H_0: \beta_\rct^\star = b_\rct, \beta_\obs = b_\obs$. Under $H_0$, the asymptotic distributions of all quantities involved in the construction of $\hat\beta$, namely $\tilde\beta, \tilde\Delta, \hat \Delta$, are known by Monte Carlo. We can then construct a histogram of the null distribution of $\hat\beta$, and compare it with the observed $\hat\beta$ to get a valid $p$-value for testing $H_0$. Run this procedure multiple times and collect all pairs of $(b_\rct, b_\obs)$ for which the null cannot be rejected. We then project this ``plausible'' region of values of $(b_\rct, b_\obs)$ to the first coordinate to get a valid confidence interval of $\beta^\star_\rct$. \sxc{This also looks spurious to me for the same reason as above.}

% This construction of confidence intervals is valid because of the following reason.
% Consider a random variable $Z$ which is asymptotically $N(0, 1)$. We essentially want the quantiles of $f(Z)$ to be well-approximated by the quantiles of $f(N(0, 1))$, where $f$ is a mapping representing our algorithm. Our algorithm, albeit non-smooth, is still continuous. So the continuous mapping theorem applies and we get $f(Z)$ has $f(N(0, 1))$ as its weak limit. In particular, all quantiles of $f(Z)$ can be approximated by $f(N(0, 1))$. \
% sxc{If we were using hard threshold, we may run into some trouble because of the discontinuity.}



\paragraph{Inverting hypothesis tests with 2-D grid search and the oracle test statistic.}
Fix two constants $b_\rct, b_\obs$ and again consider the null hypothesis $H_0: \beta_\rct^\star = b_\rct, \beta_\obs = b_\obs$. Under $H_0$, we know the value of $\Delta$ and we can thus construct a test statistic $\hat\beta_\Delta$ using the best convex combination, where we use the subscript $\Delta$ to emphasize that this estimate depends on $\Delta$. Moreover, the null distribution of $\hat\beta_\Delta$ is also known. So we can construct a valid $p$-value for $H_0$ with $\hat\beta_\Delta$ being the test statistic (as opposed to $\hat\beta$ in the previous approach). Inverting this test with 2-D grid search and projecting the confidence region to the $\beta^\star_\rct$ direction, we get a valid confidence interval for $\beta^\star_\rct$.
This approach is also valid --- it is just using a different test statistic every time we construct a confidence region. It has an additional benefit that we do not worry about the non-smoothness of the soft-thresholding operation. \sxc{The validity of this method is easy to prove. Not sure how long this interval will be. Also it looks like a form of sensitivity analysis to me.}

==> history/bias_old.tex <==


The $ \beta_o $ defined in \eqref{eq: beta o} is not necessarily equal to the target causal parameter  $ \beta_c^\star $ for two reasons: (i) there may be unmeasured confounding in the observational study, i.e., $ \beta_o\neq E( Y {(1)} -Y {(0)}   \mid S=o)$; (ii)  $ E( Y {(1)} -Y {(0)}   \mid S=o ) $ may not equal to $ \beta_c^\star $ due to nontransportability. How close $ \beta_o  $ is to $ \beta_c^\star $ depends on the magnitude of these two sources of bias. In the following, we give a theoretical analysis of the bias $ \beta_o-\beta_c^\star $.   

For reason (i), suppose there exists an unmeasured confounder $ U  $ that satisfies $ A  \perp ( Y(1), Y(0)) \mid U, X, S=o$. Let $ \pi_o(X, U) = P(A=1\mid X, U, S=o) $ and $  \gamma(X, U)= \text{OR} \{\pi_o(X, U), \pi_o(X) \} $, 
where 
\[
\text{OR} \{p_1, p_2\} =\frac{p_1/(1-p_1)}{p_2/(1-p_2)}. 
\]
 Then the bias from unmeasured confounding $  \beta_o -E( Y {(1)} - Y {(0)}  \mid S=o ) $ equals 
 \begin{align*}
 E\left[ \frac{AY(1-\pi_o(X))}{\pi_o(X)  } \left\{   1- \frac{1}{\gamma (X, U)}  \right\}  \mid S= o \right]  - E\left[ \frac{(1-A) Y\pi_o(X)}{1-\pi_o(X)} \left\{  1-\gamma(X, U)  \right\}  \mid S= o \right]     .
 \end{align*}
When $ \gamma(x, u)=1 $, it means no unmeasured confounding, and thus the bias due to unmeasured confounding equals zero. 

For reason (ii), for $ a\in \{0,1\} $, let 
\[
\lambda_a(y, x) = \frac{f_{Y(a)\mid X, S=o} (y\mid x, s=o)}{f_{Y(a)\mid X, S=c} (y\mid x, s=c)} = \text{OR} \{ P(S=o\mid Y(a), X=x), P(S=o\mid  X=x) \}. 
\]
Then the bias from nontransportability  $ E( Y {(1)}  -Y {(0)}   \mid S=o ) - \beta_c^\star $ equals 
\begin{align*}
 E( Y {(1)} (\lambda_1(Y(1), X) - 1) \mid S=c ) -  E( Y {(0)} (\lambda_0(Y(0), X)  -1) \mid S=c )  . 
\end{align*}
When $ \lambda_0(x, u)=\lambda_1(x, u)=1 $, it means that the transportability assumption holds, and thus the bias due to nontransportability equals zero. 


Combining both, we know that the bias of $ \beta_o $  can be written as  
\begin{align*}
 &  \beta_o - \beta_c^\star  =  \beta_o -E( Y {(1)} - Y {(0)}   \mid S=o )  + E( Y {(1)}  -Y {(0)}   \mid S=o ) - \beta_c^\star   \\
&=  E\left[ \frac{AY(1-\pi_o(X))}{\pi_o(X)  } \left\{   1- \frac{1}{\gamma (X, U)}  \right\}  \mid S= o \right]  - E\left[ \frac{(1-A) Y\pi_o(X)}{1-\pi_o(X)} \left\{  1-\gamma(X, U)  \right\}  \mid S= o \right]     \\
& \qquad  + E( Y {(1)} (\lambda_1(Y(1), X) - 1) \mid S=c ) -  E( Y {(0)} (\lambda_0(Y(0), X)  -1) \mid S=c )  . 
\end{align*}
Using Cauchy-Schwartz inequality,  we can bound $  \beta_o - \beta_c^\star $ as follows 
\begin{align}
	\begin{split}
	(\beta_o - \beta_c^\star)^2  & \lesssim E\left[ Y {(1)}^2  \mid S=c \right] E\left[ \{\lambda_1(Y(1), X) -1 \}^2\mid S=c \right]   \label{eq: bias} \\
	&\qquad +  E\left[ Y {(0)}^2  \mid S=c \right] E\left[ \{\lambda_0(Y(0), X)-1 \}^2\mid S=c \right]  \\
	&\qquad +   E\left[ \left\{\frac{AY(1-\pi_o(X))}{\pi_o(X)  }\right\}^2   \mid S= o \right] E\left[ \left\{ 1-\frac{1}{\gamma (X, U)}    \right\}^2\mid S=o\right]  \\
	&\qquad + E\left[ \left\{\frac{(1-A) Y \pi_o(X)}{1- \pi_o(X)  }\right\}^2   \mid S= o \right] E\left[ \left\{  1-\gamma(X, U) \right\}^2\mid S=o\right].  
\end{split}
\end{align}
where $ a\lesssim b  $ denotes that  there exists a constant $ C<\infty $ such that $ a\leq C b $.  \textcolor{red}{TY: I will clean up  the above equations.}



\emph{Remark.}  The analysis of bias is related to the sensitivity analysis that is a popular device to assess the sensitivity of the study conclusion to untestable assumptions. In particular, the  marginal  sensitivity analysis framework uses the supremum norm of $ \gamma(x, u) $ to quantify the deviation from the no unmeasured confounding assumption (Dorn and Guo, 2021), which may overstate the effect of unmeasured confounding in our analysis. Therefore, we instead use the integral norm  of $ \gamma(x, u) $. 



==> history/intro_old.tex <==

Randomized clinical trials (RCTs) have been considered the gold standard approach that generates the highest level evidence  for evaluating the causal effect of new medical products.  However, the traditional paradigm of assessing new treatments based on running large RCTs has become ever more expensive and time-consuming, which calls for new innovations and advances to accelerate medical product developments.  In the meantime, there is a proliferation of observational data that are collected for research or administrative purposes, such as disease registries, biobanks, administrative claims and electronic health records. Such massive and rich datasets and the exciting potentials of augmenting the current clinical development paradigm  have generated strong interest among industry, regulatory \citep{fda2018rwd}, and academia \citep{di2020real}. However, without proper randomization, there is often concern about confounding bias, in particular unmeasured confounding bias,  in  causal inference based on observational data \citep{Franklin:2021aa}. Therefore, an important question  is how to transfer knowledge from observational studies to improve  causal inference using only RCTs  without introducing bias. 

We consider the potential outcomes framework to formalize the causal inference question \citep{neyman1923application,rubin1974estimating}. Suppose that there exist a binary treatment indicator $ A $, baseline covariates $ X $, and a study indicator $ S$ which equals $ c $ if the subject is from the RCT, equals $ o $ if the subject is from the OS.  Let $ Y(a) $ be the potential outcome if $ A=a $, for $ a=0, 1 $.  


Much of the statistical literature on combining RCTs and  observational studies to better estimate casual effects 
can be divided into four main categories depending on the settings considered. The first category considers that the RCT and  observational study differs only in the covariate distribution $ (X\not \perp S) $ whereas the structural relationships between outcomes and covariates are the same ($ (Y(0), Y(1))\perp S\mid X $). Moreover, there is no unmeasured confounding in the observational study  ($ (Y(0), Y(1))\perp A\mid X, S=o $). This is so far the primary research setting and 




\begin{itemize}
    \item Setting 1: Let $P_X := P(X \mid S = 1)$ and $Q_X := P(X \mid S = 0)$ denote the marginal distribution in the clinical and observational dataset, and we have:
\[
f(Y(0), Y(1) \mid X) \mid S = 1 \quad = \quad f(Y(0), Y(1) \mid X) \mid S = 0,
\]
i.e., there is covariate shift and some version of the transportability assumption holds (i.e., the potential outcome distributions in the clinical dataset (S = 1) are the same as those in the observational dataset (S = 0)). There is no unmeasured confounding in observational dataset.

It seems the simplest approach in this case is importance weighting, and this is so far the primary research setting.

\item Setting 2: let $P = f(Y(0), Y(1), X \mid S = 1)$ and $Q = f(Y(0), Y(1), X \mid S = 0)$, $P \neq Q$, and there exists some high-level measure that quantifies the discrepancy between $P$ and $Q$. In other words, there may be both covariate shift ($X$ different) and posterior drift ($Y(\cdot)|X$ different). \sxc{label shift means $Y(\cdot)$s are different.}

\item Setting 3: There is covariate shift so that $P_X \neq Q_X$; for the moment, let us assume the transportability assumption holds so that $f(Y(0), Y(1), X \mid S = 1) = f(Y(0), Y(1), X \mid S = 0)$. However, there may exist unmeasured confounding in the observational dataset, i.e., $S = 0$, so that the usual IPWE does not estimate the average potential outcome over $Q_X$, i.e.,
\[
\sum_{i = 1}^{n_Q} \frac{A_i Y_i}{e(X_i)} \not\rightarrow \mathbb{E}_{X \sim Q_X, Y(0)\sim Q}[Y(1)]
\]
even as $n_Q \rightarrow \infty$. This setting is technically similar to, but conceptually different from Setting $2$. We can also think of Setting 3 as if the transportability assumption fails.  \citep{Kallus2018, yang2020improved}. 

\item Setting 4: There is covariate shift, the transportability assumption does not hold, and there is unmeasured confounding in observational dataset. Again, we may think of the failure of the transportability assumption and the unmeausred confounding under one unified framework.

\end{itemize}

Different from our goal of using observational data to improve causal inference based on RCTs, we note that there is also a large literature on knowledge transfer from the other direction. That is,  generalizing or transporting the RCT conclusion to a more representative patient population using observational data \citep{Stuart:2001aa, Buchanan:2018aa, Dahabreh:2019aa, colnet2020causal, degtiar2021review}. 



==> history/setup_old.tex <==

From the target population, we obtain a random sample selected into the randomized clinical trial (RCT), indexed by $ S=c $, and a random sample selected into the observational study, indexed by $ S=o $ {\color{red} (do two datasets overlap?)}. Subjects that are not directly sampled into the study from the target population are indexed by $ S=t $.    
Specifically,  we obtain random samples $ \{(Y_i(1), Y_i(0), A_i, X_i, S_i=c ), i \in \mathcal{C}\}$ of size $ n_c= |\mathcal{C}| $ from the RCT, which are independent and identically distributed  according to $ P(Y(1), Y(0), A, X, S\mid S=c ) $, and random samples $ \{(Y_i(1), Y_i(0), A_i, X_i, S_i=o ), i  \in \mathcal{O}\} $  of size  $ n_o= |\mathcal{O}| $ from the  observational study, which are  independent and identically distributed according to $ P(Y(1), Y(0), A, X, S\mid S=o ) $. For every unit $ i $, the observed outcome is $ Y_i= Y_i(A_i) $. To simplify the notation, we drop the subscript $ i $ when referring to a general unit from the population. 


The following assumption is guaranteed by the random treatment assignment in the RCT and is crucial for the identification of $ \beta_c $.  

\begin{assumption}[Design of  RCT]  \label{assumption: rct}
$ A  \perp ( Y(1), Y(0), X) \mid S=c$ and $ P(A=1\mid S=c) $ is known. 
\end{assumption}


We first consider the case with no covariate shift, as stated by the following assumption.  The general situation with covariate shift will be considered later in Section 4. 
\begin{assumption}[No covariate shift]  \label{assumption: no covariate shift}
$ S\perp X $. 
\end{assumption}


\subsection{Review: Fully Robust Estimators in RCT and Their Counterparts in OS}


Let  the known probability of receiving treatment in RCT be $ \pi_c = P(A=1\mid S=c)$, the conditional probability of receiving  treatment in OS be $ \pi_o(X)= P(A=1\mid X, S=o ) $,  and the conditional means of the outcome in study $ s $ be $ \mu_{sa}(X)=E(Y\mid X, A=a, S=s) $ for $ a\in \{0,1\} $ and $ s \in \{c, o\}  $.  


There are many methods to identify the causal effect in the RCT. In this article, we consider two commonly used ones that are fully robust in RCT, the inverse probability weighting (IPW), and the augmented inverse probability weighting (AIPW).   Specifically, the method of IPW identifies $ \beta_c^\star $ from 
\begin{align}
 \beta_c^\star  = E \left[ \frac{AY }{\pi_c }   -  \frac{(1-A)Y}{1- \pi_c}  \mid S=c\right],   \label{eq: ipw}
\end{align}
and this gives the IPW estimator 
\begin{align}
\hat	\beta_{c, \text{IPW}}  = \frac{1}{n_c} \sum_{i\in \mathcal{C}}  \frac{A_i Y_i }{\pi_c} - \frac{(1-A_i) Y_i }{1- \pi_c} .  \nonumber
\end{align}
The method of  AIPW identifies $ \beta_c^\star $ from 
\begin{align}
\beta_c^\star  = E \left[ \frac{A(Y- \mu_{c1}(X) ) }{\pi_c }   -  \frac{(1-A)(Y-\mu_{c0}(X))}{1- \pi_c} + \mu_{c1}(X)-   \mu_{c0}(X) \mid S=c\right],  \label{eq: aipw}
\end{align}
and this gives the  AIPW estimator 
\begin{align}
\hat	\beta_{c, \text{AIPW}}    = \frac{1}{n_c} \sum_{i\in \mathcal{C}}\frac{A_i (Y_i -\mu_{c1} (X_i; \hat \alpha_{c1} ) )  }{\pi_c} - \frac{(1-A_i)(Y_i -\mu_{c0} (X_i; \hat \alpha_{c0} ) ) }{1- \pi_c} + \mu_{c1} (X_i; \hat \alpha_{c1} )   - \mu_{c1} (X_i; \hat \alpha_{c0} ) .  \nonumber
\end{align}
where $ \mu_{ca}(X; \alpha_{ca} ) $ is a parametric specification of the outcome mean model $  \mu_{ca}(X; \alpha_{ca} ) $, and $ \hat \alpha_{ca} $ is an estimator of $ \alpha_{ca} $. 
 
In RCT where  subjects are randomly assigned to two treatment arms as in Assumption \ref{assumption: rct},  the IPW estimator $ \hat	\beta_{c, \text{IPW}}  $  is fully robust in the sense that \eqref{eq: ipw} holds regardless of outcome generating process.  

We also define the IPW and AIPW counterparts based on OS.  We denote the parameter identified by IPW and AIPW in OS as $ \beta_{o} $, and the identification formulas are respectively as follows
\begin{align}
	\begin{split}
	\beta_o &= E \left[ \frac{AY }{\pi_o(X) }   -  \frac{(1-A)Y}{1- \pi_o(X)}  \mid S=o\right],  \label{eq: beta o}\\
  \beta_o  &= E \left[ \frac{A(Y- \mu_{o1}(X) ) }{\pi_o(X) }   -  \frac{(1-A)(Y-\mu_{o0}(X))}{1- \pi_o(X)} + \mu_{o1}(X)-   \mu_{o0}(X) \mid S=o \right]. 
\end{split}
\end{align} 
The corresponding IPW and AIPW estimators are  
\begin{align}
	\hat	\beta_{o, \text{IPW}} &= \frac{1}{n_o} \sum_{i\in \mathcal{O}}  \frac{A_i Y_i }{\pi_o(X_i; \hat \eta)} - \frac{(1-A_i) Y_i }{1- \pi_o(X_i; \hat \eta) } ,\nonumber\\
		\hat	\beta_{o, \text{AIPW}} &=  \frac{1}{n_o} \sum_{i\in \mathcal{O}}\frac{A_i (Y_i -\mu_{o1} (X_i; \hat \alpha_{o1} ) )  }{\pi_o(X_i; \hat\eta )} - \frac{(1-A_i)(Y_i -\mu_{o0} (X_i; \hat \alpha_{o0} ) ) }{1- \pi_o(X_i;\hat\eta)} + \mu_{o1} (X_i; \hat \alpha_{o1} )   - \mu_{o0} (X_i; \hat \alpha_{o1} ) , \nonumber
\end{align}
where $ \mu_{oa}(X; \alpha_{oa} ) $ is a parametric specification of the outcome mean model $  \mu_{oa}(X; \alpha_{oa} ) $, and $ \hat \alpha_{oa} $ is an estimator of $ \alpha_{oa} $. It is important to note that $ \beta_o $ has no causal interpretation under Assumptions \ref{assumption: rct}-\ref{assumption: no covariate shift}; it is also not necessarily equal or close to the target causal parameter $\beta_c^\star  $. 

{\color{red}Variance formulas}

(i) When $ \mu_{ca}(x; \alpha_{ca} )  $ are linear models, then $ \sqrt{n} (\hat\beta_{c,\text{AIPW} } - \beta_c^\star) $ is asymptotically normal, with mean 0 and variance 
\begin{align*}
	\frac{{\rm var} (Y(1) - X^T \alpha_{c1} )}{\pi_c} +  	\frac{{\rm var} (Y(0) - X^T \alpha_{c0} )}{1- \pi_c}  +  {\rm var} (X^T( \alpha_{c1} - \alpha_{c0}))
\end{align*} 

(ii)  When $ \mu_{oa}(x; \alpha_{oa} )  $ are linear models, $ \pi_o (X_i; \eta) $ is a logistic model,
  then $ \sqrt{n} (\hat\beta_{o,\text{AIPW} } - \beta_o) $ is asymptotically normal, with mean 0 and variance 
